The free energy of compressed lattice knots

A compressed knotted ring polymer in a confining cavity is modelled by a knotted lattice polygon confined in a cube in ${\mathbb Z}^3$. The GAS algorithm [17] is used to sample lattice polygons of fixed knot type in a confining cube and to estimate the free energy of confined lattice knots. Lattice polygons of knot types the unknot, the trefoil knot, and the figure eight knot, are sampled and the free energies are estimated as functions of the concentration of monomers in the confining cube. The data show that the free energy is a function of knot type at low concentrations, and (mean-field) Flory-Huggins theory [12,15] is used to model the free energy as a function of monomer concentration. The Flory interaction parameter of knotted lattice polygons in ${\mathbb Z}^3$ is also estimated.

==> Figures/figure11.tex <==


\beginpicture

\normalcolor
\color{black}
\setcoordinatesystem units <1400pt,250pt>
\axes{0}{0}{0}{0}{0.20}{0.8}{-0.05}
\axis left shiftedto x=0 label {\Large$\phi_0$} 
      ticks
      withvalues 0.4 /
      at 0.4 /
 /  
\axis bottom shiftedto y=0 %label {$\phi$} 
    ticks
    withvalues 0.1 /
    at 0.1 /
/

\put {\Large$L^{-4/3}$} at 0.15 -0.07


\setplotsymbol ({\fiverm.})

%% 01 phi0
\color{Maroon}
\plot  0.1575 0.1197   0.02703 0.004617  /
\multiput {$\bullet$} at %0.2311 0.1280  
0.1575 0.1197  0.1170 0.0768  0.0917 0.0534  0.0747 0.0394  0.0625 0.0310  0.0534 0.0250  0.0464 0.0204  0.0409 0.0176  
0.0364 0.0146  0.03271 0.01167 0.02963 0.006851  0.02703 0.004617 /
\put {$\phi_0$} at 0.17 0.12

\plot  0.1575 0.2388    0.02703 0.05805  /
\multiput {$\blacktriangle$} at 0.1575 0.2388  0.1170 0.1917  0.0917 0.1593  0.0747 0.1356  0.0625 0.1170  0.0534 0.1031  0.0464 0.0912  0.0409 0.0821  0.0364 0.0756 0.03271 0.06964 0.02963 0.06252  0.02703 0.05805 /
\put {$\phi_m$} at 0.17 0.24

%At minimum negative pressure
\plot  0.1575 0.1793   0.02703 0.03134  /
\multiput {$\blacklozenge$} at 0.1575 0.1793  0.1170 0.1310  0.0917 0.1021  0.0747 0.0812  0.0625 0.0689  0.0534 0.0589  0.0464 0.0503  0.0409 0.0462  0.0364 0.0401 0.03271 0.03477 0.02963 0.03398  0.02703 0.03134 /
\put {$\phi_c$} at 0.17 0.18



%% 31 phi0
\color{Blue}
\plot  0.1574 0.6271     0.0363 0.1358  /
\multiput {$\bullet$} at 0.1574 0.6271   0.1169 0.4662   0.0917 0.3622   0.0746 0.2901  0.0625  0.2421   0.0534  0.2037    0.0464    0.1734  0.0408  0.1522    0.0363 0.1358  0.0327  0.1210 0.0296  0.1094  0.02703 0.0993 /
\put {$\phi_0 (3_1)$} at 0.18 0.63

%% 41 phi0
\color{BrickRed}
\plot  0.1575 0.7169    0.0364 0.1534  /
\multiput {$\bullet$} at 0.1575 0.7169  0.1170 0.5302  0.0917 0.4100  0.0747 0.3329  0.0625 0.2754  0.0534 0.2334  0.0464 0.1982  0.0409 0.1721  0.0364 0.1534  0.0327  0.1359 0.0296 0.1229 0.02703 0.1123 /
\put {$\phi_0 (4_1)$} at 0.18 0.72

%%There is no minimum in the free energy



\color{black}
\normalcolor


\color{blue}

\normalcolor
\color{black}

\endpicture

==> Figures/figure12.tex <==


\beginpicture

\normalcolor
\color{black}
\setcoordinatesystem units <70pt,4.25pt>
\axes{0}{-10}{0}{0}{4}{30}{-1}
\axis left shiftedto x=0 label {\Large$\Pi_{01} L^{3}$} 
      ticks
      withvalues 10 20  /
      at 10 20  /
 /  
\axis bottom shiftedto y=0 %label {$\phi$} 
    ticks
    withvalues 1 2 3 /
    at 1 2 3 /
/

\put {\large$\phi\,L^{4/3}$} at 3.5 -5


\setplotsymbol ({\fiverm.})

\plot 0.40 0 0.40 -7 /
\put {$\phi_0L^{4/3}$} at 0.40 -10

\plot 2.3 0 2.3 -7 /
\put {$\phi_mL^{4/3}$} at 2.3 -10

\plot 1.1 0 1.1 -7 /
\put {$\phi_cL^{4/3}$} at 1.1 -10



%% 01 scaled

%L=3
\color{B03}
\multiput {\tiny{$\bullet$}} at
1.1217 0.1619  1.4422 0.2657  1.7627 2.6640  2.0832 5.8512  2.4037 9.0059  2.7242 13.8142  3.0447 20.6699    /


%L=4
\color{B04}
\multiput {\tiny{$\bullet$}} at
0.6945 0.6476  0.8929 -0.5376  1.0913 -0.9137  1.2898 -0.7789  1.4882 -0.1316  1.6866 0.9703  1.8850 2.2993  2.0835 3.7287  2.2819 5.2984  2.4803 7.0651  2.6787 9.0956  2.8772 11.4511  3.0756 14.1667  3.2740 17.2918  3.4724 20.8980  
 /

%L=5
\color{B05}
\multiput {\tiny{$\bullet$}} at
0.4788 1.6297  0.6156 0.2662  0.7524 -0.5506  0.8892 -1.1415  1.0260 -1.5232  1.1628 -1.5923  1.2996 -1.2814  1.4364 -0.8770  1.5732 -0.3396  1.7100 0.3389  1.8468 1.1226  1.9836 2.1642  2.1204 2.9630  2.2572 3.8851  2.3940 4.8901  2.5308 6.2851  2.6676 7.7605  2.8044 8.9983  2.9412 10.3271  3.0780 11.9991  3.2148 13.6730  3.3516 15.5771  3.4884 17.9188  3.6251 19.8151 
   /

%L=6
\color{B06}
\multiput {\tiny{$\bullet$}} at
0.3533 2.5787  0.4543 1.1622  0.5552 0.2353  0.6562 -0.5277  0.7571 -1.1554  0.8581 -1.6127  0.9590 -1.9261  1.0600 -2.0674  1.1609 -2.0602  1.2619 -1.9531  1.3628 -1.6771  1.4638 -1.3113  1.5647 -0.8858  1.6657 -0.3698  1.7666 0.1430  1.8676 0.7350  1.9685 1.4235  2.0695 2.0783  2.1704 2.7224  2.2714 3.4666  2.3724 4.2524  2.4733 5.0192  2.5743 5.8486  2.6752 6.7635  2.7762 7.7777  2.8771 8.8276  2.9781 9.8756  3.0790 11.0173  3.1800 12.2264  3.2809 13.4442  3.3819 14.7078  3.4828 16.0358  3.5838 17.4690  3.6847 18.9490  3.7857 20.4806
  /

%L=7
\color{B07}
\multiput {\tiny{$\bullet$}} at
0.2733 3.4115  0.3514 1.9801  0.4294 1.0142  0.5075 0.2301  0.5856 -0.4646  0.6637 -1.1143  0.7417 -1.5890  0.8198 -1.9852  0.8979 -2.2769  0.9760 -2.4068  1.0541 -2.5146  1.1321 -2.5143  1.2102 -2.4070  1.2883 -2.2868  1.3664 -2.0719  1.4445 -1.7906  1.5225 -1.5147  1.6006 -1.1095  1.6787 -0.7005  1.7568 -0.3597  1.8349 0.1446  1.9129 0.6029  1.9910 1.0246  2.0691 1.5842  2.1472 2.0902  2.2252 2.5744  2.3033 3.2225  2.3814 3.8020  2.4595 4.4105  2.5376 5.0649  2.6156 5.6769  2.6937 6.4381  2.7718 7.1233  2.8499 7.9012  2.9280 8.7934  3.0060 9.5532  3.0841 10.3562  3.1622 11.2628  3.2403 12.1545  3.3184 13.0636  3.3964 14.0167  3.4745 14.9871  3.5526 16.0832  3.6307 17.1849  3.7087 18.3095  3.7868 19.5097  3.8649 20.6313 
   /

%L=8
\color{B08}
\multiput {\tiny{$\bullet$}} at
0.2188 4.1830  0.2812 2.7554  0.3438 1.8364  0.4062 1.0125  0.4688 0.2099  0.5312 -0.3709  0.5938 -0.9562  0.6562 -1.5401  0.7188 -1.9103  0.7812 -2.3850  0.8438 -2.4659  0.9062 -2.6089  0.9688 -2.9501  1.0312 -2.9334  1.0938 -2.9989  1.1562 -2.8636  1.2188 -3.0156  1.2812 -2.8317  1.3438 -2.5332  1.4062 -2.5806  1.4688 -2.0459  1.5312 -2.0421  1.5938 -2.1273  1.6562 -1.6810  1.7188 -1.0554  1.7812 -0.1235  1.8438 -0.1247  1.9062 0.7897  1.9688 1.6820  2.0312 0.2536  2.0938 0.7315  2.1562 1.9985  2.2188 1.7973  2.2812 2.5503  2.3438 3.4668  2.4062 3.6279  2.4688 3.8842  2.5312 4.6262  2.5938 4.7884  2.6562 5.5433  2.7188 5.5806  2.7812 4.9318  2.8438 8.7958  2.9062 9.7529  2.9688 6.8560  3.0312 8.6275  3.0938 9.8194  3.1562 8.8263  3.2188 12.6420  3.2812 13.6389  3.3438 12.6400  3.4062 13.8658  3.4688 12.3943  3.5312 14.5673  3.5938 15.1600  3.6562 16.8271  3.7188 16.9127  3.7812 16.4299  3.8438 19.5195  3.9062 22.8716
   /

%L=9
\color{B09}
\multiput {\tiny{$\bullet$}} at
0.1798 4.8301  0.2311 3.4021  0.2825 2.4240  0.3338 1.4800  0.3852 0.8228  0.4366 0.2004  0.4879 -0.4392  0.5393 -0.7728  0.5906 -1.0499  0.6420 -1.7174  0.6934 -2.2856  0.7447 -2.5585  0.7961 -2.6226  0.8474 -2.5342  0.8988 -2.9272  0.9502 -3.1929  1.0015 -3.0464  1.0529 -2.8229  1.1042 -3.0497  1.1556 -3.0001  1.2070 -3.5435  1.2583 -3.8123  1.3097 -2.8804  1.3610 -2.8729  1.4124 -2.7108  1.4638 -2.5874  1.5151 -2.0022  1.5665 -1.4869  1.6178 -1.0774  1.6692 -1.3583  1.7206 -1.7246  1.7719 -1.1788  1.8233 -0.9535  1.8746 -1.4891  1.9260 0.0490  1.9774 0.0976  2.0287 0.1378  2.0801 2.0179  2.1314 0.6676  2.1828 1.7600  2.2342 1.8606  2.2855 1.6201  2.3369 3.2407  2.3882 3.6906  2.4396 3.3784  2.4910 3.6068  2.5423 4.9218  2.5937 5.5564  2.6450 4.8943  2.6964 5.3364  2.7478 5.2884  2.7991 4.4632  2.8505 5.9246  2.9018 5.5589  2.9532 7.0848  3.0046 10.4818  3.0559 10.5579  3.1073 11.0890  3.1586 11.0220  3.2100 11.6178  3.2614 12.5157  3.3127 12.6426  3.3641 13.0195  3.4154 14.5335  3.4668 14.0111  3.5182 11.4342  3.5695 15.5175  3.6209 17.8321  3.6722 16.9207  3.7236 17.9195  3.7750 17.0245
 /

%L=10
\color{B10}
\multiput {\tiny{$\bullet$}} at
0.1508 5.4301  0.1939 4.0416  0.2370 3.0725  0.2801 2.1569  0.3232 1.3099  0.3663 0.6620  0.4093 0.3153  0.4524 -0.2108  0.4955 -0.7207  0.5386 -1.1992  0.5817 -1.5536  0.6248 -1.9775  0.6679 -2.4341  0.7110 -2.4612  0.7541 -2.8373  0.7971 -2.7607  0.8402 -3.1919  0.8833 -3.3306  0.9264 -3.0457  0.9695 -3.8626  1.0126 -3.4591  1.0557 -2.9662  1.0988 -3.2661  1.1419 -3.5392  1.1849 -3.2662  1.2280 -3.2257  1.2711 -3.6004  1.3142 -3.8102  1.3573 -3.9617  1.4004 -3.4568  1.4435 -2.3676  1.4866 -2.2381  1.5296 -2.1810  1.5727 -3.1008  1.6158 -3.3456  1.6589 -1.3299  1.7020 -1.0375  1.7451 -0.8360  1.7882 -0.6259  1.8313 -0.1319  1.8744 -0.0589  1.9174 -0.8583  1.9605 -0.4202  2.0036 0.2674  2.0467 1.6823  2.0898 1.5376  2.1329 0.5578  2.1760 0.6003  2.2191 1.0316  2.2622 2.3381  2.3052 2.6367  2.3483 2.2970  2.3914 2.6304  2.4345 3.6708  2.4776 4.1700  2.5207 2.3333  2.5638 4.0325  2.6069 5.7697  2.6500 3.8180  2.6930 3.8265  2.7361 4.8513  2.7792 5.7052  2.8223 6.2675  2.8654 8.7256  2.9085 9.0647  2.9516 5.9325  2.9947 6.9604  3.0378 8.3279  3.0808 9.8742  3.1239 11.7506  3.1670 12.6525  3.2101 11.2006  3.2532 7.9221  3.2963 10.2522  3.3394 12.1315  3.3825 13.3004  3.4256 13.1646  3.4686 11.9626  3.5117 13.0704  3.5548 15.8444  3.5979 15.1777  3.6410 14.7953  3.6841 18.3392  3.7272 17.1623  3.7703 16.5907  3.8133 17.4624  3.8564 19.1083  3.8995 22.7408  3.9426 21.4634  3.9857 22.8165
  /

%L=11
\color{B11}
\multiput {\tiny{$\bullet$}} at
0.1287 5.9609  0.1654 4.5055  0.2022 3.6018  0.2389 2.7928  0.2757 1.9163  0.3125 1.3066  0.3492 0.8305  0.3860 0.1518  0.4227 -0.4834  0.4595 -0.8469  0.4963 -1.4906  0.5330 -1.9710  0.5698 -1.9986  0.6065 -1.9792  0.6433 -2.0535  0.6801 -2.3222  0.7168 -2.7607  0.7536 -2.8928  0.7903 -2.8889  0.8271 -2.9494  0.8639 -2.9559  0.9006 -3.4322  0.9374 -3.2907  0.9741 -3.7382  1.0109 -4.1788  1.0477 -3.8250  1.0844 -3.7305  1.1212 -3.8280  1.1579 -3.9216  1.1947 -3.3701  1.2315 -3.0332  1.2682 -3.8473  1.3050 -3.7892  1.3417 -3.4163  1.3785 -3.4042  1.4153 -3.0490  1.4520 -3.0295  1.4888 -3.2540  1.5255 -2.8829  1.5623 -3.7147  1.5991 -3.3236  1.6358 -0.5842  1.6726 -2.7897  1.7093 -3.8151  1.7461 -2.4307  1.7829 -1.8622  1.8196 -1.0213  1.8564 0.4158  1.8931 1.5067  1.9299 -2.2613  1.9667 -2.1329  2.0034 0.8592  2.0402 -1.1548  2.0769 -1.0458  2.1137 0.7312  2.1505 2.0269  2.1872 1.9736  2.2240 1.6535  2.2607 2.1492  2.2975 1.7286  2.3343 3.3412  2.3710 3.6183  2.4078 2.3126  2.4445 3.1275  2.4813 3.1770  2.5181 5.4063  2.5548 6.1513  2.5916 2.8661  2.6283 6.9897  2.6651 6.8340  2.7019 4.4078  2.7386 7.8439  2.7754 6.5063  2.8121 6.1160  2.8489 8.1509  2.8857 7.4625  2.9224 5.8844  2.9592 7.6148  2.9959 8.8409  3.0327 8.7054  3.0695 6.7748  3.1062 6.3859  3.1430 9.4474  3.1797 11.5748  3.2165 11.3458  3.2533 10.2126  3.2900 10.1943  3.3268 10.7647  3.3635 12.7072  3.4003 10.8510  3.4371 10.5872  3.4738 11.2985  3.5106 12.0680  3.5473 15.8553  3.5841 14.2819  3.6209 16.2232  3.6576 19.9834  3.6944 15.7064  3.7311 14.1316  3.7679 16.8136  3.8047 20.5052  3.8414 24.9004  3.8782 15.7427  3.9149 12.3768  3.9517 22.7811  3.9885 21.9576 
 /

%L=12
\color{B12}
\multiput {\tiny{$\bullet$}} at
0.1113 6.5440  0.1431 5.0925  0.1749 4.0002  0.2067 3.2765  0.2385 2.5836  0.2703 1.6145  0.3021 1.0709  0.3339 0.7607  0.3657 0.0977  0.3975 -0.1252  0.4293 -0.4971  0.4611 -0.9890  0.4929 -1.3336  0.5247 -1.6246  0.5565 -2.0715  0.5883 -2.5243  0.6201 -2.5149  0.6519 -2.4386  0.6836 -2.5907  0.7154 -2.8982  0.7472 -3.5266  0.7790 -4.0580  0.8108 -3.7981  0.8426 -3.9001  0.8744 -4.2999  0.9062 -4.3462  0.9380 -3.9580  0.9698 -3.7018  1.0016 -4.1691  1.0334 -4.6451  1.0652 -3.8759  1.0970 -3.5431  1.1288 -4.3464  1.1606 -4.0916  1.1924 -3.2932  1.2242 -3.5258  1.2560 -4.2286  1.2878 -4.1980  1.3196 -3.3653  1.3514 -4.0447  1.3832 -3.9732  1.4150 -3.4510  1.4468 -3.5044  1.4786 -3.5220  1.5104 -3.9775  1.5422 -2.9379  1.5740 -2.3289  1.6058 -2.7244  1.6376 -2.5735  1.6694 -3.2431  1.7012 -2.7747  1.7330 -1.4755  1.7648 -1.7836  1.7966 -1.8866  1.8284 -3.0965  1.8602 -3.6133  1.8920 -1.9498  1.9238 1.0744  1.9556 0.3338  1.9874 -1.8193  2.0191 0.5491  2.0509 -1.2576  2.0827 -2.2739  2.1145 2.3708  2.1463 1.8946  2.1781 0.1408  2.2099 -0.0627  2.2417 0.9578  2.2735 2.7065  2.3053 2.4387  2.3371 1.3838  2.3689 1.0270  2.4007 2.2201  2.4325 3.2141  2.4643 2.5652  2.4961 2.7119  2.5279 3.4587  2.5597 3.7006  2.5915 4.2364  2.6233 5.5901  2.6551 5.3449  2.6869 3.9463  2.7187 4.3686  2.7505 7.4563  2.7823 6.1308  2.8141 4.4138  2.8459 7.1091  2.8777 8.2653  2.9095 8.0405  2.9413 7.9655  2.9731 8.4152  3.0049 7.7012  3.0367 7.1295  3.0685 7.7927  3.1003 8.4367  3.1321 8.9917  3.1639 9.6339  3.1957 7.1107  3.2275 8.5046  3.2593 11.3625  3.2911 12.8752  3.3229 12.2017  3.3546 10.0505  3.3864 11.6999  3.4182 12.0600  3.4500 13.1824  3.4818 15.2184  3.5136 15.0024  3.5454 15.0805  3.5772 17.1135  3.6090 16.4913  3.6408 17.0639  3.6726 16.9525  3.7044 15.4448  3.7362 18.8663  3.7680 19.3613  3.7998 17.5973  3.8316 16.8257  3.8634 20.8694  3.8952 21.5158  3.9270 17.7975  3.9588 20.3938  3.9906 21.1498
   /

%L=13
\color{B13}
\multiput {\tiny{$\bullet$}} at
0.0974 6.9297  0.1252 5.5675  0.1530 4.5489  0.1809 3.6306  0.2087 3.0390  0.2365 2.4159  0.2644 1.6773  0.2922 1.1639  0.3200 0.6023  0.3478 0.0910  0.3757 -0.2337  0.4035 -0.4203  0.4313 -0.8277  0.4591 -1.1797  0.4870 -1.4189  0.5148 -1.8667  0.5426 -2.5969  0.5704 -3.4632  0.5983 -3.3423  0.6261 -2.8687  0.6539 -3.2107  0.6817 -3.3512  0.7096 -3.5104  0.7374 -3.4999  0.7652 -3.5855  0.7931 -4.2780  0.8209 -3.9281  0.8487 -3.5497  0.8765 -4.1131  0.9044 -4.3808  0.9322 -4.4828  0.9600 -4.7102  0.9878 -4.7982  1.0157 -4.4608  1.0435 -4.9473  1.0713 -5.2131  1.0991 -5.1695  1.1270 -5.0674  1.1548 -4.7273  1.1826 -4.2301  1.2105 -3.7991  1.2383 -4.1795  1.2661 -4.3933  1.2939 -4.5382  1.3218 -4.1549  1.3496 -3.7349  1.3774 -2.9757  1.4052 -3.0377  1.4331 -3.3592  1.4609 -4.6344  1.4887 -5.0840  1.5165 -2.8181  1.5444 -2.6327  1.5722 -3.4619  1.6000 -4.5329  1.6278 -3.7162  1.6557 -0.6908  1.6835 0.6273  1.7113 -1.1460  1.7392 -3.9579  1.7670 -3.4139  1.7948 -3.0181  1.8226 -2.9144  1.8505 -0.1415  1.8783 0.3737  1.9061 -0.8307  1.9339 -0.4048  1.9618 -0.7423  1.9896 -2.2369  2.0174 -0.6383  2.0452 0.9392  2.0731 0.0771  2.1009 -0.1528  2.1287 0.8776  2.1565 1.1300  2.1844 1.8422  2.2122 2.4815  2.2400 2.1110  2.2679 2.8274  2.2957 2.2693  2.3235 1.8623  2.3513 2.5429  2.3792 3.3932  2.4070 3.1905  2.4348 3.7003  2.4626 4.6966  2.4905 3.5727  2.5183 2.5905  2.5461 3.0716  2.5739 2.4280  2.6018 3.7690  2.6296 4.7789  2.6574 3.7352  2.6853 5.6147  2.7131 7.6538  2.7409 6.3459  2.7687 5.4778  2.7966 9.0880  2.8244 7.4439  2.8522 8.3749  2.8800 8.3032  2.9079 5.3908  2.9357 10.1843  2.9635 8.2431  2.9913 7.0922  3.0192 11.6776  3.0470 11.9667  3.0748 9.4655  3.1026 8.8392  3.1305 10.0975  3.1583 8.3252  3.1861 7.9799  3.2140 10.5775  3.2418 11.4579  3.2696 12.0740  3.2974 11.5321  3.3253 12.6946  3.3531 14.5191  3.3809 14.3580  3.4087 13.3802  3.4366 13.2595  3.4644 14.7058  3.4922 14.9698  3.5200 16.7591  3.5479 13.7677  3.5757 12.7127  3.6035 16.3877  3.6314 15.5131  3.6592 15.3275  3.6870 10.0121  3.7148 13.8439  3.7427 17.4501  3.7705 16.5555  3.7983 16.7718  3.8261 15.0859  3.8540 17.1494  3.8818 19.9883  3.9096 21.5697  3.9374 19.3165  3.9653 18.2804  3.9931 18.6688 
/

%L=13
\color{B13}
\multiput {\tiny{$\bullet$}} at
0.0974 6.9524  0.1252 5.5531  0.1530 4.5719  0.1809 3.7210  0.2087 2.9568  0.2365 2.2723  0.2644 1.6298  0.2922 1.0953  0.3200 0.5640  0.3478 0.1203  0.3757 -0.2437  0.4035 -0.6445  0.4313 -0.9615  0.4591 -1.2848  0.4870 -1.6294  0.5148 -1.9996  0.5426 -2.2699  0.5704 -2.4700  0.5983 -2.6528  0.6261 -2.8509  0.6539 -3.1943  0.6817 -3.3356  0.7096 -3.4270  0.7374 -3.7276  0.7652 -3.7665  0.7931 -3.7910  0.8209 -3.9705  0.8487 -4.0870  0.8765 -4.1630  0.9044 -4.2589  0.9322 -4.3468  0.9600 -4.3623  0.9878 -4.4829  1.0157 -4.5509  1.0435 -4.5364  1.0713 -4.4814  1.0991 -4.5490  1.1270 -4.5358  1.1548 -4.4932  1.1826 -4.4059  1.2105 -4.1440  1.2383 -4.1665  1.2661 -4.2523  1.2939 -4.0445  1.3218 -3.9978  1.3496 -4.1378  1.3774 -3.9514  1.4052 -3.9979  1.4331 -3.8507  1.4609 -3.4913  1.4887 -3.4338  1.5165 -3.3890  1.5444 -3.2370  1.5722 -2.9748  1.6000 -2.7819  1.6278 -2.5677  1.6557 -2.6582  1.6835 -2.4193  1.7113 -2.1721  1.7392 -2.1034  1.7670 -1.9769  1.7948 -1.8652  1.8226 -1.6903  1.8505 -1.7705  1.8783 -1.5963  1.9061 -1.1326  1.9339 -1.1140  1.9618 -1.0281  1.9896 -0.5351  2.0174 -0.3780  2.0452 -0.5717  2.0731 -0.3831  2.1009 0.0637  2.1287 0.3183  2.1565 0.3191  2.1844 0.5016  2.2122 0.6547  2.2400 0.7331  2.2679 1.1166  2.2957 1.2276  2.3235 1.4689  2.3513 1.9310  2.3792 2.2035  2.4070 2.3413  2.4348 2.3736  2.4626 2.4416  2.4905 2.9089  2.5183 3.3991  2.5461 3.6686  2.5739 3.5246  2.6018 3.7237  2.6296 4.1352  2.6574 4.5535  2.6853 4.7846  2.7131 5.3397  2.7409 5.6685  2.7687 5.4986  2.7966 5.4102  2.8244 5.4254  2.8522 5.7117  2.8800 6.2622  2.9079 7.0046  2.9357 7.1374  2.9635 7.2985  2.9913 7.4988  3.0192 8.0125  3.0470 8.2611  3.0748 8.3106  3.1026 8.9057  3.1305 9.3350  3.1583 9.5276  3.1861 10.2713  3.2140 10.2856  3.2418 10.4702  3.2696 11.2846  3.2974 11.2877  3.3253 11.2776  3.3531 11.4499  3.3809 12.3267  3.4087 12.3139  3.4366 12.5261  3.4644 13.7803  3.4922 13.3054  3.5200 13.4374  3.5479 14.6589  3.5757 14.3574  3.6035 14.7769  3.6314 15.4497  3.6592 15.5749  3.6870 16.0960  3.7148 16.1733  3.7427 16.4527  3.7705 17.1939  3.7983 17.9401  3.8261 18.0740  3.8540 18.3401  3.8818 18.7650  3.9096 19.1299  3.9374 19.0907  3.9653 18.8246  3.9931 19.9459
    /

%L=14
\color{B14}
\multiput {\tiny{$\bullet$}} at
0.0861 7.3928  0.1107 6.0281  0.1353 5.0384  0.1599 4.1848  0.1844 3.3394  0.2090 2.7393  0.2336 2.1999  0.2582 1.5571  0.2828 1.0210  0.3074 0.5442  0.3320 0.1526  0.3566 -0.3030  0.3812 -0.6301  0.4058 -0.8741  0.4304 -1.3631  0.4550 -1.8535  0.4796 -1.9178  0.5042 -1.8905  0.5288 -2.1945  0.5533 -2.3256  0.5779 -2.7533  0.6025 -3.4048  0.6271 -3.3838  0.6517 -3.1205  0.6763 -3.3475  0.7009 -3.8778  0.7255 -3.7377  0.7501 -3.7503  0.7747 -4.0546  0.7993 -4.4755  0.8239 -4.9598  0.8485 -4.4757  0.8731 -4.2099  0.8977 -4.1472  0.9222 -4.2644  0.9468 -4.7123  0.9714 -4.1853  0.9960 -4.3927  1.0206 -4.7372  1.0452 -4.7772  1.0698 -4.8633  1.0944 -5.2686  1.1190 -5.1376  1.1436 -4.6998  1.1682 -4.6574  1.1928 -4.1041  1.2174 -3.7207  1.2420 -5.9301  1.2666 -5.6769  1.2911 -4.8123  1.3157 -5.1773  1.3403 -3.3371  1.3649 -4.1799  1.3895 -4.3118  1.4141 -2.9913  1.4387 -4.1025  1.4633 -5.3247  1.4879 -3.6251  1.5125 -2.5136  1.5371 -3.8602  1.5617 -3.8498  1.5863 -3.7080  1.6109 -2.3801  1.6355 -3.0665  1.6600 -3.5713  1.6846 -1.5081  1.7092 -0.8567  1.7338 -1.5182  1.7584 -0.6099  1.7830 0.2485  1.8076 -1.2098  1.8322 -1.7031  1.8568 -1.8431  1.8814 -1.1492  1.9060 -0.4678  1.9306 -1.7125  1.9552 -2.9141  1.9798 -0.0293  2.0044 -0.0148  2.0289 0.2197  2.0535 1.9275  2.0781 -0.9996  2.1027 -2.5887  2.1273 -0.9011  2.1519 -1.8843  2.1765 -0.3608  2.2011 0.5101  2.2257 0.1570  2.2503 1.7542  2.2749 1.2486  2.2995 0.2923  2.3241 2.1625  2.3487 3.0325  2.3733 1.0445  2.3978 1.2134  2.4224 -0.6950  2.4470 1.6038  2.4716 3.8362  2.4962 2.1824  2.5208 1.5993  2.5454 2.7166  2.5700 4.5072  2.5946 3.7018  2.6192 2.7149  2.6438 3.2624  2.6684 6.3976  2.6930 6.1057  2.7176 3.2351  2.7422 3.0787  2.7667 3.6035  2.7913 4.2683  2.8159 5.8859  2.8405 6.0966  2.8651 7.5389  2.8897 6.3534  2.9143 2.3722  2.9389 5.1094  2.9635 5.4689  2.9881 10.1408  3.0127 13.0305  3.0373 8.8088  3.0619 5.6379  3.0865 5.7096  3.1111 8.1504  3.1356 7.1069  3.1602 4.7983  3.1848 7.1175  3.2094 13.5974  3.2340 15.0804  3.2586 13.8373  3.2832 12.2580  3.3078 13.3295  3.3324 11.5026  3.3570 10.6798  3.3816 10.3093  3.4062 12.1216  3.4308 13.3675  3.4554 11.6658  3.4800 15.9241  3.5045 16.8238  3.5291 16.6959  3.5537 17.6762  3.5783 12.1422  3.6029 8.6453  3.6275 13.4197  3.6521 13.9210  3.6767 17.4188  3.7013 15.3497  3.7259 10.5487  3.7505 14.4342  3.7751 12.8584  3.7997 16.4415  3.8243 17.3789  3.8488 16.1637  3.8734 18.5682  3.8980 15.9514  3.9226 16.9725  3.9472 17.2687  3.9718 15.8586  3.9964 15.0293 
/


%L=15
\color{B15}
\multiput {\tiny{$\bullet$}} at
0.0767 7.7876  0.0986 6.4183  0.1206 5.4285  0.1425 4.5383  0.1644 3.7596  0.1863 3.0801  0.2083 2.4400  0.2302 1.8703  0.2521 1.3718  0.2740 0.9807  0.2959 0.5554  0.3179 0.1370  0.3398 -0.2677  0.3617 -0.6332  0.3836 -0.8867  0.4056 -1.0857  0.4275 -1.3740  0.4494 -1.7076  0.4713 -2.0793  0.4932 -2.2759  0.5152 -2.3519  0.5371 -2.6745  0.5590 -3.0156  0.5809 -3.2881  0.6029 -3.2720  0.6248 -3.6333  0.6467 -3.7633  0.6686 -3.4809  0.6905 -3.6995  0.7125 -3.7094  0.7344 -3.9047  0.7563 -4.1853  0.7782 -4.3558  0.8001 -4.4747  0.8221 -4.3886  0.8440 -4.1947  0.8659 -4.5348  0.8878 -4.5329  0.9098 -4.3460  0.9317 -4.7901  0.9536 -4.8461  0.9755 -5.0319  0.9974 -5.3478  1.0194 -4.8450  1.0413 -4.5283  1.0632 -4.8506  1.0851 -4.5082  1.1071 -4.8085  1.1290 -4.8548  1.1509 -4.5197  1.1728 -4.9413  1.1947 -4.8018  1.2167 -4.8222  1.2386 -4.7621  1.2605 -4.2399  1.2824 -4.5044  1.3044 -4.5934  1.3263 -4.6717  1.3482 -4.6865  1.3701 -4.0488  1.3920 -4.2254  1.4140 -4.4916  1.4359 -3.7149  1.4578 -3.2253  1.4797 -3.0388  1.5016 -2.9935  1.5236 -3.8150  1.5455 -3.3411  1.5674 -2.9545  1.5893 -2.9034  1.6113 -2.4253  1.6332 -3.2208  1.6551 -3.4818  1.6770 -2.9699  1.6989 -2.0555  1.7209 -2.0696  1.7428 -3.1972  1.7647 -2.7061  1.7866 -1.8753  1.8086 -2.2758  1.8305 -1.7507  1.8524 -1.3420  1.8743 -1.8635  1.8962 -1.1778  1.9182 -0.3858  1.9401 -0.5333  1.9620 -1.2057  1.9839 -1.5709  2.0059 -1.7969  2.0278 -1.2333  2.0497 -1.3804  2.0716 -1.0878  2.0935 -0.9994  2.1155 -2.2386  2.1374 -1.1524  2.1593 1.4465  2.1812 0.9221  2.2031 0.3452  2.2251 0.3937  2.2470 0.1814  2.2689 0.4873  2.2908 -0.2293  2.3128 0.5247  2.3347 1.6371  2.3566 3.3185  2.3785 2.6198  2.4004 1.9517  2.4224 2.8085  2.4443 2.7657  2.4662 2.9028  2.4881 0.9741  2.5101 1.2003  2.5320 3.5930  2.5539 3.9807  2.5758 3.7234  2.5977 2.1341  2.6197 1.7814  2.6416 3.5135  2.6635 4.8725  2.6854 4.5754  2.7074 5.3295  2.7293 6.6005  2.7512 5.4998  2.7731 5.2450  2.7950 3.5812  2.8170 4.6205  2.8389 6.2757  2.8608 4.9439  2.8827 5.9433  2.9046 6.8442  2.9266 6.4088  2.9485 7.5973  2.9704 5.8207  2.9923 6.2432  3.0143 8.3503  3.0362 6.1019  3.0581 6.1821  3.0800 6.3941  3.1019 7.6112  3.1239 7.8019  3.1458 7.4725  3.1677 10.2862  3.1896 10.5231  3.2116 9.5668  3.2335 9.3952  3.2554 11.4187  3.2773 9.8829  3.2992 6.1562  3.3212 7.4242  3.3431 11.7394  3.3650 13.1500  3.3869 11.1979  3.4089 12.9137  3.4308 15.1740  3.4527 13.2396  3.4746 13.2276  3.4965 16.9404  3.5185 14.0994  3.5404 14.2516  3.5623 14.9299  3.5842 14.4751  3.6062 15.5330  3.6281 13.2820  3.6500 15.3762  3.6719 16.7800  3.6938 15.1135  3.7158 16.0783  3.7377 16.7276  3.7596 15.7999  3.7815 16.9218  3.8034 17.6887  3.8254 19.3577  3.8473 18.4686  3.8692 17.2793  3.8911 19.3466  3.9131 20.2334  3.9350 19.7009  3.9569 19.4928  3.9788 20.4663     /





\color{black}
\normalcolor


\color{blue}

\normalcolor
\color{black}

\endpicture

==> Figures/figure18.tex <==


\beginpicture

\normalcolor
\color{black}
\setcoordinatesystem units <300pt,20pt>
\axes{0}{-0.5}{0}{0}{1}{8}{-0.25}
\axis left shiftedto x=0 label {\Large$\Pi_{4_1}$} 
      ticks
      withvalues 2 4 6  /
      at 2 4 6 /
 /  
\axis bottom shiftedto y=0 %label {$\phi$} 
    ticks
    withvalues 0.25 0.75 /
    at 0.25 0.75  /
/

\put {\Large$\phi$} at 0.6 -0.7


%L=4
\color{B04}
%\plot 0.5156 -1.2062  0.5469 -0.9693  0.5781 -0.7731  0.6094 -0.5966  0.6406 -0.4271  0.6719 -0.2577  0.7031 -0.0823  0.7344 0.1060  0.7656 0.3147  0.7969 0.5534  0.8281 0.8343  0.8594 1.1773  0.8906 1.6143  0.9219 2.2032 /
\multiput {\large$\cdot$} at 0.5156 -1.2062  0.5469 -0.9693  0.5781 -0.7731  0.6094 -0.5966  0.6406 -0.4271  0.6719 -0.2577  0.7031 -0.0823  0.7344 0.1060  0.7656 0.3147  0.7969 0.5534  0.8281 0.8343  0.8594 1.1773  0.8906 1.6143  0.9219 2.2032 /


%L=5
\color{B05}
%\plot 0.2640 -0.7494  0.2800 -0.6608  0.2960 -0.5913  0.3120 -0.5339  0.3280 -0.4836  0.3440 -0.4381  0.3600 -0.3957  0.3760 -0.3559  0.3920 -0.3178  0.4080 -0.2806  0.4240 -0.2439  0.4400 -0.2078  0.4560 -0.1721  0.4720 -0.1364  0.4880 -0.0997  0.5040 -0.0625  0.5200 -0.0248  0.5360 0.0138  0.5520 0.0542  0.5680 0.0964  0.5840 0.1403  0.6000 0.1859  0.6160 0.2334  0.6320 0.2836  0.6480 0.3373  0.6640 0.3946  0.6800 0.4551  0.6960 0.5202  0.7120 0.5898  0.7280 0.6639  0.7440 0.7448  0.7600 0.8333  0.7760 0.9289  0.7920 1.0337  0.8080 1.1490  0.8240 1.2764  0.8400 1.4191  0.8560 1.5797  0.8720 1.7629  0.8880 1.9752  0.9040 2.2243  0.9200 2.5251  0.9360 2.9024  0.9520 3.3972 /
\multiput {\large$\cdot$} at 0.2640 -0.7494  0.2800 -0.6608  0.2960 -0.5913  0.3120 -0.5339  0.3280 -0.4836  0.3440 -0.4381  0.3600 -0.3957  0.3760 -0.3559  0.3920 -0.3178  0.4080 -0.2806  0.4240 -0.2439  0.4400 -0.2078  0.4560 -0.1721  0.4720 -0.1364  0.4880 -0.0997  0.5040 -0.0625  0.5200 -0.0248  0.5360 0.0138  0.5520 0.0542  0.5680 0.0964  0.5840 0.1403  0.6000 0.1859  0.6160 0.2334  0.6320 0.2836  0.6480 0.3373  0.6640 0.3946  0.6800 0.4551  0.6960 0.5202  0.7120 0.5898  0.7280 0.6639  0.7440 0.7448  0.7600 0.8333  0.7760 0.9289  0.7920 1.0337  0.8080 1.1490  0.8240 1.2764  0.8400 1.4191  0.8560 1.5797  0.8720 1.7629  0.8880 1.9752  0.9040 2.2243  0.9200 2.5251  0.9360 2.9024  0.9520 3.3972 /


%L=6
\color{B06}
%\plot 0.1528 -0.4422  0.1620 -0.3973  0.1713 -0.3640  0.1806 -0.3377  0.1898 -0.3158  0.1991 -0.2968  0.2083 -0.2800  0.2176 -0.2644  0.2269 -0.2500  0.2361 -0.2361  0.2454 -0.2226  0.2546 -0.2097  0.2639 -0.1971  0.2731 -0.1848  0.2824 -0.1724  0.2917 -0.1602  0.3009 -0.1483  0.3102 -0.1360  0.3194 -0.1241  0.3287 -0.1121  0.3380 -0.1000  0.3472 -0.0880  0.3565 -0.0758  0.3657 -0.0635  0.3750 -0.0510  0.3843 -0.0387  0.3935 -0.0260  0.4028 -0.0130  0.4120 0.0003  0.4213 0.0141  0.4306 0.0280  0.4398 0.0418  0.4491 0.0561  0.4583 0.0713  0.4676 0.0863  0.4769 0.1013  0.4861 0.1173  0.4954 0.1338  0.5046 0.1507  0.5139 0.1680  0.5231 0.1859  0.5324 0.2044  0.5417 0.2231  0.5509 0.2429  0.5602 0.2626  0.5694 0.2835  0.5787 0.3061  0.5880 0.3284  0.5972 0.3518  0.6065 0.3762  0.6157 0.4014  0.6250 0.4274  0.6343 0.4543  0.6435 0.4827  0.6528 0.5125  0.6620 0.5431  0.6713 0.5747  0.6806 0.6082  0.6898 0.6428  0.6991 0.6796  0.7083 0.7173  0.7176 0.7570  0.7269 0.7985  0.7361 0.8420  0.7454 0.8887  0.7546 0.9372  0.7639 0.9878  0.7731 1.0414  0.7824 1.0977  0.7917 1.1572  0.8009 1.2213  0.8102 1.2883  0.8194 1.3593  0.8287 1.4354  0.8380 1.5178  0.8472 1.6058  0.8565 1.6998  0.8657 1.8016  0.8750 1.9118  0.8843 2.0315  0.8935 2.1636  0.9028 2.3085  0.9120 2.4700  0.9213 2.6520  0.9306 2.8572  0.9398 3.0961  0.9491 3.3750  0.9583 3.7165  0.9676 4.1475  0.9769 4.7271   /
\multiput {\large$\cdot$} at 0.1528 -0.4422  0.1620 -0.3973  0.1713 -0.3640  0.1806 -0.3377  0.1898 -0.3158  0.1991 -0.2968  0.2083 -0.2800  0.2176 -0.2644  0.2269 -0.2500  0.2361 -0.2361  0.2454 -0.2226  0.2546 -0.2097  0.2639 -0.1971  0.2731 -0.1848  0.2824 -0.1724  0.2917 -0.1602  0.3009 -0.1483  0.3102 -0.1360  0.3194 -0.1241  0.3287 -0.1121  0.3380 -0.1000  0.3472 -0.0880  0.3565 -0.0758  0.3657 -0.0635  0.3750 -0.0510  0.3843 -0.0387  0.3935 -0.0260  0.4028 -0.0130  0.4120 0.0003  0.4213 0.0141  0.4306 0.0280  0.4398 0.0418  0.4491 0.0561  0.4583 0.0713  0.4676 0.0863  0.4769 0.1013  0.4861 0.1173  0.4954 0.1338  0.5046 0.1507  0.5139 0.1680  0.5231 0.1859  0.5324 0.2044  0.5417 0.2231  0.5509 0.2429  0.5602 0.2626  0.5694 0.2835  0.5787 0.3061  0.5880 0.3284  0.5972 0.3518  0.6065 0.3762  0.6157 0.4014  0.6250 0.4274  0.6343 0.4543  0.6435 0.4827  0.6528 0.5125  0.6620 0.5431  0.6713 0.5747  0.6806 0.6082  0.6898 0.6428  0.6991 0.6796  0.7083 0.7173  0.7176 0.7570  0.7269 0.7985  0.7361 0.8420  0.7454 0.8887  0.7546 0.9372  0.7639 0.9878  0.7731 1.0414  0.7824 1.0977  0.7917 1.1572  0.8009 1.2213  0.8102 1.2883  0.8194 1.3593  0.8287 1.4354  0.8380 1.5178  0.8472 1.6058  0.8565 1.6998  0.8657 1.8016  0.8750 1.9118  0.8843 2.0315  0.8935 2.1636  0.9028 2.3085  0.9120 2.4700  0.9213 2.6520  0.9306 2.8572  0.9398 3.0961  0.9491 3.3750  0.9583 3.7165  0.9676 4.1475  0.9769 4.7271   /

%L=7
\color{B07}
%\plot 0.0962 -0.2777  0.1020 -0.2507  0.1079 -0.2314  0.1137 -0.2165  0.1195 -0.2041  0.1254 -0.1941  0.1312 -0.1855  0.1370 -0.1778  0.1429 -0.1710  0.1487 -0.1644  0.1545 -0.1583  0.1603 -0.1527  0.1662 -0.1471  0.1720 -0.1416  0.1778 -0.1362  0.1837 -0.1311  0.1895 -0.1257  0.1953 -0.1222  0.2012 -0.1176  0.2070 -0.1091  0.2128 -0.1043  0.2187 -0.1011  0.2245 -0.0958  0.2303 -0.0907  0.2362 -0.0859  0.2420 -0.0808  0.2478 -0.0756  0.2536 -0.0706  0.2595 -0.0658  0.2653 -0.0608  0.2711 -0.0555  0.2770 -0.0502  0.2828 -0.0451  0.2886 -0.0398  0.2945 -0.0344  0.3003 -0.0293  0.3061 -0.0237  0.3120 -0.0184  0.3178 -0.0128  0.3236 -0.0071  0.3294 -0.0017  0.3353 0.0037  0.3411 0.0097  0.3469 0.0158  0.3528 0.0217  0.3586 0.0281  0.3644 0.0344  0.3703 0.0406  0.3761 0.0470  0.3819 0.0532  0.3878 0.0595  0.3936 0.0664  0.3994 0.0735  0.4052 0.0800  0.4111 0.0869  0.4169 0.0947  0.4227 0.1019  0.4286 0.1093  0.4344 0.1169  0.4402 0.1251  0.4461 0.1328  0.4519 0.1405  0.4577 0.1493  0.4636 0.1578  0.4694 0.1661  0.4752 0.1747  0.4810 0.1839  0.4869 0.1934  0.4927 0.2028  0.4985 0.2124  0.5044 0.2222  0.5102 0.2320  0.5160 0.2423  0.5219 0.2532  0.5277 0.2641  0.5335 0.2751  0.5394 0.2860  0.5452 0.2974  0.5510 0.3095  0.5569 0.3215  0.5627 0.3334  0.5685 0.3461  0.5743 0.3597  0.5802 0.3738  0.5860 0.3875  0.5918 0.4008  0.5977 0.4142  0.6035 0.4289  0.6093 0.4445  0.6152 0.4596  0.6210 0.4757  0.6268 0.4924  0.6327 0.5094  0.6385 0.5261  0.6443 0.5434  0.6501 0.5612  0.6560 0.5799  0.6618 0.5996  0.6676 0.6186  0.6735 0.6381  0.6793 0.6591  0.6851 0.6803  0.6910 0.7021  0.6968 0.7243  0.7026 0.7467  0.7085 0.7709  0.7143 0.7951  0.7201 0.8202  0.7259 0.8468  0.7318 0.8741  0.7376 0.9017  0.7434 0.9304  0.7493 0.9602  0.7551 0.9905  0.7609 1.0219  0.7668 1.0545  0.7726 1.0885  0.7784 1.1228  0.7843 1.1589  0.7901 1.1967  0.7959 1.2358  0.8017 1.2759  0.8076 1.3178  0.8134 1.3616  0.8192 1.4061  0.8251 1.4530  0.8309 1.5020  0.8367 1.5544  0.8426 1.6092  0.8484 1.6645  0.8542 1.7152  0.8601 1.7798  0.8659 1.8438  0.8717 1.9105  0.8776 1.9852  0.8834 2.0604  0.8892 2.1441  0.8950 2.2290  0.9009 2.3255  0.9067 2.4226  0.9125 2.5210  0.9184 2.6298  0.9242 2.7592  0.9300 2.8926  0.9359 3.0318  0.9417 3.1928  0.9475 3.3765  0.9534 3.5754  0.9592 3.8022  0.9650 4.0794  0.9708 4.3862  0.9767 4.7767  0.9825 5.2945    /
\multiput {\large$\cdot$} at 0.0962 -0.2777  0.1020 -0.2507  0.1079 -0.2314  0.1137 -0.2165  0.1195 -0.2041  0.1254 -0.1941  0.1312 -0.1855  0.1370 -0.1778  0.1429 -0.1710  0.1487 -0.1644  0.1545 -0.1583  0.1603 -0.1527  0.1662 -0.1471  0.1720 -0.1416  0.1778 -0.1362  0.1837 -0.1311  0.1895 -0.1257  0.1953 -0.1222  0.2012 -0.1176  0.2070 -0.1091  0.2128 -0.1043  0.2187 -0.1011  0.2245 -0.0958  0.2303 -0.0907  0.2362 -0.0859  0.2420 -0.0808  0.2478 -0.0756  0.2536 -0.0706  0.2595 -0.0658  0.2653 -0.0608  0.2711 -0.0555  0.2770 -0.0502  0.2828 -0.0451  0.2886 -0.0398  0.2945 -0.0344  0.3003 -0.0293  0.3061 -0.0237  0.3120 -0.0184  0.3178 -0.0128  0.3236 -0.0071  0.3294 -0.0017  0.3353 0.0037  0.3411 0.0097  0.3469 0.0158  0.3528 0.0217  0.3586 0.0281  0.3644 0.0344  0.3703 0.0406  0.3761 0.0470  0.3819 0.0532  0.3878 0.0595  0.3936 0.0664  0.3994 0.0735  0.4052 0.0800  0.4111 0.0869  0.4169 0.0947  0.4227 0.1019  0.4286 0.1093  0.4344 0.1169  0.4402 0.1251  0.4461 0.1328  0.4519 0.1405  0.4577 0.1493  0.4636 0.1578  0.4694 0.1661  0.4752 0.1747  0.4810 0.1839  0.4869 0.1934  0.4927 0.2028  0.4985 0.2124  0.5044 0.2222  0.5102 0.2320  0.5160 0.2423  0.5219 0.2532  0.5277 0.2641  0.5335 0.2751  0.5394 0.2860  0.5452 0.2974  0.5510 0.3095  0.5569 0.3215  0.5627 0.3334  0.5685 0.3461  0.5743 0.3597  0.5802 0.3738  0.5860 0.3875  0.5918 0.4008  0.5977 0.4142  0.6035 0.4289  0.6093 0.4445  0.6152 0.4596  0.6210 0.4757  0.6268 0.4924  0.6327 0.5094  0.6385 0.5261  0.6443 0.5434  0.6501 0.5612  0.6560 0.5799  0.6618 0.5996  0.6676 0.6186  0.6735 0.6381  0.6793 0.6591  0.6851 0.6803  0.6910 0.7021  0.6968 0.7243  0.7026 0.7467  0.7085 0.7709  0.7143 0.7951  0.7201 0.8202  0.7259 0.8468  0.7318 0.8741  0.7376 0.9017  0.7434 0.9304  0.7493 0.9602  0.7551 0.9905  0.7609 1.0219  0.7668 1.0545  0.7726 1.0885  0.7784 1.1228  0.7843 1.1589  0.7901 1.1967  0.7959 1.2358  0.8017 1.2759  0.8076 1.3178  0.8134 1.3616  0.8192 1.4061  0.8251 1.4530  0.8309 1.5020  0.8367 1.5544  0.8426 1.6092  0.8484 1.6645  0.8542 1.7152  0.8601 1.7798  0.8659 1.8438  0.8717 1.9105  0.8776 1.9852  0.8834 2.0604  0.8892 2.1441  0.8950 2.2290  0.9009 2.3255  0.9067 2.4226  0.9125 2.5210  0.9184 2.6298  0.9242 2.7592  0.9300 2.8926  0.9359 3.0318  0.9417 3.1928  0.9475 3.3765  0.9534 3.5754  0.9592 3.8022  0.9650 4.0794  0.9708 4.3862  0.9767 4.7767  0.9825 5.2945    /

%L=8
\color{B08}
%\plot 0.0645 -0.1833  0.0684 -0.1665  0.0723 -0.1541  0.0762 -0.1446  0.0801 -0.1371  0.0840 -0.1313  0.0879 -0.1262  0.0918 -0.1221  0.0957 -0.1183  0.0996 -0.1132  0.1035 -0.1101  0.1074 -0.1076  0.1113 -0.1046  0.1152 -0.1024  0.1191 -0.1001  0.1230 -0.0968  0.1270 -0.0950  0.1309 -0.0926  0.1348 -0.0901  0.1387 -0.0880  0.1426 -0.0830  0.1465 -0.0826  0.1504 -0.0811  0.1543 -0.0754  0.1582 -0.0730  0.1621 -0.0719  0.1660 -0.0716  0.1699 -0.0703  0.1738 -0.0665  0.1777 -0.0631  0.1816 -0.0618  0.1855 -0.0594  0.1895 -0.0567  0.1934 -0.0558  0.1973 -0.0527  0.2012 -0.0469  0.2051 -0.0443  0.2090 -0.0458  0.2129 -0.0469  0.2168 -0.0406  0.2207 -0.0358  0.2246 -0.0373  0.2285 -0.0329  0.2324 -0.0285  0.2363 -0.0267  0.2402 -0.0211  0.2441 -0.0216  0.2480 -0.0174  0.2520 -0.0125  0.2559 -0.0148  0.2598 -0.0154  0.2637 -0.0059  0.2676 0.0010  0.2715 -0.0012  0.2754 -0.0000  0.2793 -0.0007  0.2832 0.0055  0.2871 0.0109  0.2910 0.0143  0.2949 0.0113  0.2988 0.0146  0.3027 0.0225  0.3066 0.0251  0.3105 0.0289  0.3145 0.0282  0.3184 0.0307  0.3223 0.0339  0.3262 0.0378  0.3301 0.0450  0.3340 0.0479  0.3379 0.0507  0.3418 0.0611  0.3457 0.0625  0.3496 0.0590  0.3535 0.0652  0.3574 0.0687  0.3613 0.0728  0.3652 0.0769  0.3691 0.0754  0.3730 0.0795  0.3770 0.0887  0.3809 0.0924  0.3848 0.0966  0.3887 0.1001  0.3926 0.1038  0.3965 0.1085  0.4004 0.1129  0.4043 0.1163  0.4082 0.1208  0.4121 0.1251  0.4160 0.1380  0.4199 0.1421  0.4238 0.1384  0.4277 0.1445  0.4316 0.1492  0.4355 0.1538  0.4395 0.1586  0.4434 0.1643  0.4473 0.1701  0.4512 0.1741  0.4551 0.1856  0.4590 0.1910  0.4629 0.1894  0.4668 0.1958  0.4707 0.2014  0.4746 0.2072  0.4785 0.2129  0.4824 0.2202  0.4863 0.2412  0.4902 0.2438  0.4941 0.2342  0.4980 0.2427  0.5020 0.2497  0.5059 0.2540  0.5098 0.2762  0.5137 0.2832  0.5176 0.2735  0.5215 0.2823  0.5254 0.2894  0.5293 0.2996  0.5332 0.3102  0.5371 0.3136  0.5410 0.3181  0.5449 0.3265  0.5488 0.3341  0.5527 0.3420  0.5566 0.3498  0.5605 0.3577  0.5645 0.3660  0.5684 0.3743  0.5723 0.3828  0.5762 0.3918  0.5801 0.4001  0.5840 0.4082  0.5879 0.4174  0.5918 0.4269  0.5957 0.4362  0.5996 0.4460  0.6035 0.4559  0.6074 0.4657  0.6113 0.4758  0.6152 0.4861  0.6191 0.4968  0.6230 0.5073  0.6270 0.5182  0.6309 0.5293  0.6348 0.5401  0.6387 0.5515  0.6426 0.5628  0.6465 0.5747  0.6504 0.5879  0.6543 0.6000  0.6582 0.6119  0.6621 0.6252  0.6660 0.6378  0.6699 0.6503  0.6738 0.6642  0.6777 0.6786  0.6816 0.6929  0.6855 0.7071  0.6895 0.7212  0.6934 0.7355  0.6973 0.7505  0.7012 0.7657  0.7051 0.7817  0.7090 0.7978  0.7129 0.8141  0.7168 0.8307  0.7207 0.8470  0.7246 0.8648  0.7285 0.8824  0.7324 0.9002  0.7363 0.9194  0.7402 0.9378  0.7441 0.9573  0.7480 0.9774  0.7520 0.9970  0.7559 1.0173  0.7598 1.0382  0.7637 1.0601  0.7676 1.0818  0.7715 1.1049  0.7754 1.1282  0.7793 1.1511  0.7832 1.1754  0.7871 1.2006  0.7910 1.2257  0.7949 1.2516  0.7988 1.2789  0.8027 1.3064  0.8066 1.3339  0.8105 1.3617  0.8145 1.3917  0.8184 1.4230  0.8223 1.4557  0.8262 1.4766  0.8301 1.5099  0.8340 1.5580  0.8379 1.5658  0.8418 1.6025  0.8457 1.6678  0.8496 1.6705  0.8535 1.7119  0.8574 1.7858  0.8613 1.8112  0.8652 1.8568  0.8691 1.8977  0.8730 1.9445  0.8770 2.0003  0.8809 2.0452  0.8848 2.1061  0.8887 2.1589  0.8926 2.2183  0.8965 2.2876  0.9004 2.3384  0.9043 2.4004  0.9082 2.4688  0.9121 2.5322  0.9160 2.6199  0.9199 2.7020  0.9238 2.7804  0.9277 2.8541  0.9316 2.9437  0.9355 3.0472  0.9395 3.1604  0.9434 3.2754  0.9473 3.3812  0.9512 3.5196  0.9551 3.6681  0.9590 3.8133  0.9629 3.9717  0.9668 4.1864  0.9707 4.3919  0.9746 4.6298  0.9785 4.9432  0.9824 5.3030  0.9863 5.7773  0.9902 6.3186     /
\multiput {\large$\cdot$} at 0.0645 -0.1833  0.0684 -0.1665  0.0723 -0.1541  0.0762 -0.1446  0.0801 -0.1371  0.0840 -0.1313  0.0879 -0.1262  0.0918 -0.1221  0.0957 -0.1183  0.0996 -0.1132  0.1035 -0.1101  0.1074 -0.1076  0.1113 -0.1046  0.1152 -0.1024  0.1191 -0.1001  0.1230 -0.0968  0.1270 -0.0950  0.1309 -0.0926  0.1348 -0.0901  0.1387 -0.0880  0.1426 -0.0830  0.1465 -0.0826  0.1504 -0.0811  0.1543 -0.0754  0.1582 -0.0730  0.1621 -0.0719  0.1660 -0.0716  0.1699 -0.0703  0.1738 -0.0665  0.1777 -0.0631  0.1816 -0.0618  0.1855 -0.0594  0.1895 -0.0567  0.1934 -0.0558  0.1973 -0.0527  0.2012 -0.0469  0.2051 -0.0443  0.2090 -0.0458  0.2129 -0.0469  0.2168 -0.0406  0.2207 -0.0358  0.2246 -0.0373  0.2285 -0.0329  0.2324 -0.0285  0.2363 -0.0267  0.2402 -0.0211  0.2441 -0.0216  0.2480 -0.0174  0.2520 -0.0125  0.2559 -0.0148  0.2598 -0.0154  0.2637 -0.0059  0.2676 0.0010  0.2715 -0.0012  0.2754 -0.0000  0.2793 -0.0007  0.2832 0.0055  0.2871 0.0109  0.2910 0.0143  0.2949 0.0113  0.2988 0.0146  0.3027 0.0225  0.3066 0.0251  0.3105 0.0289  0.3145 0.0282  0.3184 0.0307  0.3223 0.0339  0.3262 0.0378  0.3301 0.0450  0.3340 0.0479  0.3379 0.0507  0.3418 0.0611  0.3457 0.0625  0.3496 0.0590  0.3535 0.0652  0.3574 0.0687  0.3613 0.0728  0.3652 0.0769  0.3691 0.0754  0.3730 0.0795  0.3770 0.0887  0.3809 0.0924  0.3848 0.0966  0.3887 0.1001  0.3926 0.1038  0.3965 0.1085  0.4004 0.1129  0.4043 0.1163  0.4082 0.1208  0.4121 0.1251  0.4160 0.1380  0.4199 0.1421  0.4238 0.1384  0.4277 0.1445  0.4316 0.1492  0.4355 0.1538  0.4395 0.1586  0.4434 0.1643  0.4473 0.1701  0.4512 0.1741  0.4551 0.1856  0.4590 0.1910  0.4629 0.1894  0.4668 0.1958  0.4707 0.2014  0.4746 0.2072  0.4785 0.2129  0.4824 0.2202  0.4863 0.2412  0.4902 0.2438  0.4941 0.2342  0.4980 0.2427  0.5020 0.2497  0.5059 0.2540  0.5098 0.2762  0.5137 0.2832  0.5176 0.2735  0.5215 0.2823  0.5254 0.2894  0.5293 0.2996  0.5332 0.3102  0.5371 0.3136  0.5410 0.3181  0.5449 0.3265  0.5488 0.3341  0.5527 0.3420  0.5566 0.3498  0.5605 0.3577  0.5645 0.3660  0.5684 0.3743  0.5723 0.3828  0.5762 0.3918  0.5801 0.4001  0.5840 0.4082  0.5879 0.4174  0.5918 0.4269  0.5957 0.4362  0.5996 0.4460  0.6035 0.4559  0.6074 0.4657  0.6113 0.4758  0.6152 0.4861  0.6191 0.4968  0.6230 0.5073  0.6270 0.5182  0.6309 0.5293  0.6348 0.5401  0.6387 0.5515  0.6426 0.5628  0.6465 0.5747  0.6504 0.5879  0.6543 0.6000  0.6582 0.6119  0.6621 0.6252  0.6660 0.6378  0.6699 0.6503  0.6738 0.6642  0.6777 0.6786  0.6816 0.6929  0.6855 0.7071  0.6895 0.7212  0.6934 0.7355  0.6973 0.7505  0.7012 0.7657  0.7051 0.7817  0.7090 0.7978  0.7129 0.8141  0.7168 0.8307  0.7207 0.8470  0.7246 0.8648  0.7285 0.8824  0.7324 0.9002  0.7363 0.9194  0.7402 0.9378  0.7441 0.9573  0.7480 0.9774  0.7520 0.9970  0.7559 1.0173  0.7598 1.0382  0.7637 1.0601  0.7676 1.0818  0.7715 1.1049  0.7754 1.1282  0.7793 1.1511  0.7832 1.1754  0.7871 1.2006  0.7910 1.2257  0.7949 1.2516  0.7988 1.2789  0.8027 1.3064  0.8066 1.3339  0.8105 1.3617  0.8145 1.3917  0.8184 1.4230  0.8223 1.4557  0.8262 1.4766  0.8301 1.5099  0.8340 1.5580  0.8379 1.5658  0.8418 1.6025  0.8457 1.6678  0.8496 1.6705  0.8535 1.7119  0.8574 1.7858  0.8613 1.8112  0.8652 1.8568  0.8691 1.8977  0.8730 1.9445  0.8770 2.0003  0.8809 2.0452  0.8848 2.1061  0.8887 2.1589  0.8926 2.2183  0.8965 2.2876  0.9004 2.3384  0.9043 2.4004  0.9082 2.4688  0.9121 2.5322  0.9160 2.6199  0.9199 2.7020  0.9238 2.7804  0.9277 2.8541  0.9316 2.9437  0.9355 3.0472  0.9395 3.1604  0.9434 3.2754  0.9473 3.3812  0.9512 3.5196  0.9551 3.6681  0.9590 3.8133  0.9629 3.9717  0.9668 4.1864  0.9707 4.3919  0.9746 4.6298  0.9785 4.9432  0.9824 5.3030  0.9863 5.7773  0.9902 6.3186    /


%L=9
\color{B09}
%\plot 0.0453 -0.1266  0.0480 -0.1152  0.0508 -0.1069  0.0535 -0.1007  0.0562 -0.0957  0.0590 -0.0917  0.0617 -0.0884  0.0645 -0.0855  0.0672 -0.0830  0.0700 -0.0809  0.0727 -0.0793  0.0754 -0.0773  0.0782 -0.0749  0.0809 -0.0733  0.0837 -0.0720  0.0864 -0.0703  0.0892 -0.0700  0.0919 -0.0692  0.0947 -0.0672  0.0974 -0.0664  0.1001 -0.0643  0.1029 -0.0629  0.1056 -0.0620  0.1084 -0.0610  0.1111 -0.0587  0.1139 -0.0571  0.1166 -0.0566  0.1193 -0.0552  0.1221 -0.0538  0.1248 -0.0530  0.1276 -0.0533  0.1303 -0.0503  0.1331 -0.0492  0.1358 -0.0503  0.1385 -0.0483  0.1413 -0.0459  0.1440 -0.0460  0.1468 -0.0437  0.1495 -0.0417  0.1523 -0.0435  0.1550 -0.0401  0.1578 -0.0355  0.1605 -0.0355  0.1632 -0.0356  0.1660 -0.0345  0.1687 -0.0365  0.1715 -0.0325  0.1742 -0.0287  0.1770 -0.0285  0.1797 -0.0265  0.1824 -0.0269  0.1852 -0.0267  0.1879 -0.0251  0.1907 -0.0213  0.1934 -0.0221  0.1962 -0.0210  0.1989 -0.0186  0.2016 -0.0192  0.2044 -0.0150  0.2071 -0.0161  0.2099 -0.0161  0.2126 -0.0108  0.2154 -0.0115  0.2181 -0.0088  0.2209 -0.0062  0.2236 -0.0018  0.2263 -0.0039  0.2291 -0.0064  0.2318 -0.0018  0.2346 0.0008  0.2373 0.0033  0.2401 0.0024  0.2428 0.0039  0.2455 0.0068  0.2483 0.0075  0.2510 0.0060  0.2538 0.0151  0.2565 0.0201  0.2593 0.0149  0.2620 0.0197  0.2647 0.0184  0.2675 0.0203  0.2702 0.0230  0.2730 0.0184  0.2757 0.0253  0.2785 0.0306  0.2812 0.0320  0.2840 0.0347  0.2867 0.0380  0.2894 0.0324  0.2922 0.0293  0.2949 0.0353  0.2977 0.0424  0.3004 0.0418  0.3032 0.0391  0.3059 0.0419  0.3086 0.0414  0.3114 0.0430  0.3141 0.0612  0.3169 0.0690  0.3196 0.0402  0.3224 0.0528  0.3251 0.0667  0.3278 0.0681  0.3306 0.0672  0.3333 0.0710  0.3361 0.0699  0.3388 0.0620  0.3416 0.0762  0.3443 0.0662  0.3471 0.0616  0.3498 0.0973  0.3525 0.0955  0.3553 0.0599  0.3580 0.0815  0.3608 0.1055  0.3635 0.0985  0.3663 0.1005  0.3690 0.1005  0.3717 0.0868  0.3745 0.0971  0.3772 0.1077  0.3800 0.1005  0.3827 0.1038  0.3855 0.1245  0.3882 0.1264  0.3909 0.1174  0.3937 0.1207  0.3964 0.1275  0.3992 0.1301  0.4019 0.1326  0.4047 0.1358  0.4074 0.1382  0.4102 0.1413  0.4129 0.1451  0.4156 0.1482  0.4184 0.1504  0.4211 0.1567  0.4239 0.1600  0.4266 0.1630  0.4294 0.1670  0.4321 0.1669  0.4348 0.1698  0.4376 0.1769  0.4403 0.1808  0.4431 0.1809  0.4458 0.1845  0.4486 0.1875  0.4513 0.1904  0.4540 0.2016  0.4568 0.2054  0.4595 0.2012  0.4623 0.2090  0.4650 0.2161  0.4678 0.2160  0.4705 0.2169  0.4733 0.2210  0.4760 0.2245  0.4787 0.2320  0.4815 0.2360  0.4842 0.2360  0.4870 0.2477  0.4897 0.2523  0.4925 0.2489  0.4952 0.2539  0.4979 0.2582  0.5007 0.2649  0.5034 0.2687  0.5062 0.2744  0.5089 0.2863  0.5117 0.2861  0.5144 0.2846  0.5171 0.2899  0.5199 0.2977  0.5226 0.3022  0.5254 0.3031  0.5281 0.3158  0.5309 0.3206  0.5336 0.3182  0.5364 0.3237  0.5391 0.3321  0.5418 0.3411  0.5446 0.3487  0.5473 0.3505  0.5501 0.3499  0.5528 0.3554  0.5556 0.3643  0.5583 0.3723  0.5610 0.3781  0.5638 0.3814  0.5665 0.3843  0.5693 0.3894  0.5720 0.4007  0.5748 0.4144  0.5775 0.4141  0.5802 0.4139  0.5830 0.4202  0.5857 0.4320  0.5885 0.4447  0.5912 0.4453  0.5940 0.4461  0.5967 0.4518  0.5995 0.4710  0.6022 0.4772  0.6049 0.4715  0.6077 0.4794  0.6104 0.4954  0.6132 0.5012  0.6159 0.5001  0.6187 0.5088  0.6214 0.5256  0.6241 0.5324  0.6269 0.5290  0.6296 0.5398  0.6324 0.5485  0.6351 0.5550  0.6379 0.5622  0.6406 0.5704  0.6433 0.5785  0.6461 0.5864  0.6488 0.5948  0.6516 0.6024  0.6543 0.6115  0.6571 0.6211  0.6598 0.6304  0.6626 0.6396  0.6653 0.6480  0.6680 0.6577  0.6708 0.6678  0.6735 0.6766  0.6763 0.6848  0.6790 0.6943  0.6818 0.7052  0.6845 0.7151  0.6872 0.7254  0.6900 0.7356  0.6927 0.7461  0.6955 0.7562  0.6982 0.7660  0.7010 0.7779  0.7037 0.7886  0.7064 0.7993  0.7092 0.8106  0.7119 0.8220  0.7147 0.8340  0.7174 0.8461  0.7202 0.8591  0.7229 0.8710  0.7257 0.8822  0.7284 0.8951  0.7311 0.9076  0.7339 0.9202  0.7366 0.9328  0.7394 0.9453  0.7421 0.9593  0.7449 0.9740  0.7476 0.9883  0.7503 1.0017  0.7531 1.0153  0.7558 1.0304  0.7586 1.0463  0.7613 1.0601  0.7641 1.0750  0.7668 1.0904  0.7695 1.1059  0.7723 1.1228  0.7750 1.1386  0.7778 1.1552  0.7805 1.1719  0.7833 1.1880  0.7860 1.2060  0.7888 1.2242  0.7915 1.2420  0.7942 1.2601  0.7970 1.2790  0.7997 1.2977  0.8025 1.3158  0.8052 1.3363  0.8080 1.3575  0.8107 1.3795  0.8134 1.3861  0.8162 1.4064  0.8189 1.4443  0.8217 1.4516  0.8244 1.4726  0.8272 1.5111  0.8299 1.5158  0.8326 1.5402  0.8354 1.5848  0.8381 1.5879  0.8409 1.6117  0.8436 1.6580  0.8464 1.6624  0.8491 1.6900  0.8519 1.7391  0.8546 1.7503  0.8573 1.7802  0.8601 1.8266  0.8628 1.8324  0.8656 1.8653  0.8683 1.9095  0.8711 1.9359  0.8738 1.9606  0.8765 1.9951  0.8793 2.0377  0.8820 2.0724  0.8848 2.1008  0.8875 2.1401  0.8903 2.1873  0.8930 2.2268  0.8957 2.2578  0.8985 2.2972  0.9012 2.3481  0.9040 2.4004  0.9067 2.4543  0.9095 2.4913  0.9122 2.5717  0.9150 2.6208  0.9177 2.6656  0.9204 2.7292  0.9232 2.7651  0.9259 2.8259  0.9287 2.8870  0.9314 2.9636  0.9342 3.0364  0.9369 3.0972  0.9396 3.1766  0.9424 3.2622  0.9451 3.3565  0.9479 3.4140  0.9506 3.4864  0.9534 3.6090  0.9561 3.7052  0.9588 3.8003  0.9616 3.8993  0.9643 4.0636  0.9671 4.2724  0.9698 4.3778  0.9726 4.4896  0.9753 4.6857  0.9781 4.9369  0.9808 5.1508  0.9835 5.3931  0.9863 5.7872  0.9890 6.1295  0.9918 6.4196   /
\multiput {\large$\cdot$} at 0.0453 -0.1266  0.0480 -0.1152  0.0508 -0.1069  0.0535 -0.1007  0.0562 -0.0957  0.0590 -0.0917  0.0617 -0.0884  0.0645 -0.0855  0.0672 -0.0830  0.0700 -0.0809  0.0727 -0.0793  0.0754 -0.0773  0.0782 -0.0749  0.0809 -0.0733  0.0837 -0.0720  0.0864 -0.0703  0.0892 -0.0700  0.0919 -0.0692  0.0947 -0.0672  0.0974 -0.0664  0.1001 -0.0643  0.1029 -0.0629  0.1056 -0.0620  0.1084 -0.0610  0.1111 -0.0587  0.1139 -0.0571  0.1166 -0.0566  0.1193 -0.0552  0.1221 -0.0538  0.1248 -0.0530  0.1276 -0.0533  0.1303 -0.0503  0.1331 -0.0492  0.1358 -0.0503  0.1385 -0.0483  0.1413 -0.0459  0.1440 -0.0460  0.1468 -0.0437  0.1495 -0.0417  0.1523 -0.0435  0.1550 -0.0401  0.1578 -0.0355  0.1605 -0.0355  0.1632 -0.0356  0.1660 -0.0345  0.1687 -0.0365  0.1715 -0.0325  0.1742 -0.0287  0.1770 -0.0285  0.1797 -0.0265  0.1824 -0.0269  0.1852 -0.0267  0.1879 -0.0251  0.1907 -0.0213  0.1934 -0.0221  0.1962 -0.0210  0.1989 -0.0186  0.2016 -0.0192  0.2044 -0.0150  0.2071 -0.0161  0.2099 -0.0161  0.2126 -0.0108  0.2154 -0.0115  0.2181 -0.0088  0.2209 -0.0062  0.2236 -0.0018  0.2263 -0.0039  0.2291 -0.0064  0.2318 -0.0018  0.2346 0.0008  0.2373 0.0033  0.2401 0.0024  0.2428 0.0039  0.2455 0.0068  0.2483 0.0075  0.2510 0.0060  0.2538 0.0151  0.2565 0.0201  0.2593 0.0149  0.2620 0.0197  0.2647 0.0184  0.2675 0.0203  0.2702 0.0230  0.2730 0.0184  0.2757 0.0253  0.2785 0.0306  0.2812 0.0320  0.2840 0.0347  0.2867 0.0380  0.2894 0.0324  0.2922 0.0293  0.2949 0.0353  0.2977 0.0424  0.3004 0.0418  0.3032 0.0391  0.3059 0.0419  0.3086 0.0414  0.3114 0.0430  0.3141 0.0612  0.3169 0.0690  0.3196 0.0402  0.3224 0.0528  0.3251 0.0667  0.3278 0.0681  0.3306 0.0672  0.3333 0.0710  0.3361 0.0699  0.3388 0.0620  0.3416 0.0762  0.3443 0.0662  0.3471 0.0616  0.3498 0.0973  0.3525 0.0955  0.3553 0.0599  0.3580 0.0815  0.3608 0.1055  0.3635 0.0985  0.3663 0.1005  0.3690 0.1005  0.3717 0.0868  0.3745 0.0971  0.3772 0.1077  0.3800 0.1005  0.3827 0.1038  0.3855 0.1245  0.3882 0.1264  0.3909 0.1174  0.3937 0.1207  0.3964 0.1275  0.3992 0.1301  0.4019 0.1326  0.4047 0.1358  0.4074 0.1382  0.4102 0.1413  0.4129 0.1451  0.4156 0.1482  0.4184 0.1504  0.4211 0.1567  0.4239 0.1600  0.4266 0.1630  0.4294 0.1670  0.4321 0.1669  0.4348 0.1698  0.4376 0.1769  0.4403 0.1808  0.4431 0.1809  0.4458 0.1845  0.4486 0.1875  0.4513 0.1904  0.4540 0.2016  0.4568 0.2054  0.4595 0.2012  0.4623 0.2090  0.4650 0.2161  0.4678 0.2160  0.4705 0.2169  0.4733 0.2210  0.4760 0.2245  0.4787 0.2320  0.4815 0.2360  0.4842 0.2360  0.4870 0.2477  0.4897 0.2523  0.4925 0.2489  0.4952 0.2539  0.4979 0.2582  0.5007 0.2649  0.5034 0.2687  0.5062 0.2744  0.5089 0.2863  0.5117 0.2861  0.5144 0.2846  0.5171 0.2899  0.5199 0.2977  0.5226 0.3022  0.5254 0.3031  0.5281 0.3158  0.5309 0.3206  0.5336 0.3182  0.5364 0.3237  0.5391 0.3321  0.5418 0.3411  0.5446 0.3487  0.5473 0.3505  0.5501 0.3499  0.5528 0.3554  0.5556 0.3643  0.5583 0.3723  0.5610 0.3781  0.5638 0.3814  0.5665 0.3843  0.5693 0.3894  0.5720 0.4007  0.5748 0.4144  0.5775 0.4141  0.5802 0.4139  0.5830 0.4202  0.5857 0.4320  0.5885 0.4447  0.5912 0.4453  0.5940 0.4461  0.5967 0.4518  0.5995 0.4710  0.6022 0.4772  0.6049 0.4715  0.6077 0.4794  0.6104 0.4954  0.6132 0.5012  0.6159 0.5001  0.6187 0.5088  0.6214 0.5256  0.6241 0.5324  0.6269 0.5290  0.6296 0.5398  0.6324 0.5485  0.6351 0.5550  0.6379 0.5622  0.6406 0.5704  0.6433 0.5785  0.6461 0.5864  0.6488 0.5948  0.6516 0.6024  0.6543 0.6115  0.6571 0.6211  0.6598 0.6304  0.6626 0.6396  0.6653 0.6480  0.6680 0.6577  0.6708 0.6678  0.6735 0.6766  0.6763 0.6848  0.6790 0.6943  0.6818 0.7052  0.6845 0.7151  0.6872 0.7254  0.6900 0.7356  0.6927 0.7461  0.6955 0.7562  0.6982 0.7660  0.7010 0.7779  0.7037 0.7886  0.7064 0.7993  0.7092 0.8106  0.7119 0.8220  0.7147 0.8340  0.7174 0.8461  0.7202 0.8591  0.7229 0.8710  0.7257 0.8822  0.7284 0.8951  0.7311 0.9076  0.7339 0.9202  0.7366 0.9328  0.7394 0.9453  0.7421 0.9593  0.7449 0.9740  0.7476 0.9883  0.7503 1.0017  0.7531 1.0153  0.7558 1.0304  0.7586 1.0463  0.7613 1.0601  0.7641 1.0750  0.7668 1.0904  0.7695 1.1059  0.7723 1.1228  0.7750 1.1386  0.7778 1.1552  0.7805 1.1719  0.7833 1.1880  0.7860 1.2060  0.7888 1.2242  0.7915 1.2420  0.7942 1.2601  0.7970 1.2790  0.7997 1.2977  0.8025 1.3158  0.8052 1.3363  0.8080 1.3575  0.8107 1.3795  0.8134 1.3861  0.8162 1.4064  0.8189 1.4443  0.8217 1.4516  0.8244 1.4726  0.8272 1.5111  0.8299 1.5158  0.8326 1.5402  0.8354 1.5848  0.8381 1.5879  0.8409 1.6117  0.8436 1.6580  0.8464 1.6624  0.8491 1.6900  0.8519 1.7391  0.8546 1.7503  0.8573 1.7802  0.8601 1.8266  0.8628 1.8324  0.8656 1.8653  0.8683 1.9095  0.8711 1.9359  0.8738 1.9606  0.8765 1.9951  0.8793 2.0377  0.8820 2.0724  0.8848 2.1008  0.8875 2.1401  0.8903 2.1873  0.8930 2.2268  0.8957 2.2578  0.8985 2.2972  0.9012 2.3481  0.9040 2.4004  0.9067 2.4543  0.9095 2.4913  0.9122 2.5717  0.9150 2.6208  0.9177 2.6656  0.9204 2.7292  0.9232 2.7651  0.9259 2.8259  0.9287 2.8870  0.9314 2.9636  0.9342 3.0364  0.9369 3.0972  0.9396 3.1766  0.9424 3.2622  0.9451 3.3565  0.9479 3.4140  0.9506 3.4864  0.9534 3.6090  0.9561 3.7052  0.9588 3.8003  0.9616 3.8993  0.9643 4.0636  0.9671 4.2724  0.9698 4.3778  0.9726 4.4896  0.9753 4.6857  0.9781 4.9369  0.9808 5.1508  0.9835 5.3931  0.9863 5.7872  0.9890 6.1295  0.9918 6.4196    /


%L=10
\color{B10}
%\plot 0.0330 -0.0913  0.0350 -0.0833  0.0370 -0.0776  0.0390 -0.0730  0.0410 -0.0694  0.0430 -0.0666  0.0450 -0.0643  0.0470 -0.0619  0.0490 -0.0604  0.0510 -0.0589  0.0530 -0.0575  0.0550 -0.0563  0.0570 -0.0549  0.0590 -0.0538  0.0610 -0.0530  0.0630 -0.0525  0.0650 -0.0515  0.0670 -0.0504  0.0690 -0.0494  0.0710 -0.0487  0.0730 -0.0488  0.0750 -0.0481  0.0770 -0.0470  0.0790 -0.0462  0.0810 -0.0458  0.0830 -0.0445  0.0850 -0.0437  0.0870 -0.0438  0.0890 -0.0426  0.0910 -0.0419  0.0930 -0.0419  0.0950 -0.0409  0.0970 -0.0403  0.0990 -0.0395  0.1010 -0.0383  0.1030 -0.0381  0.1050 -0.0379  0.1070 -0.0365  0.1090 -0.0370  0.1110 -0.0363  0.1130 -0.0335  0.1150 -0.0330  0.1170 -0.0332  0.1190 -0.0339  0.1210 -0.0329  0.1230 -0.0323  0.1250 -0.0322  0.1270 -0.0307  0.1290 -0.0300  0.1310 -0.0286  0.1330 -0.0268  0.1350 -0.0269  0.1370 -0.0267  0.1390 -0.0250  0.1410 -0.0238  0.1430 -0.0247  0.1450 -0.0228  0.1470 -0.0228  0.1490 -0.0215  0.1510 -0.0207  0.1530 -0.0211  0.1550 -0.0183  0.1570 -0.0182  0.1590 -0.0170  0.1610 -0.0159  0.1630 -0.0152  0.1650 -0.0157  0.1670 -0.0131  0.1690 -0.0144  0.1710 -0.0136  0.1730 -0.0098  0.1750 -0.0129  0.1770 -0.0104  0.1790 -0.0088  0.1810 -0.0102  0.1830 -0.0079  0.1850 -0.0076  0.1870 -0.0076  0.1890 -0.0067  0.1910 -0.0045  0.1930 -0.0021  0.1950 -0.0024  0.1970 -0.0033  0.1990 -0.0039  0.2010 0.0003  0.2030 0.0036  0.2050 0.0020  0.2070 -0.0002  0.2090 0.0044  0.2110 0.0034  0.2130 0.0048  0.2150 0.0081  0.2170 0.0055  0.2190 0.0081  0.2210 0.0078  0.2230 0.0090  0.2250 0.0116  0.2270 0.0119  0.2290 0.0142  0.2310 0.0136  0.2330 0.0131  0.2350 0.0110  0.2370 0.0123  0.2390 0.0205  0.2410 0.0250  0.2430 0.0253  0.2450 0.0191  0.2470 0.0165  0.2490 0.0205  0.2510 0.0275  0.2530 0.0296  0.2550 0.0236  0.2570 0.0252  0.2590 0.0367  0.2610 0.0338  0.2630 0.0289  0.2650 0.0290  0.2670 0.0329  0.2690 0.0370  0.2710 0.0379  0.2730 0.0389  0.2750 0.0398  0.2770 0.0405  0.2790 0.0399  0.2810 0.0405  0.2830 0.0437  0.2850 0.0464  0.2870 0.0469  0.2890 0.0490  0.2910 0.0509  0.2930 0.0525  0.2950 0.0538  0.2970 0.0521  0.2990 0.0509  0.3010 0.0575  0.3030 0.0564  0.3050 0.0566  0.3070 0.0643  0.3090 0.0612  0.3110 0.0570  0.3130 0.0637  0.3150 0.0679  0.3170 0.0611  0.3190 0.0626  0.3210 0.0732  0.3230 0.0719  0.3250 0.0714  0.3270 0.0795  0.3290 0.0832  0.3310 0.0779  0.3330 0.0801  0.3350 0.0827  0.3370 0.0801  0.3390 0.0917  0.3410 0.0882  0.3430 0.0759  0.3450 0.0807  0.3470 0.0892  0.3490 0.0921  0.3510 0.0882  0.3530 0.0890  0.3550 0.0992  0.3570 0.1018  0.3590 0.1003  0.3610 0.0990  0.3630 0.1053  0.3650 0.1093  0.3670 0.1062  0.3690 0.1020  0.3710 0.1078  0.3730 0.1214  0.3750 0.1067  0.3770 0.1081  0.3790 0.1172  0.3810 0.1167  0.3830 0.1209  0.3850 0.1197  0.3870 0.1284  0.3890 0.1317  0.3910 0.1240  0.3930 0.1266  0.3950 0.1199  0.3970 0.1262  0.3990 0.1398  0.4010 0.1281  0.4030 0.1416  0.4050 0.1421  0.4070 0.1180  0.4090 0.1334  0.4110 0.1427  0.4130 0.1420  0.4150 0.1588  0.4170 0.1614  0.4190 0.1645  0.4210 0.1938  0.4230 0.1917  0.4250 0.1690  0.4270 0.1746  0.4290 0.1590  0.4310 0.1456  0.4330 0.1728  0.4350 0.1924  0.4370 0.1775  0.4390 0.1766  0.4410 0.1726  0.4430 0.1763  0.4450 0.1951  0.4470 0.1954  0.4490 0.1970  0.4510 0.2006  0.4530 0.2030  0.4550 0.2050  0.4570 0.2083  0.4590 0.2103  0.4610 0.2166  0.4630 0.2198  0.4650 0.2179  0.4670 0.2287  0.4690 0.2348  0.4710 0.2291  0.4730 0.2299  0.4750 0.2327  0.4770 0.2352  0.4790 0.2379  0.4810 0.2403  0.4830 0.2477  0.4850 0.2498  0.4870 0.2481  0.4890 0.2608  0.4910 0.2666  0.4930 0.2616  0.4950 0.2628  0.4970 0.2662  0.4990 0.2699  0.5010 0.2757  0.5030 0.2780  0.5050 0.2821  0.5070 0.2886  0.5090 0.2903  0.5110 0.2910  0.5130 0.2926  0.5150 0.2954  0.5170 0.3020  0.5190 0.3051  0.5210 0.3043  0.5230 0.3129  0.5250 0.3227  0.5270 0.3211  0.5290 0.3184  0.5310 0.3230  0.5330 0.3309  0.5350 0.3343  0.5370 0.3372  0.5390 0.3434  0.5410 0.3467  0.5430 0.3480  0.5450 0.3486  0.5470 0.3555  0.5490 0.3594  0.5510 0.3638  0.5530 0.3735  0.5550 0.3746  0.5570 0.3734  0.5590 0.3801  0.5610 0.3831  0.5630 0.3830  0.5650 0.3983  0.5670 0.4030  0.5690 0.3976  0.5710 0.4030  0.5730 0.4106  0.5750 0.4129  0.5770 0.4239  0.5790 0.4289  0.5810 0.4232  0.5830 0.4291  0.5850 0.4357  0.5870 0.4429  0.5890 0.4513  0.5910 0.4528  0.5930 0.4512  0.5950 0.4569  0.5970 0.4648  0.5990 0.4756  0.6010 0.4775  0.6030 0.4766  0.6050 0.4820  0.6070 0.4899  0.6090 0.5020  0.6110 0.5027  0.6130 0.5010  0.6150 0.5069  0.6170 0.5142  0.6190 0.5312  0.6210 0.5329  0.6230 0.5265  0.6250 0.5324  0.6270 0.5480  0.6290 0.5530  0.6310 0.5484  0.6330 0.5563  0.6350 0.5696  0.6370 0.5776  0.6390 0.5766  0.6410 0.5790  0.6430 0.5957  0.6450 0.6040  0.6470 0.5989  0.6490 0.6022  0.6510 0.6174  0.6530 0.6277  0.6550 0.6255  0.6570 0.6288  0.6590 0.6472  0.6610 0.6531  0.6630 0.6452  0.6650 0.6658  0.6670 0.6730  0.6690 0.6655  0.6710 0.6869  0.6730 0.6939  0.6750 0.6869  0.6770 0.7017  0.6790 0.7086  0.6810 0.7097  0.6830 0.7179  0.6850 0.7246  0.6870 0.7318  0.6890 0.7389  0.6910 0.7466  0.6930 0.7554  0.6950 0.7621  0.6970 0.7699  0.6990 0.7801  0.7010 0.7871  0.7030 0.7932  0.7050 0.8029  0.7070 0.8115  0.7090 0.8198  0.7110 0.8280  0.7130 0.8351  0.7150 0.8434  0.7170 0.8515  0.7190 0.8616  0.7210 0.8714  0.7230 0.8790  0.7250 0.8872  0.7270 0.8968  0.7290 0.9067  0.7310 0.9169  0.7330 0.9251  0.7350 0.9343  0.7370 0.9448  0.7390 0.9541  0.7410 0.9636  0.7430 0.9729  0.7450 0.9829  0.7470 0.9927  0.7490 1.0030  0.7510 1.0134  0.7530 1.0238  0.7550 1.0332  0.7570 1.0430  0.7590 1.0548  0.7610 1.0676  0.7630 1.0802  0.7650 1.0914  0.7670 1.1010  0.7690 1.1112  0.7710 1.1235  0.7730 1.1354  0.7750 1.1479  0.7770 1.1593  0.7790 1.1712  0.7810 1.1841  0.7830 1.1963  0.7850 1.2099  0.7870 1.2222  0.7890 1.2338  0.7910 1.2464  0.7930 1.2604  0.7950 1.2754  0.7970 1.2890  0.7990 1.3023  0.8010 1.3159  0.8030 1.3297  0.8050 1.3449  0.8070 1.3596  0.8090 1.3666  0.8110 1.3822  0.8130 1.4067  0.8150 1.4072  0.8170 1.4221  0.8190 1.4532  0.8210 1.4523  0.8230 1.4693  0.8250 1.5031  0.8270 1.5020  0.8290 1.5206  0.8310 1.5558  0.8330 1.5535  0.8350 1.5712  0.8370 1.6086  0.8390 1.6060  0.8410 1.6232  0.8430 1.6606  0.8450 1.6643  0.8470 1.6852  0.8490 1.7195  0.8510 1.7252  0.8530 1.7460  0.8550 1.7815  0.8570 1.7799  0.8590 1.8024  0.8610 1.8420  0.8630 1.8513  0.8650 1.8732  0.8670 1.9035  0.8690 1.9218  0.8710 1.9468  0.8730 1.9660  0.8750 1.9899  0.8770 2.0134  0.8790 2.0408  0.8810 2.0656  0.8830 2.0915  0.8850 2.1182  0.8870 2.1434  0.8890 2.1779  0.8910 2.2090  0.8930 2.2330  0.8950 2.2603  0.8970 2.2885  0.8990 2.3222  0.9010 2.3528  0.9030 2.3854  0.9050 2.4174  0.9070 2.4542  0.9090 2.4839  0.9110 2.5103  0.9130 2.5826  0.9150 2.6195  0.9170 2.6396  0.9190 2.6839  0.9210 2.7282  0.9230 2.7699  0.9250 2.8188  0.9270 2.8695  0.9290 2.8889  0.9310 2.9976  0.9330 3.0649  0.9350 3.0427  0.9370 3.0913  0.9390 3.1179  0.9410 3.2605  0.9430 3.3304  0.9450 3.3022  0.9470 3.4477  0.9490 3.5193  0.9510 3.5098  0.9530 3.5990  0.9550 3.7116  0.9570 3.7618  0.9590 3.8294  0.9610 3.9172  0.9630 4.0326  0.9650 4.1315  0.9670 4.1615  0.9690 4.3273  0.9710 4.5006  0.9730 4.5509  0.9750 4.6346  0.9770 4.7708  0.9790 4.9423  0.9810 5.2163  0.9830 5.5711  0.9850 5.6284  0.9870 5.7760  0.9890 6.0722  0.9910 6.3452  0.9930 6.8933  0.9950 7.1225     /
\multiput {\large$\cdot$} at 0.0330 -0.0913  0.0350 -0.0833  0.0370 -0.0776  0.0390 -0.0730  0.0410 -0.0694  0.0430 -0.0666  0.0450 -0.0643  0.0470 -0.0619  0.0490 -0.0604  0.0510 -0.0589  0.0530 -0.0575  0.0550 -0.0563  0.0570 -0.0549  0.0590 -0.0538  0.0610 -0.0530  0.0630 -0.0525  0.0650 -0.0515  0.0670 -0.0504  0.0690 -0.0494  0.0710 -0.0487  0.0730 -0.0488  0.0750 -0.0481  0.0770 -0.0470  0.0790 -0.0462  0.0810 -0.0458  0.0830 -0.0445  0.0850 -0.0437  0.0870 -0.0438  0.0890 -0.0426  0.0910 -0.0419  0.0930 -0.0419  0.0950 -0.0409  0.0970 -0.0403  0.0990 -0.0395  0.1010 -0.0383  0.1030 -0.0381  0.1050 -0.0379  0.1070 -0.0365  0.1090 -0.0370  0.1110 -0.0363  0.1130 -0.0335  0.1150 -0.0330  0.1170 -0.0332  0.1190 -0.0339  0.1210 -0.0329  0.1230 -0.0323  0.1250 -0.0322  0.1270 -0.0307  0.1290 -0.0300  0.1310 -0.0286  0.1330 -0.0268  0.1350 -0.0269  0.1370 -0.0267  0.1390 -0.0250  0.1410 -0.0238  0.1430 -0.0247  0.1450 -0.0228  0.1470 -0.0228  0.1490 -0.0215  0.1510 -0.0207  0.1530 -0.0211  0.1550 -0.0183  0.1570 -0.0182  0.1590 -0.0170  0.1610 -0.0159  0.1630 -0.0152  0.1650 -0.0157  0.1670 -0.0131  0.1690 -0.0144  0.1710 -0.0136  0.1730 -0.0098  0.1750 -0.0129  0.1770 -0.0104  0.1790 -0.0088  0.1810 -0.0102  0.1830 -0.0079  0.1850 -0.0076  0.1870 -0.0076  0.1890 -0.0067  0.1910 -0.0045  0.1930 -0.0021  0.1950 -0.0024  0.1970 -0.0033  0.1990 -0.0039  0.2010 0.0003  0.2030 0.0036  0.2050 0.0020  0.2070 -0.0002  0.2090 0.0044  0.2110 0.0034  0.2130 0.0048  0.2150 0.0081  0.2170 0.0055  0.2190 0.0081  0.2210 0.0078  0.2230 0.0090  0.2250 0.0116  0.2270 0.0119  0.2290 0.0142  0.2310 0.0136  0.2330 0.0131  0.2350 0.0110  0.2370 0.0123  0.2390 0.0205  0.2410 0.0250  0.2430 0.0253  0.2450 0.0191  0.2470 0.0165  0.2490 0.0205  0.2510 0.0275  0.2530 0.0296  0.2550 0.0236  0.2570 0.0252  0.2590 0.0367  0.2610 0.0338  0.2630 0.0289  0.2650 0.0290  0.2670 0.0329  0.2690 0.0370  0.2710 0.0379  0.2730 0.0389  0.2750 0.0398  0.2770 0.0405  0.2790 0.0399  0.2810 0.0405  0.2830 0.0437  0.2850 0.0464  0.2870 0.0469  0.2890 0.0490  0.2910 0.0509  0.2930 0.0525  0.2950 0.0538  0.2970 0.0521  0.2990 0.0509  0.3010 0.0575  0.3030 0.0564  0.3050 0.0566  0.3070 0.0643  0.3090 0.0612  0.3110 0.0570  0.3130 0.0637  0.3150 0.0679  0.3170 0.0611  0.3190 0.0626  0.3210 0.0732  0.3230 0.0719  0.3250 0.0714  0.3270 0.0795  0.3290 0.0832  0.3310 0.0779  0.3330 0.0801  0.3350 0.0827  0.3370 0.0801  0.3390 0.0917  0.3410 0.0882  0.3430 0.0759  0.3450 0.0807  0.3470 0.0892  0.3490 0.0921  0.3510 0.0882  0.3530 0.0890  0.3550 0.0992  0.3570 0.1018  0.3590 0.1003  0.3610 0.0990  0.3630 0.1053  0.3650 0.1093  0.3670 0.1062  0.3690 0.1020  0.3710 0.1078  0.3730 0.1214  0.3750 0.1067  0.3770 0.1081  0.3790 0.1172  0.3810 0.1167  0.3830 0.1209  0.3850 0.1197  0.3870 0.1284  0.3890 0.1317  0.3910 0.1240  0.3930 0.1266  0.3950 0.1199  0.3970 0.1262  0.3990 0.1398  0.4010 0.1281  0.4030 0.1416  0.4050 0.1421  0.4070 0.1180  0.4090 0.1334  0.4110 0.1427  0.4130 0.1420  0.4150 0.1588  0.4170 0.1614  0.4190 0.1645  0.4210 0.1938  0.4230 0.1917  0.4250 0.1690  0.4270 0.1746  0.4290 0.1590  0.4310 0.1456  0.4330 0.1728  0.4350 0.1924  0.4370 0.1775  0.4390 0.1766  0.4410 0.1726  0.4430 0.1763  0.4450 0.1951  0.4470 0.1954  0.4490 0.1970  0.4510 0.2006  0.4530 0.2030  0.4550 0.2050  0.4570 0.2083  0.4590 0.2103  0.4610 0.2166  0.4630 0.2198  0.4650 0.2179  0.4670 0.2287  0.4690 0.2348  0.4710 0.2291  0.4730 0.2299  0.4750 0.2327  0.4770 0.2352  0.4790 0.2379  0.4810 0.2403  0.4830 0.2477  0.4850 0.2498  0.4870 0.2481  0.4890 0.2608  0.4910 0.2666  0.4930 0.2616  0.4950 0.2628  0.4970 0.2662  0.4990 0.2699  0.5010 0.2757  0.5030 0.2780  0.5050 0.2821  0.5070 0.2886  0.5090 0.2903  0.5110 0.2910  0.5130 0.2926  0.5150 0.2954  0.5170 0.3020  0.5190 0.3051  0.5210 0.3043  0.5230 0.3129  0.5250 0.3227  0.5270 0.3211  0.5290 0.3184  0.5310 0.3230  0.5330 0.3309  0.5350 0.3343  0.5370 0.3372  0.5390 0.3434  0.5410 0.3467  0.5430 0.3480  0.5450 0.3486  0.5470 0.3555  0.5490 0.3594  0.5510 0.3638  0.5530 0.3735  0.5550 0.3746  0.5570 0.3734  0.5590 0.3801  0.5610 0.3831  0.5630 0.3830  0.5650 0.3983  0.5670 0.4030  0.5690 0.3976  0.5710 0.4030  0.5730 0.4106  0.5750 0.4129  0.5770 0.4239  0.5790 0.4289  0.5810 0.4232  0.5830 0.4291  0.5850 0.4357  0.5870 0.4429  0.5890 0.4513  0.5910 0.4528  0.5930 0.4512  0.5950 0.4569  0.5970 0.4648  0.5990 0.4756  0.6010 0.4775  0.6030 0.4766  0.6050 0.4820  0.6070 0.4899  0.6090 0.5020  0.6110 0.5027  0.6130 0.5010  0.6150 0.5069  0.6170 0.5142  0.6190 0.5312  0.6210 0.5329  0.6230 0.5265  0.6250 0.5324  0.6270 0.5480  0.6290 0.5530  0.6310 0.5484  0.6330 0.5563  0.6350 0.5696  0.6370 0.5776  0.6390 0.5766  0.6410 0.5790  0.6430 0.5957  0.6450 0.6040  0.6470 0.5989  0.6490 0.6022  0.6510 0.6174  0.6530 0.6277  0.6550 0.6255  0.6570 0.6288  0.6590 0.6472  0.6610 0.6531  0.6630 0.6452  0.6650 0.6658  0.6670 0.6730  0.6690 0.6655  0.6710 0.6869  0.6730 0.6939  0.6750 0.6869  0.6770 0.7017  0.6790 0.7086  0.6810 0.7097  0.6830 0.7179  0.6850 0.7246  0.6870 0.7318  0.6890 0.7389  0.6910 0.7466  0.6930 0.7554  0.6950 0.7621  0.6970 0.7699  0.6990 0.7801  0.7010 0.7871  0.7030 0.7932  0.7050 0.8029  0.7070 0.8115  0.7090 0.8198  0.7110 0.8280  0.7130 0.8351  0.7150 0.8434  0.7170 0.8515  0.7190 0.8616  0.7210 0.8714  0.7230 0.8790  0.7250 0.8872  0.7270 0.8968  0.7290 0.9067  0.7310 0.9169  0.7330 0.9251  0.7350 0.9343  0.7370 0.9448  0.7390 0.9541  0.7410 0.9636  0.7430 0.9729  0.7450 0.9829  0.7470 0.9927  0.7490 1.0030  0.7510 1.0134  0.7530 1.0238  0.7550 1.0332  0.7570 1.0430  0.7590 1.0548  0.7610 1.0676  0.7630 1.0802  0.7650 1.0914  0.7670 1.1010  0.7690 1.1112  0.7710 1.1235  0.7730 1.1354  0.7750 1.1479  0.7770 1.1593  0.7790 1.1712  0.7810 1.1841  0.7830 1.1963  0.7850 1.2099  0.7870 1.2222  0.7890 1.2338  0.7910 1.2464  0.7930 1.2604  0.7950 1.2754  0.7970 1.2890  0.7990 1.3023  0.8010 1.3159  0.8030 1.3297  0.8050 1.3449  0.8070 1.3596  0.8090 1.3666  0.8110 1.3822  0.8130 1.4067  0.8150 1.4072  0.8170 1.4221  0.8190 1.4532  0.8210 1.4523  0.8230 1.4693  0.8250 1.5031  0.8270 1.5020  0.8290 1.5206  0.8310 1.5558  0.8330 1.5535  0.8350 1.5712  0.8370 1.6086  0.8390 1.6060  0.8410 1.6232  0.8430 1.6606  0.8450 1.6643  0.8470 1.6852  0.8490 1.7195  0.8510 1.7252  0.8530 1.7460  0.8550 1.7815  0.8570 1.7799  0.8590 1.8024  0.8610 1.8420  0.8630 1.8513  0.8650 1.8732  0.8670 1.9035  0.8690 1.9218  0.8710 1.9468  0.8730 1.9660  0.8750 1.9899  0.8770 2.0134  0.8790 2.0408  0.8810 2.0656  0.8830 2.0915  0.8850 2.1182  0.8870 2.1434  0.8890 2.1779  0.8910 2.2090  0.8930 2.2330  0.8950 2.2603  0.8970 2.2885  0.8990 2.3222  0.9010 2.3528  0.9030 2.3854  0.9050 2.4174  0.9070 2.4542  0.9090 2.4839  0.9110 2.5103  0.9130 2.5826  0.9150 2.6195  0.9170 2.6396  0.9190 2.6839  0.9210 2.7282  0.9230 2.7699  0.9250 2.8188  0.9270 2.8695  0.9290 2.8889  0.9310 2.9976  0.9330 3.0649  0.9350 3.0427  0.9370 3.0913  0.9390 3.1179  0.9410 3.2605  0.9430 3.3304  0.9450 3.3022  0.9470 3.4477  0.9490 3.5193  0.9510 3.5098  0.9530 3.5990  0.9550 3.7116  0.9570 3.7618  0.9590 3.8294  0.9610 3.9172  0.9630 4.0326  0.9650 4.1315  0.9670 4.1615  0.9690 4.3273  0.9710 4.5006  0.9730 4.5509  0.9750 4.6346  0.9770 4.7708  0.9790 4.9423  0.9810 5.2163  0.9830 5.5711  0.9850 5.6284  0.9870 5.7760  0.9890 6.0722  0.9910 6.3452  0.9930 6.8933  0.9950 7.1225      /



%L=11
\color{B11}
%\plot 0.0248 -0.0684  0.0263 -0.0619  0.0278 -0.0576  0.0293 -0.0544  0.0308 -0.0516  0.0323 -0.0497  0.0338 -0.0479  0.0353 -0.0462  0.0368 -0.0447  0.0383 -0.0437  0.0398 -0.0428  0.0413 -0.0418  0.0428 -0.0415  0.0443 -0.0409  0.0458 -0.0399  0.0473 -0.0390  0.0488 -0.0386  0.0503 -0.0379  0.0518 -0.0374  0.0533 -0.0376  0.0548 -0.0372  0.0563 -0.0363  0.0579 -0.0363  0.0594 -0.0358  0.0609 -0.0354  0.0624 -0.0350  0.0639 -0.0335  0.0654 -0.0339  0.0669 -0.0335  0.0684 -0.0323  0.0699 -0.0332  0.0714 -0.0329  0.0729 -0.0323  0.0744 -0.0317  0.0759 -0.0308  0.0774 -0.0311  0.0789 -0.0310  0.0804 -0.0291  0.0819 -0.0290  0.0834 -0.0303  0.0849 -0.0289  0.0864 -0.0278  0.0879 -0.0283  0.0894 -0.0279  0.0909 -0.0264  0.0924 -0.0254  0.0939 -0.0256  0.0954 -0.0253  0.0969 -0.0252  0.0984 -0.0248  0.0999 -0.0253  0.1014 -0.0246  0.1029 -0.0235  0.1044 -0.0237  0.1059 -0.0226  0.1074 -0.0229  0.1089 -0.0233  0.1104 -0.0223  0.1119 -0.0213  0.1134 -0.0210  0.1150 -0.0208  0.1165 -0.0202  0.1180 -0.0190  0.1195 -0.0197  0.1210 -0.0194  0.1225 -0.0178  0.1240 -0.0174  0.1255 -0.0161  0.1270 -0.0172  0.1285 -0.0154  0.1300 -0.0136  0.1315 -0.0151  0.1330 -0.0152  0.1345 -0.0137  0.1360 -0.0128  0.1375 -0.0149  0.1390 -0.0139  0.1405 -0.0127  0.1420 -0.0124  0.1435 -0.0109  0.1450 -0.0099  0.1465 -0.0106  0.1480 -0.0104  0.1495 -0.0090  0.1510 -0.0097  0.1525 -0.0074  0.1540 -0.0076  0.1555 -0.0080  0.1570 -0.0067  0.1585 -0.0081  0.1600 -0.0053  0.1615 -0.0044  0.1630 -0.0056  0.1645 -0.0044  0.1660 -0.0018  0.1675 -0.0030  0.1690 -0.0044  0.1705 0.0001  0.1721 0.0011  0.1736 -0.0012  0.1751 -0.0004  0.1766 0.0012  0.1781 0.0002  0.1796 0.0014  0.1811 0.0023  0.1826 0.0029  0.1841 0.0058  0.1856 0.0053  0.1871 0.0034  0.1886 0.0045  0.1901 0.0040  0.1916 0.0046  0.1931 0.0058  0.1946 0.0073  0.1961 0.0091  0.1976 0.0091  0.1991 0.0088  0.2006 0.0118  0.2021 0.0105  0.2036 0.0078  0.2051 0.0153  0.2066 0.0148  0.2081 0.0126  0.2096 0.0139  0.2111 0.0145  0.2126 0.0124  0.2141 0.0143  0.2156 0.0205  0.2171 0.0170  0.2186 0.0160  0.2201 0.0187  0.2216 0.0186  0.2231 0.0221  0.2246 0.0223  0.2261 0.0211  0.2276 0.0239  0.2292 0.0242  0.2307 0.0236  0.2322 0.0232  0.2337 0.0225  0.2352 0.0236  0.2367 0.0271  0.2382 0.0291  0.2397 0.0288  0.2412 0.0309  0.2427 0.0302  0.2442 0.0275  0.2457 0.0303  0.2472 0.0305  0.2487 0.0337  0.2502 0.0350  0.2517 0.0332  0.2532 0.0382  0.2547 0.0350  0.2562 0.0352  0.2577 0.0398  0.2592 0.0399  0.2607 0.0357  0.2622 0.0344  0.2637 0.0409  0.2652 0.0445  0.2667 0.0438  0.2682 0.0398  0.2697 0.0435  0.2712 0.0481  0.2727 0.0418  0.2742 0.0416  0.2757 0.0423  0.2772 0.0463  0.2787 0.0465  0.2802 0.0407  0.2817 0.0494  0.2832 0.0556  0.2847 0.0553  0.2863 0.0527  0.2878 0.0530  0.2893 0.0580  0.2908 0.0568  0.2923 0.0597  0.2938 0.0579  0.2953 0.0604  0.2968 0.0656  0.2983 0.0615  0.2998 0.0596  0.3013 0.0673  0.3028 0.0685  0.3043 0.0623  0.3058 0.0660  0.3073 0.0621  0.3088 0.0697  0.3103 0.0714  0.3118 0.0649  0.3133 0.0701  0.3148 0.0731  0.3163 0.0788  0.3178 0.0747  0.3193 0.0712  0.3208 0.0846  0.3223 0.0798  0.3238 0.0718  0.3253 0.0826  0.3268 0.0813  0.3283 0.0804  0.3298 0.0857  0.3313 0.0913  0.3328 0.0864  0.3343 0.0816  0.3358 0.0871  0.3373 0.0846  0.3388 0.0904  0.3403 0.0948  0.3418 0.0871  0.3434 0.0921  0.3449 0.1014  0.3464 0.0965  0.3479 0.0965  0.3494 0.0963  0.3509 0.0923  0.3524 0.1069  0.3539 0.1104  0.3554 0.0913  0.3569 0.0977  0.3584 0.1007  0.3599 0.1052  0.3614 0.1153  0.3629 0.1180  0.3644 0.1136  0.3659 0.1128  0.3674 0.1161  0.3689 0.1151  0.3704 0.1208  0.3719 0.1182  0.3734 0.1210  0.3749 0.1177  0.3764 0.1213  0.3779 0.1272  0.3794 0.1278  0.3809 0.1217  0.3824 0.1217  0.3839 0.1327  0.3854 0.1370  0.3869 0.1350  0.3884 0.1321  0.3899 0.1344  0.3914 0.1357  0.3929 0.1338  0.3944 0.1391  0.3959 0.1353  0.3974 0.1382  0.3989 0.1540  0.4005 0.1461  0.4020 0.1447  0.4035 0.1499  0.4050 0.1475  0.4065 0.1511  0.4080 0.1514  0.4095 0.1419  0.4110 0.1501  0.4125 0.1698  0.4140 0.1563  0.4155 0.1533  0.4170 0.1671  0.4185 0.1562  0.4200 0.1596  0.4215 0.1680  0.4230 0.1707  0.4245 0.1697  0.4260 0.1749  0.4275 0.1862  0.4290 0.1683  0.4305 0.1638  0.4320 0.1773  0.4335 0.1729  0.4350 0.1623  0.4365 0.1618  0.4380 0.1916  0.4395 0.1800  0.4410 0.1838  0.4425 0.1861  0.4440 0.1703  0.4455 0.1975  0.4470 0.2005  0.4485 0.1890  0.4500 0.1939  0.4515 0.2248  0.4530 0.2293  0.4545 0.2089  0.4560 0.1556  0.4576 0.1669  0.4591 0.2585  0.4606 0.2588  0.4621 0.2206  0.4636 0.2199  0.4651 0.2287  0.4666 0.2292  0.4681 0.2168  0.4696 0.1934  0.4711 0.1740  0.4726 0.2194  0.4741 0.2044  0.4756 0.2013  0.4771 0.2470  0.4786 0.2430  0.4801 0.2486  0.4816 0.2614  0.4831 0.2503  0.4846 0.2421  0.4861 0.2596  0.4876 0.2610  0.4891 0.2629  0.4906 0.2597  0.4921 0.2622  0.4936 0.2658  0.4951 0.2687  0.4966 0.2709  0.4981 0.2728  0.4996 0.2745  0.5011 0.2776  0.5026 0.2802  0.5041 0.2898  0.5056 0.2951  0.5071 0.2942  0.5086 0.2948  0.5101 0.2924  0.5116 0.2954  0.5131 0.2976  0.5147 0.2996  0.5162 0.3024  0.5177 0.3030  0.5192 0.3183  0.5207 0.3206  0.5222 0.3154  0.5237 0.3196  0.5252 0.3177  0.5267 0.3196  0.5282 0.3222  0.5297 0.3260  0.5312 0.3314  0.5327 0.3362  0.5342 0.3412  0.5357 0.3449  0.5372 0.3425  0.5387 0.3433  0.5402 0.3470  0.5417 0.3486  0.5432 0.3548  0.5447 0.3604  0.5462 0.3591  0.5477 0.3633  0.5492 0.3697  0.5507 0.3687  0.5522 0.3690  0.5537 0.3717  0.5552 0.3734  0.5567 0.3843  0.5582 0.3869  0.5597 0.3895  0.5612 0.3924  0.5627 0.3874  0.5642 0.3934  0.5657 0.3985  0.5672 0.4000  0.5687 0.4078  0.5702 0.4186  0.5718 0.4153  0.5733 0.4117  0.5748 0.4164  0.5763 0.4192  0.5778 0.4253  0.5793 0.4317  0.5808 0.4389  0.5823 0.4387  0.5838 0.4344  0.5853 0.4394  0.5868 0.4433  0.5883 0.4501  0.5898 0.4553  0.5913 0.4627  0.5928 0.4629  0.5943 0.4583  0.5958 0.4625  0.5973 0.4702  0.5988 0.4767  0.6003 0.4840  0.6018 0.4868  0.6033 0.4840  0.6048 0.4873  0.6063 0.4915  0.6078 0.5031  0.6093 0.5084  0.6108 0.5041  0.6123 0.5052  0.6138 0.5111  0.6153 0.5165  0.6168 0.5256  0.6183 0.5271  0.6198 0.5254  0.6213 0.5297  0.6228 0.5390  0.6243 0.5493  0.6258 0.5464  0.6273 0.5453  0.6289 0.5487  0.6304 0.5576  0.6319 0.5694  0.6334 0.5676  0.6349 0.5663  0.6364 0.5722  0.6379 0.5817  0.6394 0.5921  0.6409 0.5907  0.6424 0.5881  0.6439 0.5924  0.6454 0.6018  0.6469 0.6129  0.6484 0.6119  0.6499 0.6096  0.6514 0.6204  0.6529 0.6323  0.6544 0.6311  0.6559 0.6292  0.6574 0.6397  0.6589 0.6505  0.6604 0.6510  0.6619 0.6488  0.6634 0.6605  0.6649 0.6694  0.6664 0.6665  0.6679 0.6683  0.6694 0.6801  0.6709 0.6930  0.6724 0.6913  0.6739 0.6872  0.6754 0.6986  0.6769 0.7129  0.6784 0.7125  0.6799 0.7110  0.6814 0.7216  0.6829 0.7305  0.6844 0.7315  0.6860 0.7320  0.6875 0.7500  0.6890 0.7563  0.6905 0.7484  0.6920 0.7627  0.6935 0.7679  0.6950 0.7644  0.6965 0.7856  0.6980 0.7910  0.6995 0.7820  0.7010 0.8009  0.7025 0.8073  0.7040 0.8006  0.7055 0.8197  0.7070 0.8276  0.7085 0.8208  0.7100 0.8359  0.7115 0.8417  0.7130 0.8373  0.7145 0.8525  0.7160 0.8596  0.7175 0.8579  0.7190 0.8648  0.7205 0.8724  0.7220 0.8784  0.7235 0.8860  0.7250 0.8921  0.7265 0.8982  0.7280 0.9050  0.7295 0.9120  0.7310 0.9207  0.7325 0.9265  0.7340 0.9346  0.7355 0.9428  0.7370 0.9499  0.7385 0.9575  0.7400 0.9636  0.7415 0.9691  0.7431 0.9793  0.7446 0.9874  0.7461 0.9936  0.7476 0.9995  0.7491 1.0060  0.7506 1.0169  0.7521 1.0260  0.7536 1.0327  0.7551 1.0385  0.7566 1.0481  0.7581 1.0543  0.7596 1.0608  0.7611 1.0742  0.7626 1.0815  0.7641 1.0881  0.7656 1.0969  0.7671 1.1054  0.7686 1.1151  0.7701 1.1217  0.7716 1.1303  0.7731 1.1422  0.7746 1.1513  0.7761 1.1611  0.7776 1.1697  0.7791 1.1776  0.7806 1.1884  0.7821 1.1976  0.7836 1.2046  0.7851 1.2155  0.7866 1.2259  0.7881 1.2347  0.7896 1.2439  0.7911 1.2556  0.7926 1.2654  0.7941 1.2727  0.7956 1.2824  0.7971 1.2933  0.7986 1.3050  0.8002 1.3157  0.8017 1.3263  0.8032 1.3360  0.8047 1.3467  0.8062 1.3582  0.8077 1.3679  0.8092 1.3797  0.8107 1.3829  0.8122 1.3930  0.8137 1.4160  0.8152 1.4139  0.8167 1.4256  0.8182 1.4545  0.8197 1.4453  0.8212 1.4588  0.8227 1.4929  0.8242 1.4842  0.8257 1.4965  0.8272 1.5296  0.8287 1.5240  0.8302 1.5324  0.8317 1.5623  0.8332 1.5642  0.8347 1.5790  0.8362 1.6070  0.8377 1.6014  0.8392 1.6154  0.8407 1.6488  0.8422 1.6482  0.8437 1.6608  0.8452 1.6895  0.8467 1.6870  0.8482 1.7017  0.8497 1.7379  0.8512 1.7322  0.8527 1.7446  0.8542 1.7803  0.8557 1.7808  0.8573 1.7939  0.8588 1.8285  0.8603 1.8289  0.8618 1.8432  0.8633 1.8692  0.8648 1.8787  0.8663 1.8974  0.8678 1.9123  0.8693 1.9282  0.8708 1.9467  0.8723 1.9661  0.8738 1.9836  0.8753 1.9999  0.8768 2.0260  0.8783 2.0336  0.8798 2.0586  0.8813 2.0781  0.8828 2.0972  0.8843 2.1185  0.8858 2.1365  0.8873 2.1609  0.8888 2.1821  0.8903 2.1983  0.8918 2.2271  0.8933 2.2490  0.8948 2.2691  0.8963 2.2903  0.8978 2.3129  0.8993 2.3365  0.9008 2.3531  0.9023 2.3769  0.9038 2.4106  0.9053 2.4309  0.9068 2.4637  0.9083 2.4890  0.9098 2.5042  0.9113 2.5409  0.9128 2.5734  0.9144 2.5942  0.9159 2.6118  0.9174 2.6527  0.9189 2.6676  0.9204 2.7031  0.9219 2.7527  0.9234 2.7706  0.9249 2.7916  0.9264 2.8302  0.9279 2.8488  0.9294 3.0076  0.9309 3.0508  0.9324 3.0059  0.9339 3.0369  0.9354 3.0314  0.9369 3.0631  0.9384 3.1865  0.9399 3.2549  0.9414 3.2202  0.9429 3.3423  0.9444 3.3885  0.9459 3.3373  0.9474 3.3798  0.9489 3.4812  0.9504 3.5537  0.9519 3.5435  0.9534 3.5766  0.9549 3.6630  0.9564 3.8235  0.9579 3.8778  0.9594 3.8310  0.9609 3.9197  0.9624 3.9946  0.9639 4.0442  0.9654 4.1330  0.9669 4.2018  0.9684 4.2377  0.9699 4.3209  0.9715 4.4057  0.9730 4.4655  0.9745 4.7453  0.9760 4.8376  0.9775 5.0430  0.9790 5.1177  0.9805 5.1419  0.9820 5.3428  0.9835 5.2901  0.9850 5.3739  0.9865 5.9489  0.9880 6.1666  0.9895 5.9475  0.9910 6.1271  0.9925 7.1237  0.9940 7.5722  0.9955 7.8521     /
\multiput {\large$\cdot$} at 0.0248 -0.0684  0.0263 -0.0619  0.0278 -0.0576  0.0293 -0.0544  0.0308 -0.0516  0.0323 -0.0497  0.0338 -0.0479  0.0353 -0.0462  0.0368 -0.0447  0.0383 -0.0437  0.0398 -0.0428  0.0413 -0.0418  0.0428 -0.0415  0.0443 -0.0409  0.0458 -0.0399  0.0473 -0.0390  0.0488 -0.0386  0.0503 -0.0379  0.0518 -0.0374  0.0533 -0.0376  0.0548 -0.0372  0.0563 -0.0363  0.0579 -0.0363  0.0594 -0.0358  0.0609 -0.0354  0.0624 -0.0350  0.0639 -0.0335  0.0654 -0.0339  0.0669 -0.0335  0.0684 -0.0323  0.0699 -0.0332  0.0714 -0.0329  0.0729 -0.0323  0.0744 -0.0317  0.0759 -0.0308  0.0774 -0.0311  0.0789 -0.0310  0.0804 -0.0291  0.0819 -0.0290  0.0834 -0.0303  0.0849 -0.0289  0.0864 -0.0278  0.0879 -0.0283  0.0894 -0.0279  0.0909 -0.0264  0.0924 -0.0254  0.0939 -0.0256  0.0954 -0.0253  0.0969 -0.0252  0.0984 -0.0248  0.0999 -0.0253  0.1014 -0.0246  0.1029 -0.0235  0.1044 -0.0237  0.1059 -0.0226  0.1074 -0.0229  0.1089 -0.0233  0.1104 -0.0223  0.1119 -0.0213  0.1134 -0.0210  0.1150 -0.0208  0.1165 -0.0202  0.1180 -0.0190  0.1195 -0.0197  0.1210 -0.0194  0.1225 -0.0178  0.1240 -0.0174  0.1255 -0.0161  0.1270 -0.0172  0.1285 -0.0154  0.1300 -0.0136  0.1315 -0.0151  0.1330 -0.0152  0.1345 -0.0137  0.1360 -0.0128  0.1375 -0.0149  0.1390 -0.0139  0.1405 -0.0127  0.1420 -0.0124  0.1435 -0.0109  0.1450 -0.0099  0.1465 -0.0106  0.1480 -0.0104  0.1495 -0.0090  0.1510 -0.0097  0.1525 -0.0074  0.1540 -0.0076  0.1555 -0.0080  0.1570 -0.0067  0.1585 -0.0081  0.1600 -0.0053  0.1615 -0.0044  0.1630 -0.0056  0.1645 -0.0044  0.1660 -0.0018  0.1675 -0.0030  0.1690 -0.0044  0.1705 0.0001  0.1721 0.0011  0.1736 -0.0012  0.1751 -0.0004  0.1766 0.0012  0.1781 0.0002  0.1796 0.0014  0.1811 0.0023  0.1826 0.0029  0.1841 0.0058  0.1856 0.0053  0.1871 0.0034  0.1886 0.0045  0.1901 0.0040  0.1916 0.0046  0.1931 0.0058  0.1946 0.0073  0.1961 0.0091  0.1976 0.0091  0.1991 0.0088  0.2006 0.0118  0.2021 0.0105  0.2036 0.0078  0.2051 0.0153  0.2066 0.0148  0.2081 0.0126  0.2096 0.0139  0.2111 0.0145  0.2126 0.0124  0.2141 0.0143  0.2156 0.0205  0.2171 0.0170  0.2186 0.0160  0.2201 0.0187  0.2216 0.0186  0.2231 0.0221  0.2246 0.0223  0.2261 0.0211  0.2276 0.0239  0.2292 0.0242  0.2307 0.0236  0.2322 0.0232  0.2337 0.0225  0.2352 0.0236  0.2367 0.0271  0.2382 0.0291  0.2397 0.0288  0.2412 0.0309  0.2427 0.0302  0.2442 0.0275  0.2457 0.0303  0.2472 0.0305  0.2487 0.0337  0.2502 0.0350  0.2517 0.0332  0.2532 0.0382  0.2547 0.0350  0.2562 0.0352  0.2577 0.0398  0.2592 0.0399  0.2607 0.0357  0.2622 0.0344  0.2637 0.0409  0.2652 0.0445  0.2667 0.0438  0.2682 0.0398  0.2697 0.0435  0.2712 0.0481  0.2727 0.0418  0.2742 0.0416  0.2757 0.0423  0.2772 0.0463  0.2787 0.0465  0.2802 0.0407  0.2817 0.0494  0.2832 0.0556  0.2847 0.0553  0.2863 0.0527  0.2878 0.0530  0.2893 0.0580  0.2908 0.0568  0.2923 0.0597  0.2938 0.0579  0.2953 0.0604  0.2968 0.0656  0.2983 0.0615  0.2998 0.0596  0.3013 0.0673  0.3028 0.0685  0.3043 0.0623  0.3058 0.0660  0.3073 0.0621  0.3088 0.0697  0.3103 0.0714  0.3118 0.0649  0.3133 0.0701  0.3148 0.0731  0.3163 0.0788  0.3178 0.0747  0.3193 0.0712  0.3208 0.0846  0.3223 0.0798  0.3238 0.0718  0.3253 0.0826  0.3268 0.0813  0.3283 0.0804  0.3298 0.0857  0.3313 0.0913  0.3328 0.0864  0.3343 0.0816  0.3358 0.0871  0.3373 0.0846  0.3388 0.0904  0.3403 0.0948  0.3418 0.0871  0.3434 0.0921  0.3449 0.1014  0.3464 0.0965  0.3479 0.0965  0.3494 0.0963  0.3509 0.0923  0.3524 0.1069  0.3539 0.1104  0.3554 0.0913  0.3569 0.0977  0.3584 0.1007  0.3599 0.1052  0.3614 0.1153  0.3629 0.1180  0.3644 0.1136  0.3659 0.1128  0.3674 0.1161  0.3689 0.1151  0.3704 0.1208  0.3719 0.1182  0.3734 0.1210  0.3749 0.1177  0.3764 0.1213  0.3779 0.1272  0.3794 0.1278  0.3809 0.1217  0.3824 0.1217  0.3839 0.1327  0.3854 0.1370  0.3869 0.1350  0.3884 0.1321  0.3899 0.1344  0.3914 0.1357  0.3929 0.1338  0.3944 0.1391  0.3959 0.1353  0.3974 0.1382  0.3989 0.1540  0.4005 0.1461  0.4020 0.1447  0.4035 0.1499  0.4050 0.1475  0.4065 0.1511  0.4080 0.1514  0.4095 0.1419  0.4110 0.1501  0.4125 0.1698  0.4140 0.1563  0.4155 0.1533  0.4170 0.1671  0.4185 0.1562  0.4200 0.1596  0.4215 0.1680  0.4230 0.1707  0.4245 0.1697  0.4260 0.1749  0.4275 0.1862  0.4290 0.1683  0.4305 0.1638  0.4320 0.1773  0.4335 0.1729  0.4350 0.1623  0.4365 0.1618  0.4380 0.1916  0.4395 0.1800  0.4410 0.1838  0.4425 0.1861  0.4440 0.1703  0.4455 0.1975  0.4470 0.2005  0.4485 0.1890  0.4500 0.1939  0.4515 0.2248  0.4530 0.2293  0.4545 0.2089  0.4560 0.1556  0.4576 0.1669  0.4591 0.2585  0.4606 0.2588  0.4621 0.2206  0.4636 0.2199  0.4651 0.2287  0.4666 0.2292  0.4681 0.2168  0.4696 0.1934  0.4711 0.1740  0.4726 0.2194  0.4741 0.2044  0.4756 0.2013  0.4771 0.2470  0.4786 0.2430  0.4801 0.2486  0.4816 0.2614  0.4831 0.2503  0.4846 0.2421  0.4861 0.2596  0.4876 0.2610  0.4891 0.2629  0.4906 0.2597  0.4921 0.2622  0.4936 0.2658  0.4951 0.2687  0.4966 0.2709  0.4981 0.2728  0.4996 0.2745  0.5011 0.2776  0.5026 0.2802  0.5041 0.2898  0.5056 0.2951  0.5071 0.2942  0.5086 0.2948  0.5101 0.2924  0.5116 0.2954  0.5131 0.2976  0.5147 0.2996  0.5162 0.3024  0.5177 0.3030  0.5192 0.3183  0.5207 0.3206  0.5222 0.3154  0.5237 0.3196  0.5252 0.3177  0.5267 0.3196  0.5282 0.3222  0.5297 0.3260  0.5312 0.3314  0.5327 0.3362  0.5342 0.3412  0.5357 0.3449  0.5372 0.3425  0.5387 0.3433  0.5402 0.3470  0.5417 0.3486  0.5432 0.3548  0.5447 0.3604  0.5462 0.3591  0.5477 0.3633  0.5492 0.3697  0.5507 0.3687  0.5522 0.3690  0.5537 0.3717  0.5552 0.3734  0.5567 0.3843  0.5582 0.3869  0.5597 0.3895  0.5612 0.3924  0.5627 0.3874  0.5642 0.3934  0.5657 0.3985  0.5672 0.4000  0.5687 0.4078  0.5702 0.4186  0.5718 0.4153  0.5733 0.4117  0.5748 0.4164  0.5763 0.4192  0.5778 0.4253  0.5793 0.4317  0.5808 0.4389  0.5823 0.4387  0.5838 0.4344  0.5853 0.4394  0.5868 0.4433  0.5883 0.4501  0.5898 0.4553  0.5913 0.4627  0.5928 0.4629  0.5943 0.4583  0.5958 0.4625  0.5973 0.4702  0.5988 0.4767  0.6003 0.4840  0.6018 0.4868  0.6033 0.4840  0.6048 0.4873  0.6063 0.4915  0.6078 0.5031  0.6093 0.5084  0.6108 0.5041  0.6123 0.5052  0.6138 0.5111  0.6153 0.5165  0.6168 0.5256  0.6183 0.5271  0.6198 0.5254  0.6213 0.5297  0.6228 0.5390  0.6243 0.5493  0.6258 0.5464  0.6273 0.5453  0.6289 0.5487  0.6304 0.5576  0.6319 0.5694  0.6334 0.5676  0.6349 0.5663  0.6364 0.5722  0.6379 0.5817  0.6394 0.5921  0.6409 0.5907  0.6424 0.5881  0.6439 0.5924  0.6454 0.6018  0.6469 0.6129  0.6484 0.6119  0.6499 0.6096  0.6514 0.6204  0.6529 0.6323  0.6544 0.6311  0.6559 0.6292  0.6574 0.6397  0.6589 0.6505  0.6604 0.6510  0.6619 0.6488  0.6634 0.6605  0.6649 0.6694  0.6664 0.6665  0.6679 0.6683  0.6694 0.6801  0.6709 0.6930  0.6724 0.6913  0.6739 0.6872  0.6754 0.6986  0.6769 0.7129  0.6784 0.7125  0.6799 0.7110  0.6814 0.7216  0.6829 0.7305  0.6844 0.7315  0.6860 0.7320  0.6875 0.7500  0.6890 0.7563  0.6905 0.7484  0.6920 0.7627  0.6935 0.7679  0.6950 0.7644  0.6965 0.7856  0.6980 0.7910  0.6995 0.7820  0.7010 0.8009  0.7025 0.8073  0.7040 0.8006  0.7055 0.8197  0.7070 0.8276  0.7085 0.8208  0.7100 0.8359  0.7115 0.8417  0.7130 0.8373  0.7145 0.8525  0.7160 0.8596  0.7175 0.8579  0.7190 0.8648  0.7205 0.8724  0.7220 0.8784  0.7235 0.8860  0.7250 0.8921  0.7265 0.8982  0.7280 0.9050  0.7295 0.9120  0.7310 0.9207  0.7325 0.9265  0.7340 0.9346  0.7355 0.9428  0.7370 0.9499  0.7385 0.9575  0.7400 0.9636  0.7415 0.9691  0.7431 0.9793  0.7446 0.9874  0.7461 0.9936  0.7476 0.9995  0.7491 1.0060  0.7506 1.0169  0.7521 1.0260  0.7536 1.0327  0.7551 1.0385  0.7566 1.0481  0.7581 1.0543  0.7596 1.0608  0.7611 1.0742  0.7626 1.0815  0.7641 1.0881  0.7656 1.0969  0.7671 1.1054  0.7686 1.1151  0.7701 1.1217  0.7716 1.1303  0.7731 1.1422  0.7746 1.1513  0.7761 1.1611  0.7776 1.1697  0.7791 1.1776  0.7806 1.1884  0.7821 1.1976  0.7836 1.2046  0.7851 1.2155  0.7866 1.2259  0.7881 1.2347  0.7896 1.2439  0.7911 1.2556  0.7926 1.2654  0.7941 1.2727  0.7956 1.2824  0.7971 1.2933  0.7986 1.3050  0.8002 1.3157  0.8017 1.3263  0.8032 1.3360  0.8047 1.3467  0.8062 1.3582  0.8077 1.3679  0.8092 1.3797  0.8107 1.3829  0.8122 1.3930  0.8137 1.4160  0.8152 1.4139  0.8167 1.4256  0.8182 1.4545  0.8197 1.4453  0.8212 1.4588  0.8227 1.4929  0.8242 1.4842  0.8257 1.4965  0.8272 1.5296  0.8287 1.5240  0.8302 1.5324  0.8317 1.5623  0.8332 1.5642  0.8347 1.5790  0.8362 1.6070  0.8377 1.6014  0.8392 1.6154  0.8407 1.6488  0.8422 1.6482  0.8437 1.6608  0.8452 1.6895  0.8467 1.6870  0.8482 1.7017  0.8497 1.7379  0.8512 1.7322  0.8527 1.7446  0.8542 1.7803  0.8557 1.7808  0.8573 1.7939  0.8588 1.8285  0.8603 1.8289  0.8618 1.8432  0.8633 1.8692  0.8648 1.8787  0.8663 1.8974  0.8678 1.9123  0.8693 1.9282  0.8708 1.9467  0.8723 1.9661  0.8738 1.9836  0.8753 1.9999  0.8768 2.0260  0.8783 2.0336  0.8798 2.0586  0.8813 2.0781  0.8828 2.0972  0.8843 2.1185  0.8858 2.1365  0.8873 2.1609  0.8888 2.1821  0.8903 2.1983  0.8918 2.2271  0.8933 2.2490  0.8948 2.2691  0.8963 2.2903  0.8978 2.3129  0.8993 2.3365  0.9008 2.3531  0.9023 2.3769  0.9038 2.4106  0.9053 2.4309  0.9068 2.4637  0.9083 2.4890  0.9098 2.5042  0.9113 2.5409  0.9128 2.5734  0.9144 2.5942  0.9159 2.6118  0.9174 2.6527  0.9189 2.6676  0.9204 2.7031  0.9219 2.7527  0.9234 2.7706  0.9249 2.7916  0.9264 2.8302  0.9279 2.8488  0.9294 3.0076  0.9309 3.0508  0.9324 3.0059  0.9339 3.0369  0.9354 3.0314  0.9369 3.0631  0.9384 3.1865  0.9399 3.2549  0.9414 3.2202  0.9429 3.3423  0.9444 3.3885  0.9459 3.3373  0.9474 3.3798  0.9489 3.4812  0.9504 3.5537  0.9519 3.5435  0.9534 3.5766  0.9549 3.6630  0.9564 3.8235  0.9579 3.8778  0.9594 3.8310  0.9609 3.9197  0.9624 3.9946  0.9639 4.0442  0.9654 4.1330  0.9669 4.2018  0.9684 4.2377  0.9699 4.3209  0.9715 4.4057  0.9730 4.4655  0.9745 4.7453  0.9760 4.8376  0.9775 5.0430  0.9790 5.1177  0.9805 5.1419  0.9820 5.3428  0.9835 5.2901  0.9850 5.3739  0.9865 5.9489  0.9880 6.1666  0.9895 5.9475  0.9910 6.1271  0.9925 7.1237  0.9940 7.5722  0.9955 7.8521     /


%L=12
\color{B12}
%\plot 0.0191 -0.0516  0.0203 -0.0474  0.0214 -0.0441  0.0226 -0.0415  0.0237 -0.0393  0.0249 -0.0377  0.0260 -0.0363  0.0272 -0.0352  0.0284 -0.0342  0.0295 -0.0336  0.0307 -0.0327  0.0318 -0.0317  0.0330 -0.0313  0.0341 -0.0307  0.0353 -0.0302  0.0365 -0.0300  0.0376 -0.0296  0.0388 -0.0292  0.0399 -0.0284  0.0411 -0.0283  0.0422 -0.0287  0.0434 -0.0282  0.0446 -0.0274  0.0457 -0.0272  0.0469 -0.0277  0.0480 -0.0274  0.0492 -0.0268  0.0503 -0.0260  0.0515 -0.0253  0.0527 -0.0256  0.0538 -0.0255  0.0550 -0.0251  0.0561 -0.0250  0.0573 -0.0251  0.0584 -0.0242  0.0596 -0.0238  0.0608 -0.0240  0.0619 -0.0238  0.0631 -0.0239  0.0642 -0.0236  0.0654 -0.0235  0.0666 -0.0231  0.0677 -0.0228  0.0689 -0.0230  0.0700 -0.0227  0.0712 -0.0215  0.0723 -0.0209  0.0735 -0.0212  0.0747 -0.0210  0.0758 -0.0204  0.0770 -0.0206  0.0781 -0.0209  0.0793 -0.0196  0.0804 -0.0192  0.0816 -0.0197  0.0828 -0.0193  0.0839 -0.0191  0.0851 -0.0189  0.0862 -0.0183  0.0874 -0.0177  0.0885 -0.0177  0.0897 -0.0185  0.0909 -0.0185  0.0920 -0.0171  0.0932 -0.0170  0.0943 -0.0172  0.0955 -0.0174  0.0966 -0.0170  0.0978 -0.0152  0.0990 -0.0160  0.1001 -0.0159  0.1013 -0.0154  0.1024 -0.0155  0.1036 -0.0140  0.1047 -0.0141  0.1059 -0.0149  0.1071 -0.0144  0.1082 -0.0135  0.1094 -0.0137  0.1105 -0.0128  0.1117 -0.0126  0.1128 -0.0130  0.1140 -0.0119  0.1152 -0.0114  0.1163 -0.0108  0.1175 -0.0108  0.1186 -0.0101  0.1198 -0.0089  0.1209 -0.0097  0.1221 -0.0101  0.1233 -0.0088  0.1244 -0.0093  0.1256 -0.0096  0.1267 -0.0067  0.1279 -0.0066  0.1291 -0.0079  0.1302 -0.0090  0.1314 -0.0085  0.1325 -0.0066  0.1337 -0.0060  0.1348 -0.0064  0.1360 -0.0073  0.1372 -0.0064  0.1383 -0.0051  0.1395 -0.0039  0.1406 -0.0030  0.1418 -0.0023  0.1429 -0.0036  0.1441 -0.0045  0.1453 -0.0032  0.1464 -0.0033  0.1476 -0.0029  0.1487 -0.0023  0.1499 -0.0023  0.1510 -0.0005  0.1522 -0.0004  0.1534 -0.0004  0.1545 -0.0001  0.1557 -0.0007  0.1568 -0.0001  0.1580 0.0010  0.1591 0.0023  0.1603 0.0022  0.1615 0.0027  0.1626 0.0041  0.1638 0.0040  0.1649 0.0029  0.1661 0.0021  0.1672 0.0042  0.1684 0.0060  0.1696 0.0071  0.1707 0.0047  0.1719 0.0047  0.1730 0.0078  0.1742 0.0066  0.1753 0.0065  0.1765 0.0093  0.1777 0.0100  0.1788 0.0085  0.1800 0.0070  0.1811 0.0101  0.1823 0.0097  0.1834 0.0074  0.1846 0.0106  0.1858 0.0118  0.1869 0.0121  0.1881 0.0111  0.1892 0.0130  0.1904 0.0134  0.1916 0.0111  0.1927 0.0128  0.1939 0.0149  0.1950 0.0141  0.1962 0.0160  0.1973 0.0172  0.1985 0.0156  0.1997 0.0159  0.2008 0.0157  0.2020 0.0156  0.2031 0.0148  0.2043 0.0164  0.2054 0.0173  0.2066 0.0212  0.2078 0.0213  0.2089 0.0183  0.2101 0.0216  0.2112 0.0232  0.2124 0.0216  0.2135 0.0219  0.2147 0.0198  0.2159 0.0192  0.2170 0.0226  0.2182 0.0238  0.2193 0.0260  0.2205 0.0269  0.2216 0.0256  0.2228 0.0231  0.2240 0.0243  0.2251 0.0291  0.2263 0.0288  0.2274 0.0261  0.2286 0.0270  0.2297 0.0286  0.2309 0.0308  0.2321 0.0278  0.2332 0.0290  0.2344 0.0290  0.2355 0.0293  0.2367 0.0318  0.2378 0.0290  0.2390 0.0365  0.2402 0.0403  0.2413 0.0352  0.2425 0.0352  0.2436 0.0343  0.2448 0.0343  0.2459 0.0374  0.2471 0.0369  0.2483 0.0375  0.2494 0.0409  0.2506 0.0443  0.2517 0.0433  0.2529 0.0400  0.2541 0.0361  0.2552 0.0383  0.2564 0.0463  0.2575 0.0448  0.2587 0.0421  0.2598 0.0435  0.2610 0.0446  0.2622 0.0468  0.2633 0.0471  0.2645 0.0480  0.2656 0.0457  0.2668 0.0448  0.2679 0.0467  0.2691 0.0488  0.2703 0.0507  0.2714 0.0521  0.2726 0.0544  0.2737 0.0526  0.2749 0.0517  0.2760 0.0507  0.2772 0.0523  0.2784 0.0569  0.2795 0.0584  0.2807 0.0536  0.2818 0.0537  0.2830 0.0535  0.2841 0.0564  0.2853 0.0586  0.2865 0.0589  0.2876 0.0621  0.2888 0.0579  0.2899 0.0601  0.2911 0.0629  0.2922 0.0615  0.2934 0.0571  0.2946 0.0609  0.2957 0.0669  0.2969 0.0649  0.2980 0.0690  0.2992 0.0693  0.3003 0.0666  0.3015 0.0687  0.3027 0.0683  0.3038 0.0705  0.3050 0.0753  0.3061 0.0713  0.3073 0.0715  0.3084 0.0739  0.3096 0.0737  0.3108 0.0734  0.3119 0.0735  0.3131 0.0692  0.3142 0.0745  0.3154 0.0796  0.3166 0.0778  0.3177 0.0812  0.3189 0.0775  0.3200 0.0812  0.3212 0.0890  0.3223 0.0859  0.3235 0.0784  0.3247 0.0860  0.3258 0.0873  0.3270 0.0841  0.3281 0.0873  0.3293 0.0886  0.3304 0.0857  0.3316 0.0846  0.3328 0.0916  0.3339 0.0983  0.3351 0.0945  0.3362 0.0894  0.3374 0.0946  0.3385 0.0957  0.3397 0.0913  0.3409 0.0960  0.3420 0.1002  0.3432 0.0987  0.3443 0.0973  0.3455 0.1004  0.3466 0.1015  0.3478 0.0971  0.3490 0.1034  0.3501 0.1069  0.3513 0.1031  0.3524 0.1063  0.3536 0.1078  0.3547 0.1060  0.3559 0.1074  0.3571 0.1080  0.3582 0.1105  0.3594 0.1103  0.3605 0.1136  0.3617 0.1161  0.3628 0.1111  0.3640 0.1130  0.3652 0.1123  0.3663 0.1146  0.3675 0.1211  0.3686 0.1190  0.3698 0.1252  0.3709 0.1264  0.3721 0.1184  0.3733 0.1241  0.3744 0.1263  0.3756 0.1248  0.3767 0.1309  0.3779 0.1245  0.3791 0.1270  0.3802 0.1364  0.3814 0.1281  0.3825 0.1262  0.3837 0.1368  0.3848 0.1475  0.3860 0.1349  0.3872 0.1333  0.3883 0.1502  0.3895 0.1354  0.3906 0.1303  0.3918 0.1357  0.3929 0.1438  0.3941 0.1459  0.3953 0.1335  0.3964 0.1415  0.3976 0.1601  0.3987 0.1626  0.3999 0.1413  0.4010 0.1403  0.4022 0.1498  0.4034 0.1549  0.4045 0.1546  0.4057 0.1505  0.4068 0.1612  0.4080 0.1595  0.4091 0.1532  0.4103 0.1554  0.4115 0.1622  0.4126 0.1624  0.4138 0.1663  0.4149 0.1593  0.4161 0.1576  0.4172 0.1713  0.4184 0.1713  0.4196 0.1664  0.4207 0.1660  0.4219 0.1692  0.4230 0.1688  0.4242 0.1745  0.4253 0.1729  0.4265 0.1756  0.4277 0.1801  0.4288 0.1688  0.4300 0.1705  0.4311 0.1777  0.4323 0.1762  0.4334 0.1743  0.4346 0.1940  0.4358 0.1984  0.4369 0.1774  0.4381 0.1818  0.4392 0.1921  0.4404 0.1907  0.4416 0.1954  0.4427 0.2148  0.4439 0.2020  0.4450 0.1864  0.4462 0.2038  0.4473 0.2040  0.4485 0.1854  0.4497 0.1967  0.4508 0.1927  0.4520 0.1705  0.4531 0.2134  0.4543 0.2170  0.4554 0.1932  0.4566 0.2068  0.4578 0.2146  0.4589 0.2140  0.4601 0.2141  0.4612 0.2133  0.4624 0.2124  0.4635 0.2330  0.4647 0.2243  0.4659 0.2283  0.4670 0.2222  0.4682 0.1279  0.4693 0.1334  0.4705 0.2248  0.4716 0.1913  0.4728 0.2481  0.4740 0.2461  0.4751 0.1904  0.4763 0.2405  0.4774 0.2994  0.4786 0.2477  0.4797 0.1934  0.4809 0.2544  0.4821 0.2624  0.4832 0.2684  0.4844 0.3103  0.4855 0.3083  0.4867 0.2589  0.4878 0.2473  0.4890 0.1930  0.4902 0.2760  0.4913 0.2920  0.4925 0.2531  0.4936 0.2940  0.4948 0.2858  0.4959 0.2401  0.4971 0.2343  0.4983 0.2730  0.4994 0.2658  0.5006 0.2810  0.5017 0.2821  0.5029 0.2823  0.5041 0.2845  0.5052 0.2876  0.5064 0.2875  0.5075 0.2914  0.5087 0.2940  0.5098 0.2951  0.5110 0.3075  0.5122 0.3111  0.5133 0.3081  0.5145 0.3042  0.5156 0.3019  0.5168 0.3085  0.5179 0.3081  0.5191 0.3075  0.5203 0.3096  0.5214 0.3134  0.5226 0.3253  0.5237 0.3208  0.5249 0.3261  0.5260 0.3330  0.5272 0.3230  0.5284 0.3263  0.5295 0.3288  0.5307 0.3302  0.5318 0.3342  0.5330 0.3348  0.5341 0.3377  0.5353 0.3499  0.5365 0.3517  0.5376 0.3436  0.5388 0.3438  0.5399 0.3502  0.5411 0.3521  0.5422 0.3528  0.5434 0.3580  0.5446 0.3594  0.5457 0.3662  0.5469 0.3756  0.5480 0.3698  0.5492 0.3645  0.5503 0.3689  0.5515 0.3722  0.5527 0.3715  0.5538 0.3776  0.5550 0.3848  0.5561 0.3878  0.5573 0.3849  0.5584 0.3881  0.5596 0.3907  0.5608 0.3874  0.5619 0.3937  0.5631 0.3973  0.5642 0.3984  0.5654 0.4000  0.5666 0.4085  0.5677 0.4089  0.5689 0.4043  0.5700 0.4075  0.5712 0.4107  0.5723 0.4191  0.5735 0.4223  0.5747 0.4247  0.5758 0.4311  0.5770 0.4290  0.5781 0.4261  0.5793 0.4290  0.5804 0.4275  0.5816 0.4384  0.5828 0.4432  0.5839 0.4459  0.5851 0.4486  0.5862 0.4412  0.5874 0.4443  0.5885 0.4498  0.5897 0.4593  0.5909 0.4644  0.5920 0.4692  0.5932 0.4679  0.5943 0.4630  0.5955 0.4649  0.5966 0.4649  0.5978 0.4787  0.5990 0.4859  0.6001 0.4839  0.6013 0.4855  0.6024 0.4816  0.6036 0.4847  0.6047 0.4948  0.6059 0.5030  0.6071 0.5016  0.6082 0.4972  0.6094 0.4978  0.6105 0.5011  0.6117 0.5020  0.6128 0.5197  0.6140 0.5312  0.6152 0.5217  0.6163 0.5198  0.6175 0.5234  0.6186 0.5268  0.6198 0.5366  0.6209 0.5443  0.6221 0.5386  0.6233 0.5355  0.6244 0.5385  0.6256 0.5415  0.6267 0.5555  0.6279 0.5632  0.6291 0.5578  0.6302 0.5595  0.6314 0.5623  0.6325 0.5749  0.6337 0.5751  0.6348 0.5671  0.6360 0.5764  0.6372 0.5780  0.6383 0.5776  0.6395 0.5916  0.6406 0.5968  0.6418 0.5895  0.6429 0.5909  0.6441 0.5947  0.6453 0.6090  0.6464 0.6166  0.6476 0.6100  0.6487 0.6121  0.6499 0.6116  0.6510 0.6262  0.6522 0.6373  0.6534 0.6311  0.6545 0.6330  0.6557 0.6335  0.6568 0.6443  0.6580 0.6525  0.6591 0.6460  0.6603 0.6426  0.6615 0.6540  0.6626 0.6702  0.6638 0.6639  0.6649 0.6591  0.6661 0.6659  0.6672 0.6804  0.6684 0.6827  0.6696 0.6748  0.6707 0.6843  0.6719 0.6917  0.6730 0.6992  0.6742 0.7016  0.6753 0.6968  0.6765 0.7070  0.6777 0.7233  0.6788 0.7191  0.6800 0.7148  0.6811 0.7220  0.6823 0.7343  0.6834 0.7309  0.6846 0.7217  0.6858 0.7345  0.6869 0.7528  0.6881 0.7568  0.6892 0.7507  0.6904 0.7563  0.6916 0.7695  0.6927 0.7708  0.6939 0.7696  0.6950 0.7792  0.6962 0.7851  0.6973 0.7803  0.6985 0.7784  0.6997 0.8007  0.7008 0.8091  0.7020 0.7956  0.7031 0.8031  0.7043 0.8179  0.7054 0.8195  0.7066 0.8197  0.7078 0.8305  0.7089 0.8311  0.7101 0.8250  0.7112 0.8413  0.7124 0.8465  0.7135 0.8453  0.7147 0.8644  0.7159 0.8649  0.7170 0.8603  0.7182 0.8766  0.7193 0.8792  0.7205 0.8785  0.7216 0.8934  0.7228 0.8989  0.7240 0.8959  0.7251 0.9098  0.7263 0.9135  0.7274 0.9070  0.7286 0.9214  0.7297 0.9295  0.7309 0.9313  0.7321 0.9428  0.7332 0.9431  0.7344 0.9431  0.7355 0.9568  0.7367 0.9573  0.7378 0.9569  0.7390 0.9714  0.7402 0.9707  0.7413 0.9742  0.7425 0.9918  0.7436 0.9930  0.7448 0.9894  0.7459 0.9985  0.7471 1.0048  0.7483 1.0084  0.7494 1.0170  0.7506 1.0191  0.7517 1.0218  0.7529 1.0323  0.7541 1.0422  0.7552 1.0469  0.7564 1.0508  0.7575 1.0536  0.7587 1.0612  0.7598 1.0688  0.7610 1.0760  0.7622 1.0857  0.7633 1.0892  0.7645 1.0937  0.7656 1.1035  0.7668 1.1102  0.7679 1.1143  0.7691 1.1201  0.7703 1.1278  0.7714 1.1372  0.7726 1.1422  0.7737 1.1486  0.7749 1.1586  0.7760 1.1648  0.7772 1.1692  0.7784 1.1757  0.7795 1.1843  0.7807 1.1899  0.7818 1.1935  0.7830 1.2034  0.7841 1.2136  0.7853 1.2218  0.7865 1.2301  0.7876 1.2364  0.7888 1.2437  0.7899 1.2545  0.7911 1.2612  0.7922 1.2663  0.7934 1.2750  0.7946 1.2827  0.7957 1.2894  0.7969 1.2941  0.7980 1.3038  0.7992 1.3160  0.8003 1.3224  0.8015 1.3266  0.8027 1.3334  0.8038 1.3448  0.8050 1.3553  0.8061 1.3651  0.8073 1.3774  0.8084 1.3830  0.8096 1.3884  0.8108 1.3970  0.8119 1.4067  0.8131 1.4201  0.8142 1.4120  0.8154 1.4189  0.8166 1.4454  0.8177 1.4440  0.8189 1.4555  0.8200 1.4755  0.8212 1.4654  0.8223 1.4769  0.8235 1.5029  0.8247 1.4942  0.8258 1.5053  0.8270 1.5325  0.8281 1.5274  0.8293 1.5345  0.8304 1.5572  0.8316 1.5517  0.8328 1.5626  0.8339 1.5889  0.8351 1.5835  0.8362 1.5949  0.8374 1.6236  0.8385 1.6168  0.8397 1.6273  0.8409 1.6542  0.8420 1.6466  0.8432 1.6591  0.8443 1.6884  0.8455 1.6821  0.8466 1.6925  0.8478 1.7211  0.8490 1.7133  0.8501 1.7256  0.8513 1.7587  0.8524 1.7512  0.8536 1.7603  0.8547 1.7891  0.8559 1.7827  0.8571 1.7960  0.8582 1.8285  0.8594 1.8209  0.8605 1.8339  0.8617 1.8507  0.8628 1.8586  0.8640 1.8851  0.8652 1.8816  0.8663 1.8942  0.8675 1.9205  0.8686 1.9264  0.8698 1.9415  0.8709 1.9626  0.8721 1.9755  0.8733 1.9856  0.8744 1.9982  0.8756 2.0201  0.8767 2.0283  0.8779 2.0400  0.8791 2.0606  0.8802 2.0692  0.8814 2.0812  0.8825 2.0922  0.8837 2.1201  0.8848 2.1408  0.8860 2.1473  0.8872 2.1637  0.8883 2.1808  0.8895 2.1969  0.8906 2.2144  0.8918 2.2303  0.8929 2.2444  0.8941 2.2590  0.8953 2.2794  0.8964 2.2988  0.8976 2.3161  0.8987 2.3351  0.8999 2.3509  0.9010 2.3674  0.9022 2.3885  0.9034 2.4106  0.9045 2.4286  0.9057 2.4459  0.9068 2.4667  0.9080 2.4893  0.9091 2.5010  0.9103 2.5261  0.9115 2.5478  0.9126 2.5706  0.9138 2.5918  0.9149 2.6042  0.9161 2.6383  0.9172 2.6587  0.9184 2.6774  0.9196 2.6996  0.9207 2.7223  0.9219 2.7422  0.9230 2.7588  0.9242 2.7848  0.9253 2.8199  0.9265 2.8114  0.9277 2.8205  0.9288 2.9451  0.9300 2.9846  0.9311 2.9288  0.9323 3.0685  0.9334 3.1206  0.9346 3.0053  0.9358 3.0669  0.9369 3.1377  0.9381 3.1054  0.9392 3.1226  0.9404 3.2784  0.9416 3.2775  0.9427 3.2182  0.9439 3.4287  0.9450 3.4138  0.9462 3.3028  0.9473 3.5245  0.9485 3.5409  0.9497 3.4357  0.9508 3.4907  0.9520 3.5451  0.9531 3.6426  0.9543 3.6892  0.9554 3.6827  0.9566 3.7023  0.9578 3.8180  0.9589 3.8542  0.9601 3.7746  0.9612 3.8524  0.9624 3.9708  0.9635 4.0355  0.9647 4.2349  0.9659 4.1937  0.9670 4.0181  0.9682 4.1532  0.9693 3.9487  0.9705 5.3571  0.9716 5.6031  0.9728 4.2978  0.9740 4.2794  0.9751 5.1387  0.9763 5.3680  0.9774 4.7052  0.9786 4.8236  0.9797 4.7489  0.9809 4.9848  0.9821 5.8368  0.9832 5.7463  
% /
\multiput {\large$\cdot$} at 0.0191 -0.0516  0.0203 -0.0474  0.0214 -0.0441  0.0226 -0.0415  0.0237 -0.0393  0.0249 -0.0377  0.0260 -0.0363  0.0272 -0.0352  0.0284 -0.0342  0.0295 -0.0336  0.0307 -0.0327  0.0318 -0.0317  0.0330 -0.0313  0.0341 -0.0307  0.0353 -0.0302  0.0365 -0.0300  0.0376 -0.0296  0.0388 -0.0292  0.0399 -0.0284  0.0411 -0.0283  0.0422 -0.0287  0.0434 -0.0282  0.0446 -0.0274  0.0457 -0.0272  0.0469 -0.0277  0.0480 -0.0274  0.0492 -0.0268  0.0503 -0.0260  0.0515 -0.0253  0.0527 -0.0256  0.0538 -0.0255  0.0550 -0.0251  0.0561 -0.0250  0.0573 -0.0251  0.0584 -0.0242  0.0596 -0.0238  0.0608 -0.0240  0.0619 -0.0238  0.0631 -0.0239  0.0642 -0.0236  0.0654 -0.0235  0.0666 -0.0231  0.0677 -0.0228  0.0689 -0.0230  0.0700 -0.0227  0.0712 -0.0215  0.0723 -0.0209  0.0735 -0.0212  0.0747 -0.0210  0.0758 -0.0204  0.0770 -0.0206  0.0781 -0.0209  0.0793 -0.0196  0.0804 -0.0192  0.0816 -0.0197  0.0828 -0.0193  0.0839 -0.0191  0.0851 -0.0189  0.0862 -0.0183  0.0874 -0.0177  0.0885 -0.0177  0.0897 -0.0185  0.0909 -0.0185  0.0920 -0.0171  0.0932 -0.0170  0.0943 -0.0172  0.0955 -0.0174  0.0966 -0.0170  0.0978 -0.0152  0.0990 -0.0160  0.1001 -0.0159  0.1013 -0.0154  0.1024 -0.0155  0.1036 -0.0140  0.1047 -0.0141  0.1059 -0.0149  0.1071 -0.0144  0.1082 -0.0135  0.1094 -0.0137  0.1105 -0.0128  0.1117 -0.0126  0.1128 -0.0130  0.1140 -0.0119  0.1152 -0.0114  0.1163 -0.0108  0.1175 -0.0108  0.1186 -0.0101  0.1198 -0.0089  0.1209 -0.0097  0.1221 -0.0101  0.1233 -0.0088  0.1244 -0.0093  0.1256 -0.0096  0.1267 -0.0067  0.1279 -0.0066  0.1291 -0.0079  0.1302 -0.0090  0.1314 -0.0085  0.1325 -0.0066  0.1337 -0.0060  0.1348 -0.0064  0.1360 -0.0073  0.1372 -0.0064  0.1383 -0.0051  0.1395 -0.0039  0.1406 -0.0030  0.1418 -0.0023  0.1429 -0.0036  0.1441 -0.0045  0.1453 -0.0032  0.1464 -0.0033  0.1476 -0.0029  0.1487 -0.0023  0.1499 -0.0023  0.1510 -0.0005  0.1522 -0.0004  0.1534 -0.0004  0.1545 -0.0001  0.1557 -0.0007  0.1568 -0.0001  0.1580 0.0010  0.1591 0.0023  0.1603 0.0022  0.1615 0.0027  0.1626 0.0041  0.1638 0.0040  0.1649 0.0029  0.1661 0.0021  0.1672 0.0042  0.1684 0.0060  0.1696 0.0071  0.1707 0.0047  0.1719 0.0047  0.1730 0.0078  0.1742 0.0066  0.1753 0.0065  0.1765 0.0093  0.1777 0.0100  0.1788 0.0085  0.1800 0.0070  0.1811 0.0101  0.1823 0.0097  0.1834 0.0074  0.1846 0.0106  0.1858 0.0118  0.1869 0.0121  0.1881 0.0111  0.1892 0.0130  0.1904 0.0134  0.1916 0.0111  0.1927 0.0128  0.1939 0.0149  0.1950 0.0141  0.1962 0.0160  0.1973 0.0172  0.1985 0.0156  0.1997 0.0159  0.2008 0.0157  0.2020 0.0156  0.2031 0.0148  0.2043 0.0164  0.2054 0.0173  0.2066 0.0212  0.2078 0.0213  0.2089 0.0183  0.2101 0.0216  0.2112 0.0232  0.2124 0.0216  0.2135 0.0219  0.2147 0.0198  0.2159 0.0192  0.2170 0.0226  0.2182 0.0238  0.2193 0.0260  0.2205 0.0269  0.2216 0.0256  0.2228 0.0231  0.2240 0.0243  0.2251 0.0291  0.2263 0.0288  0.2274 0.0261  0.2286 0.0270  0.2297 0.0286  0.2309 0.0308  0.2321 0.0278  0.2332 0.0290  0.2344 0.0290  0.2355 0.0293  0.2367 0.0318  0.2378 0.0290  0.2390 0.0365  0.2402 0.0403  0.2413 0.0352  0.2425 0.0352  0.2436 0.0343  0.2448 0.0343  0.2459 0.0374  0.2471 0.0369  0.2483 0.0375  0.2494 0.0409  0.2506 0.0443  0.2517 0.0433  0.2529 0.0400  0.2541 0.0361  0.2552 0.0383  0.2564 0.0463  0.2575 0.0448  0.2587 0.0421  0.2598 0.0435  0.2610 0.0446  0.2622 0.0468  0.2633 0.0471  0.2645 0.0480  0.2656 0.0457  0.2668 0.0448  0.2679 0.0467  0.2691 0.0488  0.2703 0.0507  0.2714 0.0521  0.2726 0.0544  0.2737 0.0526  0.2749 0.0517  0.2760 0.0507  0.2772 0.0523  0.2784 0.0569  0.2795 0.0584  0.2807 0.0536  0.2818 0.0537  0.2830 0.0535  0.2841 0.0564  0.2853 0.0586  0.2865 0.0589  0.2876 0.0621  0.2888 0.0579  0.2899 0.0601  0.2911 0.0629  0.2922 0.0615  0.2934 0.0571  0.2946 0.0609  0.2957 0.0669  0.2969 0.0649  0.2980 0.0690  0.2992 0.0693  0.3003 0.0666  0.3015 0.0687  0.3027 0.0683  0.3038 0.0705  0.3050 0.0753  0.3061 0.0713  0.3073 0.0715  0.3084 0.0739  0.3096 0.0737  0.3108 0.0734  0.3119 0.0735  0.3131 0.0692  0.3142 0.0745  0.3154 0.0796  0.3166 0.0778  0.3177 0.0812  0.3189 0.0775  0.3200 0.0812  0.3212 0.0890  0.3223 0.0859  0.3235 0.0784  0.3247 0.0860  0.3258 0.0873  0.3270 0.0841  0.3281 0.0873  0.3293 0.0886  0.3304 0.0857  0.3316 0.0846  0.3328 0.0916  0.3339 0.0983  0.3351 0.0945  0.3362 0.0894  0.3374 0.0946  0.3385 0.0957  0.3397 0.0913  0.3409 0.0960  0.3420 0.1002  0.3432 0.0987  0.3443 0.0973  0.3455 0.1004  0.3466 0.1015  0.3478 0.0971  0.3490 0.1034  0.3501 0.1069  0.3513 0.1031  0.3524 0.1063  0.3536 0.1078  0.3547 0.1060  0.3559 0.1074  0.3571 0.1080  0.3582 0.1105  0.3594 0.1103  0.3605 0.1136  0.3617 0.1161  0.3628 0.1111  0.3640 0.1130  0.3652 0.1123  0.3663 0.1146  0.3675 0.1211  0.3686 0.1190  0.3698 0.1252  0.3709 0.1264  0.3721 0.1184  0.3733 0.1241  0.3744 0.1263  0.3756 0.1248  0.3767 0.1309  0.3779 0.1245  0.3791 0.1270  0.3802 0.1364  0.3814 0.1281  0.3825 0.1262  0.3837 0.1368  0.3848 0.1475  0.3860 0.1349  0.3872 0.1333  0.3883 0.1502  0.3895 0.1354  0.3906 0.1303  0.3918 0.1357  0.3929 0.1438  0.3941 0.1459  0.3953 0.1335  0.3964 0.1415  0.3976 0.1601  0.3987 0.1626  0.3999 0.1413  0.4010 0.1403  0.4022 0.1498  0.4034 0.1549  0.4045 0.1546  0.4057 0.1505  0.4068 0.1612  0.4080 0.1595  0.4091 0.1532  0.4103 0.1554  0.4115 0.1622  0.4126 0.1624  0.4138 0.1663  0.4149 0.1593  0.4161 0.1576  0.4172 0.1713  0.4184 0.1713  0.4196 0.1664  0.4207 0.1660  0.4219 0.1692  0.4230 0.1688  0.4242 0.1745  0.4253 0.1729  0.4265 0.1756  0.4277 0.1801  0.4288 0.1688  0.4300 0.1705  0.4311 0.1777  0.4323 0.1762  0.4334 0.1743  0.4346 0.1940  0.4358 0.1984  0.4369 0.1774  0.4381 0.1818  0.4392 0.1921  0.4404 0.1907  0.4416 0.1954  0.4427 0.2148  0.4439 0.2020  0.4450 0.1864  0.4462 0.2038  0.4473 0.2040  0.4485 0.1854  0.4497 0.1967  0.4508 0.1927  0.4520 0.1705  0.4531 0.2134  0.4543 0.2170  0.4554 0.1932  0.4566 0.2068  0.4578 0.2146  0.4589 0.2140  0.4601 0.2141  0.4612 0.2133  0.4624 0.2124  0.4635 0.2330  0.4647 0.2243  0.4659 0.2283  0.4670 0.2222  0.4682 0.1279  0.4693 0.1334  0.4705 0.2248  0.4716 0.1913  0.4728 0.2481  0.4740 0.2461  0.4751 0.1904  0.4763 0.2405  0.4774 0.2994  0.4786 0.2477  0.4797 0.1934  0.4809 0.2544  0.4821 0.2624  0.4832 0.2684  0.4844 0.3103  0.4855 0.3083  0.4867 0.2589  0.4878 0.2473  0.4890 0.1930  0.4902 0.2760  0.4913 0.2920  0.4925 0.2531  0.4936 0.2940  0.4948 0.2858  0.4959 0.2401  0.4971 0.2343  0.4983 0.2730  0.4994 0.2658  0.5006 0.2810  0.5017 0.2821  0.5029 0.2823  0.5041 0.2845  0.5052 0.2876  0.5064 0.2875  0.5075 0.2914  0.5087 0.2940  0.5098 0.2951  0.5110 0.3075  0.5122 0.3111  0.5133 0.3081  0.5145 0.3042  0.5156 0.3019  0.5168 0.3085  0.5179 0.3081  0.5191 0.3075  0.5203 0.3096  0.5214 0.3134  0.5226 0.3253  0.5237 0.3208  0.5249 0.3261  0.5260 0.3330  0.5272 0.3230  0.5284 0.3263  0.5295 0.3288  0.5307 0.3302  0.5318 0.3342  0.5330 0.3348  0.5341 0.3377  0.5353 0.3499  0.5365 0.3517  0.5376 0.3436  0.5388 0.3438  0.5399 0.3502  0.5411 0.3521  0.5422 0.3528  0.5434 0.3580  0.5446 0.3594  0.5457 0.3662  0.5469 0.3756  0.5480 0.3698  0.5492 0.3645  0.5503 0.3689  0.5515 0.3722  0.5527 0.3715  0.5538 0.3776  0.5550 0.3848  0.5561 0.3878  0.5573 0.3849  0.5584 0.3881  0.5596 0.3907  0.5608 0.3874  0.5619 0.3937  0.5631 0.3973  0.5642 0.3984  0.5654 0.4000  0.5666 0.4085  0.5677 0.4089  0.5689 0.4043  0.5700 0.4075  0.5712 0.4107  0.5723 0.4191  0.5735 0.4223  0.5747 0.4247  0.5758 0.4311  0.5770 0.4290  0.5781 0.4261  0.5793 0.4290  0.5804 0.4275  0.5816 0.4384  0.5828 0.4432  0.5839 0.4459  0.5851 0.4486  0.5862 0.4412  0.5874 0.4443  0.5885 0.4498  0.5897 0.4593  0.5909 0.4644  0.5920 0.4692  0.5932 0.4679  0.5943 0.4630  0.5955 0.4649  0.5966 0.4649  0.5978 0.4787  0.5990 0.4859  0.6001 0.4839  0.6013 0.4855  0.6024 0.4816  0.6036 0.4847  0.6047 0.4948  0.6059 0.5030  0.6071 0.5016  0.6082 0.4972  0.6094 0.4978  0.6105 0.5011  0.6117 0.5020  0.6128 0.5197  0.6140 0.5312  0.6152 0.5217  0.6163 0.5198  0.6175 0.5234  0.6186 0.5268  0.6198 0.5366  0.6209 0.5443  0.6221 0.5386  0.6233 0.5355  0.6244 0.5385  0.6256 0.5415  0.6267 0.5555  0.6279 0.5632  0.6291 0.5578  0.6302 0.5595  0.6314 0.5623  0.6325 0.5749  0.6337 0.5751  0.6348 0.5671  0.6360 0.5764  0.6372 0.5780  0.6383 0.5776  0.6395 0.5916  0.6406 0.5968  0.6418 0.5895  0.6429 0.5909  0.6441 0.5947  0.6453 0.6090  0.6464 0.6166  0.6476 0.6100  0.6487 0.6121  0.6499 0.6116  0.6510 0.6262  0.6522 0.6373  0.6534 0.6311  0.6545 0.6330  0.6557 0.6335  0.6568 0.6443  0.6580 0.6525  0.6591 0.6460  0.6603 0.6426  0.6615 0.6540  0.6626 0.6702  0.6638 0.6639  0.6649 0.6591  0.6661 0.6659  0.6672 0.6804  0.6684 0.6827  0.6696 0.6748  0.6707 0.6843  0.6719 0.6917  0.6730 0.6992  0.6742 0.7016  0.6753 0.6968  0.6765 0.7070  0.6777 0.7233  0.6788 0.7191  0.6800 0.7148  0.6811 0.7220  0.6823 0.7343  0.6834 0.7309  0.6846 0.7217  0.6858 0.7345  0.6869 0.7528  0.6881 0.7568  0.6892 0.7507  0.6904 0.7563  0.6916 0.7695  0.6927 0.7708  0.6939 0.7696  0.6950 0.7792  0.6962 0.7851  0.6973 0.7803  0.6985 0.7784  0.6997 0.8007  0.7008 0.8091  0.7020 0.7956  0.7031 0.8031  0.7043 0.8179  0.7054 0.8195  0.7066 0.8197  0.7078 0.8305  0.7089 0.8311  0.7101 0.8250  0.7112 0.8413  0.7124 0.8465  0.7135 0.8453  0.7147 0.8644  0.7159 0.8649  0.7170 0.8603  0.7182 0.8766  0.7193 0.8792  0.7205 0.8785  0.7216 0.8934  0.7228 0.8989  0.7240 0.8959  0.7251 0.9098  0.7263 0.9135  0.7274 0.9070  0.7286 0.9214  0.7297 0.9295  0.7309 0.9313  0.7321 0.9428  0.7332 0.9431  0.7344 0.9431  0.7355 0.9568  0.7367 0.9573  0.7378 0.9569  0.7390 0.9714  0.7402 0.9707  0.7413 0.9742  0.7425 0.9918  0.7436 0.9930  0.7448 0.9894  0.7459 0.9985  0.7471 1.0048  0.7483 1.0084  0.7494 1.0170  0.7506 1.0191  0.7517 1.0218  0.7529 1.0323  0.7541 1.0422  0.7552 1.0469  0.7564 1.0508  0.7575 1.0536  0.7587 1.0612  0.7598 1.0688  0.7610 1.0760  0.7622 1.0857  0.7633 1.0892  0.7645 1.0937  0.7656 1.1035  0.7668 1.1102  0.7679 1.1143  0.7691 1.1201  0.7703 1.1278  0.7714 1.1372  0.7726 1.1422  0.7737 1.1486  0.7749 1.1586  0.7760 1.1648  0.7772 1.1692  0.7784 1.1757  0.7795 1.1843  0.7807 1.1899  0.7818 1.1935  0.7830 1.2034  0.7841 1.2136  0.7853 1.2218  0.7865 1.2301  0.7876 1.2364  0.7888 1.2437  0.7899 1.2545  0.7911 1.2612  0.7922 1.2663  0.7934 1.2750  0.7946 1.2827  0.7957 1.2894  0.7969 1.2941  0.7980 1.3038  0.7992 1.3160  0.8003 1.3224  0.8015 1.3266  0.8027 1.3334  0.8038 1.3448  0.8050 1.3553  0.8061 1.3651  0.8073 1.3774  0.8084 1.3830  0.8096 1.3884  0.8108 1.3970  0.8119 1.4067  0.8131 1.4201  0.8142 1.4120  0.8154 1.4189  0.8166 1.4454  0.8177 1.4440  0.8189 1.4555  0.8200 1.4755  0.8212 1.4654  0.8223 1.4769  0.8235 1.5029  0.8247 1.4942  0.8258 1.5053  0.8270 1.5325  0.8281 1.5274  0.8293 1.5345  0.8304 1.5572  0.8316 1.5517  0.8328 1.5626  0.8339 1.5889  0.8351 1.5835  0.8362 1.5949  0.8374 1.6236  0.8385 1.6168  0.8397 1.6273  0.8409 1.6542  0.8420 1.6466  0.8432 1.6591  0.8443 1.6884  0.8455 1.6821  0.8466 1.6925  0.8478 1.7211  0.8490 1.7133  0.8501 1.7256  0.8513 1.7587  0.8524 1.7512  0.8536 1.7603  0.8547 1.7891  0.8559 1.7827  0.8571 1.7960  0.8582 1.8285  0.8594 1.8209  0.8605 1.8339  0.8617 1.8507  0.8628 1.8586  0.8640 1.8851  0.8652 1.8816  0.8663 1.8942  0.8675 1.9205  0.8686 1.9264  0.8698 1.9415  0.8709 1.9626  0.8721 1.9755  0.8733 1.9856  0.8744 1.9982  0.8756 2.0201  0.8767 2.0283  0.8779 2.0400  0.8791 2.0606  0.8802 2.0692  0.8814 2.0812  0.8825 2.0922  0.8837 2.1201  0.8848 2.1408  0.8860 2.1473  0.8872 2.1637  0.8883 2.1808  0.8895 2.1969  0.8906 2.2144  0.8918 2.2303  0.8929 2.2444  0.8941 2.2590  0.8953 2.2794  0.8964 2.2988  0.8976 2.3161  0.8987 2.3351  0.8999 2.3509  0.9010 2.3674  0.9022 2.3885  0.9034 2.4106  0.9045 2.4286  0.9057 2.4459  0.9068 2.4667  0.9080 2.4893  0.9091 2.5010  0.9103 2.5261  0.9115 2.5478  0.9126 2.5706  0.9138 2.5918  0.9149 2.6042  0.9161 2.6383  0.9172 2.6587  0.9184 2.6774  0.9196 2.6996  0.9207 2.7223  0.9219 2.7422  0.9230 2.7588  0.9242 2.7848  0.9253 2.8199  0.9265 2.8114  0.9277 2.8205  0.9288 2.9451  0.9300 2.9846  0.9311 2.9288  0.9323 3.0685  0.9334 3.1206  0.9346 3.0053  0.9358 3.0669  0.9369 3.1377  0.9381 3.1054  0.9392 3.1226  0.9404 3.2784  0.9416 3.2775  0.9427 3.2182  0.9439 3.4287  0.9450 3.4138  0.9462 3.3028  0.9473 3.5245  0.9485 3.5409  0.9497 3.4357  0.9508 3.4907  0.9520 3.5451  0.9531 3.6426  0.9543 3.6892  0.9554 3.6827  0.9566 3.7023  0.9578 3.8180  0.9589 3.8542  0.9601 3.7746  0.9612 3.8524  0.9624 3.9708  0.9635 4.0355  0.9647 4.2349  0.9659 4.1937  0.9670 4.0181  0.9682 4.1532  0.9693 3.9487  0.9705 5.3571  0.9716 5.6031  0.9728 4.2978  0.9740 4.2794  0.9751 5.1387  0.9763 5.3680  0.9774 4.7052  0.9786 4.8236  0.9797 4.7489  0.9809 4.9848  0.9821 5.8368  0.9832 5.7463 
/

%L=13
\color{B13}
%\plot 0.5156 -1.2062  0.5469 -0.9693  0.5781 -0.7731  0.6094 -0.5966  0.6406 -0.4271  0.6719 -0.2577  0.7031 -0.0823  0.7344 0.1060  0.7656 0.3147  0.7969 0.5534  0.8281 0.8343  0.8594 1.1773  0.8906 1.6143  0.9219 2.2032 /
\multiput {\large$\cdot$} at 0.0150 -0.0418  0.0159 -0.0377  0.0168 -0.0349  0.0178 -0.0327  0.0187 -0.0310  0.0196 -0.0296  0.0205 -0.0285  0.0214 -0.0275  0.0223 -0.0267  0.0232 -0.0260  0.0241 -0.0254  0.0250 -0.0249  0.0259 -0.0245  0.0269 -0.0240  0.0278 -0.0236  0.0287 -0.0233  0.0296 -0.0229  0.0305 -0.0226  0.0314 -0.0224  0.0323 -0.0222  0.0332 -0.0219  0.0341 -0.0216  0.0350 -0.0215  0.0360 -0.0212  0.0369 -0.0210  0.0378 -0.0208  0.0387 -0.0207  0.0396 -0.0205  0.0405 -0.0203  0.0414 -0.0202  0.0423 -0.0200  0.0432 -0.0198  0.0442 -0.0197  0.0451 -0.0195  0.0460 -0.0194  0.0469 -0.0193  0.0478 -0.0191  0.0487 -0.0190  0.0496 -0.0188  0.0505 -0.0186  0.0514 -0.0186  0.0523 -0.0183  0.0533 -0.0182  0.0542 -0.0180  0.0551 -0.0178  0.0560 -0.0176  0.0569 -0.0175  0.0578 -0.0174  0.0587 -0.0173  0.0596 -0.0171  0.0605 -0.0170  0.0614 -0.0169  0.0624 -0.0169  0.0633 -0.0166  0.0642 -0.0164  0.0651 -0.0162  0.0660 -0.0159  0.0669 -0.0158  0.0678 -0.0158  0.0687 -0.0156  0.0696 -0.0153  0.0706 -0.0152  0.0715 -0.0151  0.0724 -0.0149  0.0733 -0.0148  0.0742 -0.0146  0.0751 -0.0145  0.0760 -0.0142  0.0769 -0.0140  0.0778 -0.0140  0.0787 -0.0138  0.0797 -0.0135  0.0806 -0.0134  0.0815 -0.0132  0.0824 -0.0130  0.0833 -0.0128  0.0842 -0.0126  0.0851 -0.0124  0.0860 -0.0121  0.0869 -0.0119  0.0878 -0.0119  0.0888 -0.0118  0.0897 -0.0115  0.0906 -0.0113  0.0915 -0.0111  0.0924 -0.0108  0.0933 -0.0106  0.0942 -0.0105  0.0951 -0.0102  0.0960 -0.0102  0.0970 -0.0099  0.0979 -0.0096  0.0988 -0.0095  0.0997 -0.0093  0.1006 -0.0091  0.1015 -0.0088  0.1024 -0.0087  0.1033 -0.0085  0.1042 -0.0081  0.1051 -0.0080  0.1061 -0.0079  0.1070 -0.0076  0.1079 -0.0072  0.1088 -0.0070  0.1097 -0.0070  0.1106 -0.0068  0.1115 -0.0065  0.1124 -0.0062  0.1133 -0.0058  0.1142 -0.0057  0.1152 -0.0055  0.1161 -0.0054  0.1170 -0.0053  0.1179 -0.0050  0.1188 -0.0048  0.1197 -0.0045  0.1206 -0.0043  0.1215 -0.0043  0.1224 -0.0040  0.1234 -0.0036  0.1243 -0.0035  0.1252 -0.0033  0.1261 -0.0028  0.1270 -0.0026  0.1279 -0.0027  0.1288 -0.0025  0.1297 -0.0019  0.1306 -0.0016  0.1315 -0.0015  0.1325 -0.0014  0.1334 -0.0006  0.1343 -0.0006  0.1352 -0.0007  0.1361 -0.0000  0.1370 0.0002  0.1379 0.0003  0.1388 0.0007  0.1397 0.0009  0.1406 0.0010  0.1416 0.0011  0.1425 0.0014  0.1434 0.0019  0.1443 0.0021  0.1452 0.0025  0.1461 0.0031  0.1470 0.0029  0.1479 0.0030  0.1488 0.0033  0.1497 0.0035  0.1507 0.0040  0.1516 0.0041  0.1525 0.0042  0.1534 0.0044  0.1543 0.0049  0.1552 0.0054  0.1561 0.0055  0.1570 0.0059  0.1579 0.0063  0.1589 0.0062  0.1598 0.0067  0.1607 0.0073  0.1616 0.0069  0.1625 0.0068  0.1634 0.0075  0.1643 0.0081  0.1652 0.0084  0.1661 0.0086  0.1670 0.0088  0.1680 0.0092  0.1689 0.0096  0.1698 0.0098  0.1707 0.0098  0.1716 0.0104  0.1725 0.0107  0.1734 0.0109  0.1743 0.0112  0.1752 0.0114  0.1761 0.0121  0.1771 0.0120  0.1780 0.0126  0.1789 0.0130  0.1798 0.0131  0.1807 0.0134  0.1816 0.0134  0.1825 0.0139  0.1834 0.0147  0.1843 0.0151  0.1853 0.0150  0.1862 0.0152  0.1871 0.0158  0.1880 0.0161  0.1889 0.0164  0.1898 0.0167  0.1907 0.0172  0.1916 0.0177  0.1925 0.0179  0.1934 0.0179  0.1944 0.0183  0.1953 0.0185  0.1962 0.0190  0.1971 0.0195  0.1980 0.0194  0.1989 0.0200  0.1998 0.0203  0.2007 0.0207  0.2016 0.0211  0.2025 0.0212  0.2035 0.0218  0.2044 0.0223  0.2053 0.0226  0.2062 0.0231  0.2071 0.0233  0.2080 0.0235  0.2089 0.0235  0.2098 0.0241  0.2107 0.0250  0.2117 0.0253  0.2126 0.0262  0.2135 0.0264  0.2144 0.0261  0.2153 0.0263  0.2162 0.0268  0.2171 0.0275  0.2180 0.0276  0.2189 0.0277  0.2198 0.0283  0.2208 0.0286  0.2217 0.0297  0.2226 0.0305  0.2235 0.0298  0.2244 0.0303  0.2253 0.0308  0.2262 0.0311  0.2271 0.0319  0.2280 0.0319  0.2289 0.0319  0.2299 0.0324  0.2308 0.0330  0.2317 0.0339  0.2326 0.0350  0.2335 0.0349  0.2344 0.0345  0.2353 0.0350  0.2362 0.0356  0.2371 0.0358  0.2381 0.0365  0.2390 0.0374  0.2399 0.0381  0.2408 0.0383  0.2417 0.0387  0.2426 0.0393  0.2435 0.0396  0.2444 0.0401  0.2453 0.0406  0.2462 0.0408  0.2472 0.0409  0.2481 0.0411  0.2490 0.0422  0.2499 0.0427  0.2508 0.0424  0.2517 0.0432  0.2526 0.0444  0.2535 0.0445  0.2544 0.0451  0.2553 0.0457  0.2563 0.0462  0.2572 0.0466  0.2581 0.0466  0.2590 0.0470  0.2599 0.0477  0.2608 0.0482  0.2617 0.0487  0.2626 0.0491  0.2635 0.0500  0.2645 0.0507  0.2654 0.0507  0.2663 0.0514  0.2672 0.0521  0.2681 0.0522  0.2690 0.0532  0.2699 0.0541  0.2708 0.0541  0.2717 0.0544  0.2726 0.0551  0.2736 0.0556  0.2745 0.0559  0.2754 0.0563  0.2763 0.0567  0.2772 0.0571  0.2781 0.0581  0.2790 0.0585  0.2799 0.0585  0.2808 0.0589  0.2817 0.0594  0.2827 0.0602  0.2836 0.0608  0.2845 0.0606  0.2854 0.0616  0.2863 0.0631  0.2872 0.0630  0.2881 0.0632  0.2890 0.0637  0.2899 0.0644  0.2909 0.0656  0.2918 0.0657  0.2927 0.0658  0.2936 0.0662  0.2945 0.0668  0.2954 0.0676  0.2963 0.0680  0.2972 0.0687  0.2981 0.0699  0.2990 0.0709  0.3000 0.0709  0.3009 0.0713  0.3018 0.0720  0.3027 0.0729  0.3036 0.0738  0.3045 0.0742  0.3054 0.0742  0.3063 0.0753  0.3072 0.0762  0.3081 0.0768  0.3091 0.0772  0.3100 0.0764  0.3109 0.0770  0.3118 0.0783  0.3127 0.0786  0.3136 0.0793  0.3145 0.0808  0.3154 0.0821  0.3163 0.0830  0.3173 0.0833  0.3182 0.0835  0.3191 0.0838  0.3200 0.0845  0.3209 0.0855  0.3218 0.0861  0.3227 0.0865  0.3236 0.0877  0.3245 0.0883  0.3254 0.0881  0.3264 0.0890  0.3273 0.0902  0.3282 0.0904  0.3291 0.0910  0.3300 0.0918  0.3309 0.0919  0.3318 0.0928  0.3327 0.0941  0.3336 0.0947  0.3345 0.0947  0.3355 0.0955  0.3364 0.0963  0.3373 0.0969  0.3382 0.0980  0.3391 0.0983  0.3400 0.0991  0.3409 0.1007  0.3418 0.1006  0.3427 0.1013  0.3437 0.1025  0.3446 0.1026  0.3455 0.1036  0.3464 0.1040  0.3473 0.1047  0.3482 0.1056  0.3491 0.1064  0.3500 0.1071  0.3509 0.1076  0.3518 0.1084  0.3528 0.1094  0.3537 0.1108  0.3546 0.1113  0.3555 0.1119  0.3564 0.1119  0.3573 0.1134  0.3582 0.1146  0.3591 0.1143  0.3600 0.1157  0.3609 0.1158  0.3619 0.1165  0.3628 0.1179  0.3637 0.1180  0.3646 0.1189  0.3655 0.1209  0.3664 0.1215  0.3673 0.1216  0.3682 0.1218  0.3691 0.1236  0.3701 0.1247  0.3710 0.1251  0.3719 0.1262  0.3728 0.1258  0.3737 0.1271  0.3746 0.1288  0.3755 0.1293  0.3764 0.1306  0.3773 0.1311  0.3782 0.1317  0.3792 0.1325  0.3801 0.1324  0.3810 0.1343  0.3819 0.1358  0.3828 0.1364  0.3837 0.1378  0.3846 0.1377  0.3855 0.1381  0.3864 0.1391  0.3873 0.1396  0.3883 0.1410  0.3892 0.1423  0.3901 0.1434  0.3910 0.1441  0.3919 0.1454  0.3928 0.1455  0.3937 0.1465  0.3946 0.1488  0.3955 0.1504  0.3964 0.1502  0.3974 0.1497  0.3983 0.1512  0.3992 0.1524  0.4001 0.1537  0.4010 0.1545  0.4019 0.1548  0.4028 0.1562  0.4037 0.1576  0.4046 0.1578  0.4056 0.1584  0.4065 0.1596  0.4074 0.1604  0.4083 0.1612  0.4092 0.1629  0.4101 0.1638  0.4110 0.1647  0.4119 0.1657  0.4128 0.1656  0.4137 0.1675  0.4147 0.1686  0.4156 0.1688  0.4165 0.1705  0.4174 0.1712  0.4183 0.1718  0.4192 0.1736  0.4201 0.1742  0.4210 0.1747  0.4219 0.1759  0.4228 0.1768  0.4238 0.1779  0.4247 0.1791  0.4256 0.1803  0.4265 0.1821  0.4274 0.1832  0.4283 0.1828  0.4292 0.1841  0.4301 0.1860  0.4310 0.1864  0.4320 0.1877  0.4329 0.1894  0.4338 0.1902  0.4347 0.1901  0.4356 0.1916  0.4365 0.1939  0.4374 0.1949  0.4383 0.1962  0.4392 0.1973  0.4401 0.1989  0.4411 0.1989  0.4420 0.1998  0.4429 0.2014  0.4438 0.2025  0.4447 0.2041  0.4456 0.2041  0.4465 0.2057  0.4474 0.2079  0.4483 0.2079  0.4492 0.2085  0.4502 0.2095  0.4511 0.2121  0.4520 0.2141  0.4529 0.2146  0.4538 0.2157  0.4547 0.2168  0.4556 0.2174  0.4565 0.2186  0.4574 0.2204  0.4584 0.2202  0.4593 0.2215  0.4602 0.2242  0.4611 0.2246  0.4620 0.2256  0.4629 0.2278  0.4638 0.2288  0.4647 0.2264  0.4656 0.2285  0.4665 0.2329  0.4675 0.2339  0.4684 0.2353  0.4693 0.2362  0.4702 0.2378  0.4711 0.2378  0.4720 0.2386  0.4729 0.2408  0.4738 0.2415  0.4747 0.2432  0.4756 0.2457  0.4766 0.2479  0.4775 0.2489  0.4784 0.2495  0.4793 0.2484  0.4802 0.2518  0.4811 0.2552  0.4820 0.2515  0.4829 0.2539  0.4838 0.2557  0.4848 0.2621  0.4857 0.2653  0.4866 0.2597  0.4875 0.2612  0.4884 0.2631  0.4893 0.2646  0.4902 0.2660  0.4911 0.2671  0.4920 0.2662  0.4929 0.2691  0.4939 0.2689  0.4948 0.2726  0.4957 0.2773  0.4966 0.2712  0.4975 0.2764  0.4984 0.2810  0.4993 0.2797  0.5002 0.2779  0.5011 0.2833  0.5020 0.2867  0.5030 0.2842  0.5039 0.2880  0.5048 0.2850  0.5057 0.2852  0.5066 0.2910  0.5075 0.2932  0.5084 0.2952  0.5093 0.2967  0.5102 0.2968  0.5112 0.2994  0.5121 0.3023  0.5130 0.3036  0.5139 0.3065  0.5148 0.3086  0.5157 0.3042  0.5166 0.3061  0.5175 0.3096  0.5184 0.3124  0.5193 0.3172  0.5203 0.3159  0.5212 0.3162  0.5221 0.3173  0.5230 0.3185  0.5239 0.3194  0.5248 0.3186  0.5257 0.3219  0.5266 0.3256  0.5275 0.3278  0.5284 0.3314  0.5294 0.3318  0.5303 0.3328  0.5312 0.3380  0.5321 0.3398  0.5330 0.3350  0.5339 0.3394  0.5348 0.3475  0.5357 0.3383  0.5366 0.3401  0.5376 0.3473  0.5385 0.3376  0.5394 0.3675  0.5403 0.3732  0.5412 0.3497  0.5421 0.3563  0.5430 0.3555  0.5439 0.3541  0.5448 0.3578  0.5457 0.3647  0.5467 0.3647  0.5476 0.3624  0.5485 0.3629  0.5494 0.3733  0.5503 0.3855  0.5512 0.3806  0.5521 0.3743  0.5530 0.3770  0.5539 0.3777  0.5548 0.3774  0.5558 0.3754  0.5567 0.3797  0.5576 0.3839  0.5585 0.3826  0.5594 0.3884  0.5603 0.3942  0.5612 0.3922  0.5621 0.3973  0.5630 0.4019  0.5640 0.4000  0.5649 0.4001  0.5658 0.4014  0.5667 0.4022  0.5676 0.4022  0.5685 0.4073  0.5694 0.4059  0.5703 0.4054  0.5712 0.4105  0.5721 0.4158  0.5731 0.4169  0.5740 0.4191  0.5749 0.4147  0.5758 0.4150  0.5767 0.4267  0.5776 0.4301  0.5785 0.4294  0.5794 0.4322  0.5803 0.4362  0.5812 0.4341  0.5822 0.4359  0.5831 0.4412  0.5840 0.4435  0.5849 0.4440  0.5858 0.4461  0.5867 0.4495  0.5876 0.4468  0.5885 0.4488  0.5894 0.4538  0.5904 0.4597  0.5913 0.4557  0.5922 0.4550  0.5931 0.4648  0.5940 0.4646  0.5949 0.4665  0.5958 0.4673  0.5967 0.4701  0.5976 0.4794  0.5985 0.4802  0.5995 0.4741  0.6004 0.4786  0.6013 0.4763  0.6022 0.4848  0.6031 0.4864  0.6040 0.4903  0.6049 0.5057  0.6058 0.5254  0.6067 0.5192  0.6076 0.4947  0.6086 0.5001  0.6095 0.5026  0.6104 0.5011  0.6113 0.5042  0.6122 0.5136  0.6131 0.5152  0.6140 0.5110  0.6149 0.5159  0.6158 0.5236  0.6168 0.5238  0.6177 0.5228  0.6186 0.5280  0.6195 0.5238  0.6204 0.5244  0.6213 0.5364  0.6222 0.5335  0.6231 0.5389  0.6240 0.5451  0.6249 0.5415  0.6259 0.5446  0.6268 0.5464  0.6277 0.5496  0.6286 0.5543  0.6295 0.5559  0.6304 0.5589  0.6313 0.5568  0.6322 0.5605  0.6331 0.5698  0.6340 0.5725  0.6350 0.5716  0.6359 0.5840  0.6368 0.5895  0.6377 0.5799  0.6386 0.5816  0.6395 0.5845  0.6404 0.5884  0.6413 0.5826  0.6422 0.5858  0.6431 0.5997  0.6441 0.5999  0.6450 0.6036  0.6459 0.6062  0.6468 0.6075  0.6477 0.6122  0.6486 0.6165  0.6495 0.6073  0.6504 0.6108  0.6513 0.6214  0.6523 0.6233  0.6532 0.6203  0.6541 0.6389  0.6550 0.6485  0.6559 0.6344  0.6568 0.6411  0.6577 0.6416  0.6586 0.6525  0.6595 0.6560  0.6604 0.6768  0.6614 0.6637  0.6623 0.6334  0.6632 0.6551  0.6641 0.6648  0.6650 0.6651  0.6659 0.6623  0.6668 0.6616  0.6677 0.6772  0.6686 0.6861  0.6695 0.6806  0.6705 0.6840  0.6714 0.6881  0.6723 0.6903  0.6732 0.6900  0.6741 0.6955  0.6750 0.7024  0.6759 0.7005  0.6768 0.7058  0.6777 0.7064  0.6787 0.7094  0.6796 0.7138  0.6805 0.7096  0.6814 0.7088  0.6823 0.7365  0.6832 0.7483  0.6841 0.7227  0.6850 0.7344  0.6859 0.7295  0.6868 0.7298  0.6878 0.7508  0.6887 0.7475  0.6896 0.7454  0.6905 0.7560  0.6914 0.7659  0.6923 0.7441  0.6932 0.7769  0.6941 0.7974  0.6950 0.7692  0.6959 0.7768  0.6969 0.7842  0.6978 0.7849  0.6987 0.7487  0.6996 0.7550  0.7005 0.8039  0.7014 0.8021  0.7023 0.7975  0.7032 0.8239  0.7041 0.8280  0.7051 0.8292  0.7060 0.8346  0.7069 0.8402  0.7078 0.9483  0.7087 0.9141  0.7096 0.8110  0.7105 0.8420  0.7114 0.8340  0.7123 0.8273  0.7132 0.8435  0.7142 0.8538  0.7151 0.8502  0.7160 0.8558  0.7169 0.8691  0.7178 0.8685  0.7187 0.8640  0.7196 0.8923  0.7205 0.9002  0.7214 0.8754  0.7223 0.8803  0.7233 0.8845  0.7242 0.9066  0.7251 0.9068  0.7260 0.8916  0.7269 0.8985  0.7278 0.9079  0.7287 0.9194  0.7296 0.9256  0.7305 0.9211  0.7315 0.9206  0.7324 0.9339  0.7333 0.9314  0.7342 0.9371  0.7351 0.9458  0.7360 0.9467  0.7369 0.9410  0.7378 0.9460  0.7387 0.9750  0.7396 0.9767  0.7406 0.9711  0.7415 0.9732  0.7424 0.9762  0.7433 0.9862  0.7442 0.9930  0.7451 0.9830  0.7460 0.9901  0.7469 0.9995  0.7478 1.0033  0.7487 1.0078  0.7497 1.0109  0.7506 1.0265  0.7515 1.0195  0.7524 1.0148  0.7533 1.0564  0.7542 1.0659  0.7551 1.0460  0.7560 1.0543  0.7569 1.0529  0.7579 1.0603  0.7588 1.0719  0.7597 1.0636  0.7606 1.0675  0.7615 1.0798  0.7624 1.0877  0.7633 1.0849  0.7642 1.0880  0.7651 1.0885  0.7660 1.0860  0.7670 1.1113  0.7679 1.1237  0.7688 1.1299  0.7697 1.1310  0.7706 1.1357  0.7715 1.1317  0.7724 1.1344  0.7733 1.1459  0.7742 1.1579  0.7751 1.1473  0.7761 1.1289  0.7770 1.1597  0.7779 1.1847  0.7788 1.1888  0.7797 1.1939  0.7806 1.1835  0.7815 1.1816  0.7824 1.1879  0.7833 1.2499  0.7843 1.2630  0.7852 1.2131  0.7861 1.2290  0.7870 1.2190  0.7879 1.2021  0.7888 1.2250  0.7897 1.2540  0.7906 1.2623  0.7915 1.2679  0.7924 1.2655  0.7934 1.2632  0.7943 1.2640  0.7952 1.2764  0.7961 1.2991  0.7970 1.2998  0.7979 1.3076  0.7988 1.2801  0.7997 1.2842  0.8006 1.3264  0.8015 1.3259  0.8025 1.3450  0.8034 1.3207  0.8043 1.3749  0.8052 1.4074  0.8061 1.3578  0.8070 1.3828  0.8079 1.3418  0.8088 1.3412  0.8097 1.3992  0.8107 1.3980  0.8116 1.4035  0.8125 1.3555  0.8134 1.3662  0.8143 1.4391  0.8152 1.4385  0.8161 1.4290  0.8170 1.4482  0.8179 1.3613  0.8188 1.3696  0.8198 1.4742  0.8207 1.4553  0.8216 1.4678  0.8225 1.3741  0.8234 1.4307  0.8243 2.2952  0.8252 2.1369  0.8261 1.4056  0.8270 1.5338  0.8279 1.5113  0.8289 1.5249  0.8298 1.5618  0.8307 1.5638  0.8316 1.5606  0.8325 1.5612  0.8334 1.6095  0.8343 1.6264  0.8352 1.6062  0.8361 1.6358  0.8371 1.6368  0.8380 1.5974  0.8389 1.6160  0.8398 1.6468  0.8407 1.6230  0.8416 1.6225  0.8425 1.7172  0.8434 1.7374  0.8443 1.6777  0.8452 1.6958  0.8462 1.6800  0.8471 1.7200  0.8480 1.7557  0.8489 1.7250  0.8498 1.7071  0.8507 1.7274  0.8516 1.7460  0.8525 1.7354  0.8534 1.7497  0.8543 1.7825  0.8553 1.7675  0.8562 1.7775  0.8571 1.7860  0.8580 1.8145  0.8589 1.8656  0.8598 1.8610  0.8607 1.8563  0.8616 1.9650  0.8625 1.9704  0.8635 1.8542  0.8644 1.8773  0.8653 1.9085  0.8662 1.9745  0.8671 1.9482  0.8680 1.8829  0.8689 1.9545  0.8698 1.9947  0.8707 1.9572  0.8716 1.9753  0.8726 1.9698  0.8735 1.9637  0.8744 2.0117  0.8753 2.0260  0.8762 2.0088  0.8771 2.0088  0.8780 2.0503  0.8789 2.0195  0.8798 2.0253  0.8807 2.0937  0.8817 2.0621  0.8826 2.3100  0.8835 2.3388  0.8844 2.0857  0.8853 2.0893  0.8862 2.1450  0.8871 2.1732  0.8880 2.1845  0.8889 2.1839  0.8898 2.1869  0.8908 2.2152  0.8917 2.2078  0.8926 2.2185  0.8935 2.3454  0.8944 2.4126  0.8953 2.2798  0.8962 2.2733  0.8971 2.3318  0.8980 2.2998  0.8990 2.4210  0.8999 2.4779  0.9008 2.3579  0.9017 2.3632  0.9026 2.3938  0.9035 2.4026  0.9044 2.4263  0.9053 2.4585  0.9062 2.3894  0.9071 2.4026  0.9081 2.5013  0.9090 2.5177  0.9099 2.4950  0.9108 2.5990  0.9117 2.5905  0.9126 2.5098  0.9135 2.6235  0.9144 2.5497  0.9153 2.5822  0.9162 2.5628  0.9172 2.5584  0.9181 2.7153  0.9190 2.5389  0.9199 2.5851  0.9208 2.7890  0.9217 2.6898  0.9226 3.1238  0.9235 3.0605  0.9244 2.7190  0.9254 2.6099  0.9263 2.6123  0.9272 2.7470  0.9281 4.4398  0.9290 4.4608  0.9299 2.7968  0.9308 3.0379  0.9317 3.0487  0.9326 2.8199  0.9335 2.8113  0.9345 3.0563  0.9354 3.2627  0.9363 3.1916  0.9372 3.1095  0.9381 3.2372  0.9390 3.1013  0.9399 3.1718  0.9408 3.0525  0.9417 3.1906  0.9426 3.4353  
 /

%L=14
\color{B14}
%\plot 0.5156 -1.2062  0.5469 -0.9693  0.5781 -0.7731  0.6094 -0.5966  0.6406 -0.4271  0.6719 -0.2577  0.7031 -0.0823  0.7344 0.1060  0.7656 0.3147  0.7969 0.5534  0.8281 0.8343  0.8594 1.1773  0.8906 1.6143  0.9219 2.2032 /
\multiput {\large$\cdot$} at 0.0120 -0.0332  0.0128 -0.0300  0.0135 -0.0277  0.0142 -0.0260  0.0149 -0.0247  0.0157 -0.0236  0.0164 -0.0227  0.0171 -0.0219  0.0179 -0.0213  0.0186 -0.0207  0.0193 -0.0202  0.0200 -0.0198  0.0208 -0.0194  0.0215 -0.0191  0.0222 -0.0188  0.0230 -0.0185  0.0237 -0.0182  0.0244 -0.0180  0.0251 -0.0178  0.0259 -0.0176  0.0266 -0.0174  0.0273 -0.0173  0.0281 -0.0171  0.0288 -0.0170  0.0295 -0.0168  0.0302 -0.0167  0.0310 -0.0165  0.0317 -0.0164  0.0324 -0.0163  0.0332 -0.0161  0.0339 -0.0159  0.0346 -0.0159  0.0353 -0.0159  0.0361 -0.0157  0.0368 -0.0156  0.0375 -0.0155  0.0383 -0.0154  0.0390 -0.0152  0.0397 -0.0152  0.0405 -0.0152  0.0412 -0.0150  0.0419 -0.0150  0.0426 -0.0148  0.0434 -0.0147  0.0441 -0.0147  0.0448 -0.0145  0.0456 -0.0144  0.0463 -0.0143  0.0470 -0.0142  0.0477 -0.0142  0.0485 -0.0142  0.0492 -0.0141  0.0499 -0.0140  0.0507 -0.0138  0.0514 -0.0136  0.0521 -0.0135  0.0528 -0.0134  0.0536 -0.0134  0.0543 -0.0132  0.0550 -0.0130  0.0558 -0.0131  0.0565 -0.0130  0.0572 -0.0128  0.0579 -0.0127  0.0587 -0.0127  0.0594 -0.0126  0.0601 -0.0123  0.0609 -0.0121  0.0616 -0.0121  0.0623 -0.0121  0.0630 -0.0120  0.0638 -0.0118  0.0645 -0.0116  0.0652 -0.0116  0.0660 -0.0115  0.0667 -0.0113  0.0674 -0.0113  0.0681 -0.0111  0.0689 -0.0109  0.0696 -0.0108  0.0703 -0.0106  0.0711 -0.0105  0.0718 -0.0104  0.0725 -0.0104  0.0733 -0.0102  0.0740 -0.0102  0.0747 -0.0103  0.0754 -0.0099  0.0762 -0.0096  0.0769 -0.0095  0.0776 -0.0093  0.0784 -0.0092  0.0791 -0.0091  0.0798 -0.0091  0.0805 -0.0088  0.0813 -0.0085  0.0820 -0.0087  0.0827 -0.0086  0.0835 -0.0084  0.0842 -0.0081  0.0849 -0.0081  0.0856 -0.0081  0.0864 -0.0078  0.0871 -0.0076  0.0878 -0.0074  0.0886 -0.0073  0.0893 -0.0074  0.0900 -0.0073  0.0907 -0.0070  0.0915 -0.0069  0.0922 -0.0068  0.0929 -0.0067  0.0937 -0.0066  0.0944 -0.0062  0.0951 -0.0060  0.0958 -0.0057  0.0966 -0.0057  0.0973 -0.0059  0.0980 -0.0058  0.0988 -0.0054  0.0995 -0.0051  0.1002 -0.0052  0.1009 -0.0050  0.1017 -0.0048  0.1024 -0.0047  0.1031 -0.0046  0.1039 -0.0044  0.1046 -0.0042  0.1053 -0.0041  0.1060 -0.0040  0.1068 -0.0038  0.1075 -0.0036  0.1082 -0.0034  0.1090 -0.0035  0.1097 -0.0031  0.1104 -0.0030  0.1112 -0.0029  0.1119 -0.0025  0.1126 -0.0024  0.1133 -0.0023  0.1141 -0.0021  0.1148 -0.0020  0.1155 -0.0018  0.1163 -0.0017  0.1170 -0.0015  0.1177 -0.0014  0.1184 -0.0011  0.1192 -0.0008  0.1199 -0.0007  0.1206 -0.0007  0.1214 -0.0003  0.1221 -0.0001  0.1228 -0.0002  0.1235 -0.0001  0.1243 0.0003  0.1250 0.0006  0.1257 0.0007  0.1265 0.0011  0.1272 0.0013  0.1279 0.0012  0.1286 0.0011  0.1294 0.0013  0.1301 0.0015  0.1308 0.0017  0.1316 0.0018  0.1323 0.0020  0.1330 0.0023  0.1337 0.0024  0.1345 0.0028  0.1352 0.0031  0.1359 0.0031  0.1367 0.0032  0.1374 0.0036  0.1381 0.0039  0.1388 0.0041  0.1396 0.0043  0.1403 0.0044  0.1410 0.0046  0.1418 0.0050  0.1425 0.0047  0.1432 0.0046  0.1440 0.0051  0.1447 0.0056  0.1454 0.0058  0.1461 0.0056  0.1469 0.0058  0.1476 0.0061  0.1483 0.0062  0.1491 0.0063  0.1498 0.0071  0.1505 0.0072  0.1512 0.0069  0.1520 0.0074  0.1527 0.0074  0.1534 0.0077  0.1542 0.0082  0.1549 0.0080  0.1556 0.0085  0.1563 0.0086  0.1571 0.0085  0.1578 0.0091  0.1585 0.0091  0.1593 0.0091  0.1600 0.0093  0.1607 0.0096  0.1614 0.0098  0.1622 0.0104  0.1629 0.0107  0.1636 0.0106  0.1644 0.0109  0.1651 0.0109  0.1658 0.0106  0.1665 0.0112  0.1673 0.0119  0.1680 0.0120  0.1687 0.0119  0.1695 0.0122  0.1702 0.0127  0.1709 0.0130  0.1716 0.0129  0.1724 0.0132  0.1731 0.0137  0.1738 0.0135  0.1746 0.0136  0.1753 0.0145  0.1760 0.0149  0.1767 0.0148  0.1775 0.0156  0.1782 0.0158  0.1789 0.0161  0.1797 0.0161  0.1804 0.0158  0.1811 0.0159  0.1819 0.0163  0.1826 0.0170  0.1833 0.0171  0.1840 0.0173  0.1848 0.0179  0.1855 0.0180  0.1862 0.0180  0.1870 0.0190  0.1877 0.0191  0.1884 0.0187  0.1891 0.0189  0.1899 0.0195  0.1906 0.0198  0.1913 0.0201  0.1921 0.0210  0.1928 0.0206  0.1935 0.0202  0.1942 0.0209  0.1950 0.0216  0.1957 0.0219  0.1964 0.0220  0.1972 0.0219  0.1979 0.0223  0.1986 0.0230  0.1993 0.0230  0.2001 0.0231  0.2008 0.0232  0.2015 0.0235  0.2023 0.0245  0.2030 0.0244  0.2037 0.0242  0.2044 0.0248  0.2052 0.0251  0.2059 0.0255  0.2066 0.0258  0.2074 0.0259  0.2081 0.0267  0.2088 0.0269  0.2095 0.0264  0.2103 0.0268  0.2110 0.0265  0.2117 0.0268  0.2125 0.0277  0.2132 0.0275  0.2139 0.0283  0.2147 0.0281  0.2154 0.0279  0.2161 0.0286  0.2168 0.0290  0.2176 0.0294  0.2183 0.0297  0.2190 0.0303  0.2198 0.0304  0.2205 0.0303  0.2212 0.0310  0.2219 0.0314  0.2227 0.0313  0.2234 0.0319  0.2241 0.0324  0.2249 0.0329  0.2256 0.0338  0.2263 0.0336  0.2270 0.0336  0.2278 0.0340  0.2285 0.0338  0.2292 0.0346  0.2300 0.0355  0.2307 0.0360  0.2314 0.0359  0.2321 0.0360  0.2329 0.0361  0.2336 0.0353  0.2343 0.0357  0.2351 0.0367  0.2358 0.0372  0.2365 0.0379  0.2372 0.0389  0.2380 0.0393  0.2387 0.0391  0.2394 0.0398  0.2402 0.0401  0.2409 0.0401  0.2416 0.0403  0.2423 0.0410  0.2431 0.0421  0.2438 0.0414  0.2445 0.0408  0.2453 0.0412  0.2460 0.0420  0.2467 0.0424  0.2474 0.0421  0.2482 0.0431  0.2489 0.0437  0.2496 0.0443  0.2504 0.0454  0.2511 0.0449  0.2518 0.0447  0.2526 0.0461  0.2533 0.0471  0.2540 0.0468  0.2547 0.0469  0.2555 0.0469  0.2562 0.0476  0.2569 0.0469  0.2577 0.0468  0.2584 0.0493  0.2591 0.0482  0.2598 0.0481  0.2606 0.0508  0.2613 0.0517  0.2620 0.0512  0.2628 0.0519  0.2635 0.0514  0.2642 0.0506  0.2649 0.0515  0.2657 0.0531  0.2664 0.0532  0.2671 0.0525  0.2679 0.0537  0.2686 0.0547  0.2693 0.0553  0.2700 0.0557  0.2708 0.0567  0.2715 0.0569  0.2722 0.0562  0.2730 0.0563  0.2737 0.0572  0.2744 0.0583  0.2751 0.0575  0.2759 0.0565  0.2766 0.0596  0.2773 0.0589  0.2781 0.0573  0.2788 0.0589  0.2795 0.0603  0.2802 0.0613  0.2810 0.0609  0.2817 0.0608  0.2824 0.0614  0.2832 0.0628  0.2839 0.0632  0.2846 0.0624  0.2853 0.0629  0.2861 0.0640  0.2868 0.0637  0.2875 0.0646  0.2883 0.0644  0.2890 0.0638  0.2897 0.0660  0.2905 0.0661  0.2912 0.0663  0.2919 0.0674  0.2926 0.0682  0.2934 0.0682  0.2941 0.0681  0.2948 0.0684  0.2956 0.0689  0.2963 0.0695  0.2970 0.0700  0.2977 0.0707  0.2985 0.0702  0.2992 0.0712  0.2999 0.0724  0.3007 0.0721  0.3014 0.0731  0.3021 0.0742  0.3028 0.0746  0.3036 0.0762  0.3043 0.0759  0.3050 0.0743  0.3058 0.0745  0.3065 0.0763  0.3072 0.0769  0.3079 0.0758  0.3087 0.0773  0.3094 0.0797  0.3101 0.0793  0.3109 0.0788  0.3116 0.0798  0.3123 0.0801  0.3130 0.0807  0.3138 0.0810  0.3145 0.0812  0.3152 0.0816  0.3160 0.0830  0.3167 0.0834  0.3174 0.0832  0.3181 0.0843  0.3189 0.0836  0.3196 0.0840  0.3203 0.0873  0.3211 0.0866  0.3218 0.0850  0.3225 0.0863  0.3233 0.0865  0.3240 0.0877  0.3247 0.0890  0.3254 0.0890  0.3262 0.0902  0.3269 0.0900  0.3276 0.0906  0.3284 0.0923  0.3291 0.0906  0.3298 0.0918  0.3305 0.0929  0.3313 0.0915  0.3320 0.0926  0.3327 0.0934  0.3335 0.0940  0.3342 0.0954  0.3349 0.0966  0.3356 0.0972  0.3364 0.0979  0.3371 0.1000  0.3378 0.1006  0.3386 0.0988  0.3393 0.0982  0.3400 0.0992  0.3407 0.1003  0.3415 0.1005  0.3422 0.1023  0.3429 0.1040  0.3437 0.1022  0.3444 0.1038  0.3451 0.1059  0.3458 0.1045  0.3466 0.1047  0.3473 0.1054  0.3480 0.1058  0.3488 0.1065  0.3495 0.1050  0.3502 0.1056  0.3509 0.1054  0.3517 0.1056  0.3524 0.1094  0.3531 0.1103  0.3539 0.1095  0.3546 0.1106  0.3553 0.1123  0.3560 0.1138  0.3568 0.1146  0.3575 0.1155  0.3582 0.1155  0.3590 0.1141  0.3597 0.1146  0.3604 0.1134  0.3612 0.1142  0.3619 0.1189  0.3626 0.1191  0.3633 0.1194  0.3641 0.1218  0.3648 0.1203  0.3655 0.1194  0.3663 0.1203  0.3670 0.1215  0.3677 0.1219  0.3684 0.1226  0.3692 0.1252  0.3699 0.1279  0.3706 0.1263  0.3714 0.1263  0.3721 0.1280  0.3728 0.1272  0.3735 0.1286  0.3743 0.1297  0.3750 0.1302  0.3757 0.1293  0.3765 0.1309  0.3772 0.1308  0.3779 0.1312  0.3786 0.1328  0.3794 0.1351  0.3801 0.1381  0.3808 0.1363  0.3816 0.1356  0.3823 0.1349  0.3830 0.1348  0.3837 0.1383  0.3845 0.1403  0.3852 0.1415  0.3859 0.1422  0.3867 0.1419  0.3874 0.1418  0.3881 0.1404  0.3888 0.1421  0.3896 0.1420  0.3903 0.1419  0.3910 0.1453  0.3918 0.1480  0.3925 0.1477  0.3932 0.1492  0.3940 0.1498  0.3947 0.1494  0.3954 0.1518  0.3961 0.1501  0.3969 0.1498  0.3976 0.1527  0.3983 0.1542  0.3991 0.1511  0.3998 0.1503  0.4005 0.1569  0.4012 0.1572  0.4020 0.1582  0.4027 0.1593  0.4034 0.1559  0.4042 0.1534  0.4049 0.1561  0.4056 0.1578  0.4063 0.1576  0.4071 0.1622  0.4078 0.1621  0.4085 0.1595  0.4093 0.1616  0.4100 0.1624  0.4107 0.1611  0.4114 0.1668  0.4122 0.1683  0.4129 0.1651  0.4136 0.1657  0.4144 0.1669  0.4151 0.1704  0.4158 0.1723  0.4165 0.1743  0.4173 0.1793  0.4180 0.1761  0.4187 0.1750  0.4195 0.1766  0.4202 0.1762  0.4209 0.1761  0.4216 0.1749  0.4224 0.1766  0.4231 0.1769  0.4238 0.1796  0.4246 0.1815  0.4253 0.1802  0.4260 0.1790  0.4267 0.1800  0.4275 0.1815  0.4282 0.1846  0.4289 0.1860  0.4297 0.1856  0.4304 0.1852  0.4311 0.1879  0.4319 0.1927  0.4326 0.1905  0.4333 0.1901  0.4340 0.1909  0.4348 0.1949  0.4355 0.1938  0.4362 0.1906  0.4370 0.1934  0.4377 0.1929  0.4384 0.1929  0.4391 0.1980  0.4399 0.1990  0.4406 0.1980  0.4413 0.1991  0.4421 0.1989  0.4428 0.1985  0.4435 0.1999  0.4442 0.2047  0.4450 0.2064  0.4457 0.2069  0.4464 0.2077  0.4472 0.2070  0.4479 0.2071  0.4486 0.2035  0.4493 0.2043  0.4501 0.2147  0.4508 0.2135  0.4515 0.2083  0.4523 0.2109  0.4530 0.2134  0.4537 0.2155  0.4544 0.2149  0.4552 0.2158  0.4559 0.2081  0.4566 0.2194  0.4574 0.2308  0.4581 0.2234  0.4588 0.2163  0.4595 0.2150  0.4603 0.2287  0.4610 0.2299  0.4617 0.2160  0.4625 0.2143  0.4632 0.2261  0.4639 0.2318  0.4647 0.2331  0.4654 0.2352  0.4661 0.2329  0.4668 0.2308  0.4676 0.2289  0.4683 0.2292  0.4690 0.2352  0.4698 0.2354  0.4705 0.2284  0.4712 0.2279  0.4719 0.2424  0.4727 0.2617  0.4734 0.2521  0.4741 0.2430  0.4749 0.2501  0.4756 0.2399  0.4763 0.2411  0.4770 0.2484  0.4778 0.2506  0.4785 0.2449  0.4792 0.2447  0.4800 0.2518  0.4807 0.2516  0.4814 0.2466  0.4821 0.2492  0.4829 0.2542  0.4836 0.2511  0.4843 0.2550  0.4851 0.2557  0.4858 0.2603  0.4865 0.2664  0.4872 0.2638  0.4880 0.2599  0.4887 0.2587  0.4894 0.2640  0.4902 0.2639  0.4909 0.2673  0.4916 0.2709  0.4923 0.2647  0.4931 0.2660  0.4938 0.2713  0.4945 0.2765  0.4953 0.2774  0.4960 0.2741  0.4967 0.2740  0.4974 0.2641  0.4982 0.2670  0.4989 0.2827  0.4996 0.2835  0.5004 0.2802  0.5011 0.2824  0.5018 0.2847  0.5026 0.2854  0.5033 0.2870  0.5040 0.2889  0.5047 0.2860  0.5055 0.2852  0.5062 0.2919  0.5069 0.2953  0.5077 0.2922  0.5084 0.2897  0.5091 0.2956  0.5098 0.2983  0.5106 0.2978  0.5113 0.2970  0.5120 0.2896  0.5128 0.2947  0.5135 0.2992  0.5142 0.3023  0.5149 0.3097  0.5157 0.3073  0.5164 0.3104  0.5171 0.3148  0.5179 0.3142  0.5186 0.3139  0.5193 0.3148  0.5200 0.3144  0.5208 0.3137  0.5215 0.3188  0.5222 0.3212  0.5230 0.3190  0.5237 0.3198  0.5244 0.3047  0.5251 0.3035  0.5259 0.3166  0.5266 0.3220  0.5273 0.3315  0.5281 0.3312  0.5288 0.3337  0.5295 0.3372  0.5302 0.3342  0.5310 0.3359  0.5317 0.3353  0.5324 0.3368  0.5332 0.3414  0.5339 0.3393  0.5346 0.3404  0.5353 0.3453  0.5361 0.3459  0.5368 0.3447  0.5375 0.3454  0.5383 0.3436  0.5390 0.3437  0.5397 0.3554  0.5405 0.3550  0.5412 0.3513  0.5419 0.3609  0.5426 0.3413  0.5434 0.3391  0.5441 0.3645  0.5448 0.3676  0.5456 0.3681  0.5463 0.3639  0.5470 0.3606  0.5477 0.3611  0.5485 0.3685  0.5492 0.3722  0.5499 0.3703  0.5507 0.3730  0.5514 0.3739  0.5521 0.3741  0.5528 0.3687  0.5536 0.3745  0.5543 0.3887  0.5550 0.3897  0.5558 0.3614  0.5565 0.3690  0.5572 0.3918  0.5579 0.3823  0.5587 0.3886  0.5594 0.3941  0.5601 0.3975  0.5609 0.3986  0.5616 0.3927  0.5623 0.3788  0.5630 0.3819  0.5638 0.4255  0.5645 0.4243  0.5652 0.3979  0.5660 0.4078  0.5667 0.3831  0.5674 0.3841  0.5681 0.4153  0.5689 0.4138  0.5696 0.4156  0.5703 0.4123  0.5711 0.4128  0.5718 0.4183  0.5725 0.4166  0.5733 0.4186  0.5740 0.4198  0.5747 0.4211  0.5754 0.4238  0.5762 0.4285  0.5769 0.4312  0.5776 0.4313  0.5784 0.4375  0.5791 0.4103  0.5798 0.4125  0.5805 0.4421  0.5813 0.4353  0.5820 0.4371  0.5827 0.4433  0.5835 0.4422  0.5842 0.4426  0.5849 0.4429  0.5856 0.4462  0.5864 0.4640  0.5871 0.4136  0.5878 0.4097  0.5886 0.4615  0.5893 0.4552  0.5900 0.4588  0.5907 0.4632  0.5915 0.4621  0.5922 0.4656  0.5929 0.4710  0.5937 0.4638  0.5944 0.4636  0.5951 0.4727  0.5958 0.4848  0.5966 0.4009  0.5973 0.3988  0.5980 0.4873  0.5988 0.4850  0.5995 0.4880  0.6002 0.4847  0.6009 0.4829  0.6017 0.4872  0.6024 0.4957  0.6031 0.4718  0.6039 0.4637  0.6046 0.4686  0.6053 0.4452  0.6060 0.4647  0.6068 0.5093  0.6075 0.4948  0.6082 0.4470  0.6090 0.4028  0.6097 0.3482  0.6104 0.1524  0.6112 1.4469  0.6119 1.5681  0.6126 0.3648  0.6133 0.5171  0.6141 0.5200  0.6148 0.5202  0.6155 0.5180  0.6163 0.5174  0.6170 0.5213  0.6177 0.5252  0.6184 0.5219  0.6192 0.5415  0.6199 0.5455  0.6206 0.5275  0.6214 0.5344  0.6221 0.5377  0.6228 0.5393  0.6235 0.5461  0.6243 0.5509  0.6250 0.5456  0.6257 0.5498  0.6265 0.5416  0.6272 0.5290  0.6279 0.5471  0.6286 0.5449  0.6294 0.5995  0.6301 0.6049  0.6308 0.5476  0.6316 0.5630  0.6323 0.5687  0.6330 0.5687  0.6337 0.5675  0.6345 0.5673  0.6352 0.5868  0.6359 0.5915  0.6367 0.5735  0.6374 0.5797  0.6381 0.5891  0.6388 0.6049  0.6396 0.6042  0.6403 0.5821  0.6410 0.5819  0.6418 0.5944  0.6425 0.5945  0.6432 0.5952  0.6440 0.6090  0.6447 0.6111  0.6454 0.6028  0.6461 0.5986  0.6469 0.6080  0.6476 0.6099  0.6483 0.6094  0.6491 0.6151  0.6498 0.6171  0.6505 0.6223  0.6512 0.6205  0.6520 0.6217  0.6527 0.6276  0.6534 0.6102  0.6542 0.6136  0.6549 0.6391  0.6556 0.6439  0.6563 0.6425  0.6571 0.6340  0.6578 0.6367  0.6585 0.6546  0.6593 0.6534  0.6600 0.6511  0.6607 0.6611  0.6614 0.6630  0.6622 0.6379  0.6629 0.6440  0.6636 0.6712  0.6644 0.6684  0.6651 0.6644  0.6658 0.6803  0.6665 0.6817  0.6673 0.6666  0.6680 0.6540  0.6687 0.6809  0.6695 0.8204  0.6702 0.7885  0.6709 0.6669  0.6716 0.6850  0.6724 0.6960  0.6731 0.6917  0.6738 0.6955  0.6746 0.7094  0.6753 0.7000  0.6760 0.6923  0.6767 0.7293  0.6775 0.7243  0.6782 0.7038  0.6789 0.7191  0.6797 0.7212  0.6804 0.7143  0.6811 0.7118  0.6819 0.7250  0.6826 0.7264  0.6833 0.7286  0.6840 0.7366  0.6848 0.7389  0.6855 0.7362  0.6862 0.7437  0.6870 0.7591  0.6877 0.7492  0.6884 0.7521  0.6891 0.7642  0.6899 0.7540  0.6906 0.7558  0.6913 0.7650  0.6921 0.7570  0.6928 0.7537  0.6935 0.7590  0.6942 0.7749  0.6950 0.7741  0.6957 0.7598  0.6964 0.7762  0.6972 0.7810  0.6979 0.7827  0.6986 0.7990  0.6993 0.8006  0.7001 0.7999  0.7008 0.7924  0.7015 0.7899  0.7023 0.8052  0.7030 0.8097  0.7037 0.8035  0.7044 0.8096  0.7052 0.8187  0.7059 0.8107  0.7066 0.8169  0.7074 0.8305  0.7081 0.8236  0.7088 0.8248  0.7095 0.8347  0.7103 0.8343  0.7110 0.8374  0.7117 0.8376  0.7125 0.8432  0.7132 0.8510  0.7139 0.8491  0.7147 0.8473  0.7154 0.8690  0.7161 0.8735  0.7168 0.8534  0.7176 0.8596  0.7183 0.8747  0.7190 0.8796  0.7198 0.8712  0.7205 0.8808  0.7212 0.8937  0.7219 0.8840  0.7227 0.8725  0.7234 0.8713  0.7241 0.8888  0.7249 0.9072  0.7256 0.9084  0.7263 0.9108  0.7270 0.9138  0.7278 0.9147  0.7285 0.9107  0.7292 0.9369  0.7300 0.9429  0.7307 0.8999  0.7314 0.9106  0.7321 0.9420  0.7329 0.9490  0.7336 0.9521  0.7343 0.9464  0.7351 0.9466  0.7358 0.9233  0.7365 1.0559  0.7372 1.1414  0.7380 1.0075  0.7387 0.9552  0.7394 0.9713  0.7402 0.9807  0.7409 0.9818  0.7416 0.9798  0.7423 0.9835  0.7431 0.9909  0.7438 0.9830  0.7445 0.9893  0.7453 1.0007  0.7460 1.0058  0.7467 0.9995  0.7474 1.0018  0.7482 1.0031  0.7489 1.0086  0.7496 1.0274  0.7504 1.0297  0.7511 1.0277  0.7518 1.0199  0.7526 1.0123  0.7533 1.0297  0.7540 1.0530  0.7547 1.0433  0.7555 1.0474  0.7562 1.0625  0.7569 1.0486  0.7577 1.0582  0.7584 1.0766  0.7591 1.0571  0.7598 1.0672  0.7606 1.0832  0.7613 1.0673  0.7620 1.0722  0.7628 1.0924  0.7635 1.0921  0.7642 1.0966  0.7649 1.0990  0.7657 1.1044  0.7664 1.1148  0.7671 1.1138  0.7679 1.1198  0.7686 1.1108  0.7693 1.0987  0.7700 1.1266  0.7708 1.1468  0.7715 1.1368  0.7722 1.1343  0.7730 1.1296  0.7737 1.1810  0.7744 1.1792  0.7751 1.1441  0.7759 1.1680  0.7766 1.1833  0.7773 1.1613  0.7781 1.1405  0.7788 1.1821  0.7795 1.1914  0.7802 1.1866  0.7810 1.1884  0.7817 1.1991  0.7824 1.2024  0.7832 1.1758  0.7839 1.1977  0.7846 1.2297  0.7853 1.2104  0.7861 1.2156  0.7868 1.2463  0.7875 1.3116  0.7883 1.2923  0.7890 1.2348  0.7897 1.2652  0.7905 1.2405  0.7912 1.2446  0.7919 1.2757  0.7926 1.2723  0.7934 1.2830  0.7941 1.2779  0.7948 1.2769  0.7956 1.2760  0.7963 1.2851  0.7970 1.3045  0.7977 1.3078  0.7985 1.3122  0.7992 1.3161  0.7999 1.3666  0.8007 1.3705  0.8014 1.3038  0.8021 1.3011  0.8028 1.3315  0.8036 1.3506  0.8043 1.3608  0.8050 1.3287  0.8058 1.3395  0.8065 1.3812  0.8072 1.3813  0.8079 1.3831  0.8087 1.3862  0.8094 1.3642  0.8101 1.3856  0.8109 1.4430  0.8116 1.4301  0.8123 1.4105  0.8130 1.4230  0.8138 1.3848  0.8145 1.3913  0.8152 1.4911  0.8160 1.4859  0.8167 1.4439  0.8174 1.4624  0.8181 1.4474  0.8189 1.4338  0.8196 1.4540  0.8203 1.4779  0.8211 1.4932  0.8218 1.4513  0.8225 1.4528  0.8233 1.5067  0.8240 1.5120  0.8247 1.5118  0.8254 1.5191  0.8262 1.5362  0.8269 1.4833  0.8276 1.4820  0.8284 1.5465  0.8291 1.5526  0.8298 1.5111  0.8305 1.5264  0.8313 1.5736  0.8320 1.5662  0.8327 1.5883  0.8335 1.5249  0.8342 1.5291  0.8349 1.6371  0.8356 1.6223  0.8364 1.6028  0.8371 1.6215  0.8378 1.5638  0.8386 1.4677  0.8393 1.5375  0.8400 1.6543  0.8407 1.6664  0.8415 1.6562  0.8422 1.6821  0.8429 1.5029  0.8437 1.4986  0.8444 1.7270  0.8451 1.6903  0.8458 1.6859  0.8466 1.4921  0.8473 3.1867  0.8480 3.2000  0.8488 1.4963  0.8495 1.7016  0.8502 1.7119  0.8509 1.7413  0.8517 1.7391  0.8524 1.7428  0.8531 1.7530  0.8539 1.7725  0.8546 1.7928  0.8553 1.8114  0.8560 1.7873  0.8568 1.7571  0.8575 1.7732  0.8582 1.8212  0.8590 1.8611  0.8597 1.9346  0.8604 1.8624  0.8612 1.7967  0.8619 1.8478  0.8626 1.8792  0.8633 1.8738  0.8641 1.8198  0.8648 1.8747  0.8655 1.9065  0.8663 1.9367  0.8670 1.8302  0.8677 1.8210  0.8684 1.9635  0.8692 1.9699  0.8699 1.9209  0.8706 1.9326  0.8714 1.9189  0.8721 1.9193  0.8728 1.9979  0.8735 2.0327  0.8743 1.9262  0.8750 2.1192  0.8757 2.2217  0.8765 1.9931  0.8772 1.9593  0.8779 1.9533  0.8786 2.0415  0.8794 2.1022  0.8801 2.0229  0.8808 1.8981  0.8816 2.0092  0.8823 2.1341  0.8830 2.0954  0.8837 2.1203  0.8845 2.1402  0.8852 1.9943  0.8859 2.0247  0.8867 2.1955  0.8874 2.1458  0.8881 1.9824  0.8888 2.0946  0.8896 2.0632  0.8903 2.0125  0.8910 2.1490  0.8918 2.2238  0.8925 2.0186  0.8932 1.9587  0.8940 2.2423  0.8947 2.3481  0.8954 1.7957  0.8961 1.8074  0.8969 2.4352  0.8976 1.6396  0.8983 5.6093  0.8991 5.8668  
 /

%L=15
\color{B15}
%\plot 0.5156 -1.2062  0.5469 -0.9693  0.5781 -0.7731  0.6094 -0.5966  0.6406 -0.4271  0.6719 -0.2577  0.7031 -0.0823  0.7344 0.1060  0.7656 0.3147  0.7969 0.5534  0.8281 0.8343  0.8594 1.1773  0.8906 1.6143  0.9219 2.2032 /
\multiput {\large$\cdot$} at 0.0098 -0.0268  0.0104 -0.0243  0.0110 -0.0224  0.0116 -0.0210  0.0121 -0.0199  0.0127 -0.0190  0.0133 -0.0183  0.0139 -0.0177  0.0145 -0.0172  0.0151 -0.0167  0.0157 -0.0163  0.0163 -0.0160  0.0169 -0.0157  0.0175 -0.0154  0.0181 -0.0152  0.0187 -0.0149  0.0193 -0.0148  0.0199 -0.0146  0.0204 -0.0144  0.0210 -0.0142  0.0216 -0.0141  0.0222 -0.0140  0.0228 -0.0139  0.0234 -0.0137  0.0240 -0.0136  0.0246 -0.0135  0.0252 -0.0134  0.0258 -0.0133  0.0264 -0.0132  0.0270 -0.0131  0.0276 -0.0131  0.0281 -0.0130  0.0287 -0.0129  0.0293 -0.0128  0.0299 -0.0127  0.0305 -0.0127  0.0311 -0.0126  0.0317 -0.0126  0.0323 -0.0124  0.0329 -0.0123  0.0335 -0.0124  0.0341 -0.0123  0.0347 -0.0122  0.0353 -0.0122  0.0359 -0.0121  0.0364 -0.0120  0.0370 -0.0119  0.0376 -0.0118  0.0382 -0.0120  0.0388 -0.0119  0.0394 -0.0117  0.0400 -0.0117  0.0406 -0.0116  0.0412 -0.0115  0.0418 -0.0115  0.0424 -0.0114  0.0430 -0.0113  0.0436 -0.0113  0.0441 -0.0112  0.0447 -0.0111  0.0453 -0.0112  0.0459 -0.0109  0.0465 -0.0107  0.0471 -0.0108  0.0477 -0.0108  0.0483 -0.0106  0.0489 -0.0106  0.0495 -0.0105  0.0501 -0.0104  0.0507 -0.0102  0.0513 -0.0103  0.0519 -0.0102  0.0524 -0.0100  0.0530 -0.0100  0.0536 -0.0098  0.0542 -0.0097  0.0548 -0.0097  0.0554 -0.0096  0.0560 -0.0097  0.0566 -0.0097  0.0572 -0.0097  0.0578 -0.0095  0.0584 -0.0092  0.0590 -0.0092  0.0596 -0.0092  0.0601 -0.0092  0.0607 -0.0091  0.0613 -0.0090  0.0619 -0.0089  0.0625 -0.0087  0.0631 -0.0086  0.0637 -0.0085  0.0643 -0.0084  0.0649 -0.0082  0.0655 -0.0083  0.0661 -0.0083  0.0667 -0.0081  0.0673 -0.0080  0.0679 -0.0078  0.0684 -0.0076  0.0690 -0.0076  0.0696 -0.0077  0.0702 -0.0077  0.0708 -0.0075  0.0714 -0.0072  0.0720 -0.0071  0.0726 -0.0071  0.0732 -0.0072  0.0738 -0.0073  0.0744 -0.0070  0.0750 -0.0068  0.0756 -0.0067  0.0761 -0.0068  0.0767 -0.0068  0.0773 -0.0067  0.0779 -0.0065  0.0785 -0.0063  0.0791 -0.0062  0.0797 -0.0061  0.0803 -0.0059  0.0809 -0.0059  0.0815 -0.0060  0.0821 -0.0058  0.0827 -0.0056  0.0833 -0.0053  0.0839 -0.0052  0.0844 -0.0052  0.0850 -0.0050  0.0856 -0.0050  0.0862 -0.0050  0.0868 -0.0050  0.0874 -0.0049  0.0880 -0.0046  0.0886 -0.0046  0.0892 -0.0045  0.0898 -0.0044  0.0904 -0.0040  0.0910 -0.0041  0.0916 -0.0043  0.0921 -0.0041  0.0927 -0.0038  0.0933 -0.0039  0.0939 -0.0036  0.0945 -0.0031  0.0951 -0.0033  0.0957 -0.0034  0.0963 -0.0033  0.0969 -0.0030  0.0975 -0.0030  0.0981 -0.0028  0.0987 -0.0026  0.0993 -0.0024  0.0999 -0.0024  0.1004 -0.0024  0.1010 -0.0021  0.1016 -0.0023  0.1022 -0.0024  0.1028 -0.0021  0.1034 -0.0018  0.1040 -0.0018  0.1046 -0.0014  0.1052 -0.0014  0.1058 -0.0016  0.1064 -0.0011  0.1070 -0.0008  0.1076 -0.0011  0.1081 -0.0011  0.1087 -0.0009  0.1093 -0.0005  0.1099 -0.0004  0.1105 0.0001  0.1111 0.0001  0.1117 -0.0003  0.1123 0.0000  0.1129 0.0001  0.1135 -0.0000  0.1141 0.0002  0.1147 0.0008  0.1153 0.0010  0.1159 0.0006  0.1164 0.0008  0.1170 0.0011  0.1176 0.0012  0.1182 0.0015  0.1188 0.0018  0.1194 0.0017  0.1200 0.0018  0.1206 0.0016  0.1212 0.0018  0.1218 0.0026  0.1224 0.0027  0.1230 0.0024  0.1236 0.0022  0.1241 0.0025  0.1247 0.0026  0.1253 0.0027  0.1259 0.0033  0.1265 0.0039  0.1271 0.0039  0.1277 0.0034  0.1283 0.0038  0.1289 0.0042  0.1295 0.0042  0.1301 0.0038  0.1307 0.0040  0.1313 0.0046  0.1319 0.0044  0.1324 0.0049  0.1330 0.0052  0.1336 0.0046  0.1342 0.0050  0.1348 0.0057  0.1354 0.0052  0.1360 0.0050  0.1366 0.0053  0.1372 0.0057  0.1378 0.0058  0.1384 0.0058  0.1390 0.0063  0.1396 0.0065  0.1401 0.0066  0.1407 0.0067  0.1413 0.0067  0.1419 0.0065  0.1425 0.0069  0.1431 0.0071  0.1437 0.0070  0.1443 0.0073  0.1449 0.0073  0.1455 0.0077  0.1461 0.0080  0.1467 0.0077  0.1473 0.0080  0.1479 0.0087  0.1484 0.0082  0.1490 0.0079  0.1496 0.0083  0.1502 0.0088  0.1508 0.0093  0.1514 0.0095  0.1520 0.0095  0.1526 0.0097  0.1532 0.0097  0.1538 0.0101  0.1544 0.0098  0.1550 0.0098  0.1556 0.0109  0.1561 0.0108  0.1567 0.0113  0.1573 0.0109  0.1579 0.0112  0.1585 0.0118  0.1591 0.0115  0.1597 0.0117  0.1603 0.0116  0.1609 0.0117  0.1615 0.0118  0.1621 0.0123  0.1627 0.0128  0.1633 0.0127  0.1639 0.0131  0.1644 0.0140  0.1650 0.0135  0.1656 0.0125  0.1662 0.0132  0.1668 0.0141  0.1674 0.0142  0.1680 0.0141  0.1686 0.0145  0.1692 0.0153  0.1698 0.0151  0.1704 0.0149  0.1710 0.0145  0.1716 0.0147  0.1721 0.0154  0.1727 0.0153  0.1733 0.0161  0.1739 0.0166  0.1745 0.0158  0.1751 0.0160  0.1757 0.0168  0.1763 0.0175  0.1769 0.0174  0.1775 0.0164  0.1781 0.0163  0.1787 0.0174  0.1793 0.0178  0.1799 0.0177  0.1804 0.0172  0.1810 0.0174  0.1816 0.0188  0.1822 0.0185  0.1828 0.0189  0.1834 0.0193  0.1840 0.0193  0.1846 0.0195  0.1852 0.0199  0.1858 0.0203  0.1864 0.0199  0.1870 0.0203  0.1876 0.0205  0.1881 0.0198  0.1887 0.0203  0.1893 0.0223  0.1899 0.0210  0.1905 0.0212  0.1911 0.0230  0.1917 0.0211  0.1923 0.0211  0.1929 0.0227  0.1935 0.0233  0.1941 0.0239  0.1947 0.0232  0.1953 0.0232  0.1959 0.0229  0.1964 0.0221  0.1970 0.0230  0.1976 0.0231  0.1982 0.0238  0.1988 0.0247  0.1994 0.0249  0.2000 0.0251  0.2006 0.0257  0.2012 0.0253  0.2018 0.0254  0.2024 0.0264  0.2030 0.0257  0.2036 0.0258  0.2041 0.0263  0.2047 0.0278  0.2053 0.0280  0.2059 0.0252  0.2065 0.0265  0.2071 0.0281  0.2077 0.0279  0.2083 0.0284  0.2089 0.0289  0.2095 0.0291  0.2101 0.0283  0.2107 0.0279  0.2113 0.0303  0.2119 0.0300  0.2124 0.0287  0.2130 0.0304  0.2136 0.0293  0.2142 0.0300  0.2148 0.0316  0.2154 0.0314  0.2160 0.0316  0.2166 0.0315  0.2172 0.0313  0.2178 0.0318  0.2184 0.0321  0.2190 0.0322  0.2196 0.0321  0.2201 0.0327  0.2207 0.0325  0.2213 0.0318  0.2219 0.0327  0.2225 0.0327  0.2231 0.0335  0.2237 0.0339  0.2243 0.0338  0.2249 0.0339  0.2255 0.0345  0.2261 0.0348  0.2267 0.0359  0.2273 0.0369  0.2279 0.0360  0.2284 0.0356  0.2290 0.0356  0.2296 0.0375  0.2302 0.0387  0.2308 0.0379  0.2314 0.0369  0.2320 0.0373  0.2326 0.0380  0.2332 0.0384  0.2338 0.0385  0.2344 0.0386  0.2350 0.0383  0.2356 0.0390  0.2361 0.0401  0.2367 0.0393  0.2373 0.0409  0.2379 0.0415  0.2385 0.0411  0.2391 0.0419  0.2397 0.0414  0.2403 0.0405  0.2409 0.0411  0.2415 0.0418  0.2421 0.0415  0.2427 0.0419  0.2433 0.0420  0.2439 0.0417  0.2444 0.0420  0.2450 0.0447  0.2456 0.0451  0.2462 0.0435  0.2468 0.0440  0.2474 0.0438  0.2480 0.0437  0.2486 0.0438  0.2492 0.0448  0.2498 0.0456  0.2504 0.0458  0.2510 0.0469  0.2516 0.0474  0.2521 0.0470  0.2527 0.0473  0.2533 0.0484  0.2539 0.0484  0.2545 0.0473  0.2551 0.0478  0.2557 0.0492  0.2563 0.0505  0.2569 0.0501  0.2575 0.0498  0.2581 0.0502  0.2587 0.0506  0.2593 0.0505  0.2599 0.0503  0.2604 0.0519  0.2610 0.0523  0.2616 0.0518  0.2622 0.0525  0.2628 0.0520  0.2634 0.0533  0.2640 0.0541  0.2646 0.0529  0.2652 0.0534  0.2658 0.0538  0.2664 0.0529  0.2670 0.0541  0.2676 0.0554  0.2681 0.0544  0.2687 0.0548  0.2693 0.0562  0.2699 0.0564  0.2705 0.0557  0.2711 0.0576  0.2717 0.0589  0.2723 0.0583  0.2729 0.0579  0.2735 0.0577  0.2741 0.0598  0.2747 0.0599  0.2753 0.0601  0.2759 0.0590  0.2764 0.0580  0.2770 0.0601  0.2776 0.0601  0.2782 0.0614  0.2788 0.0613  0.2794 0.0618  0.2800 0.0627  0.2806 0.0628  0.2812 0.0627  0.2818 0.0626  0.2824 0.0636  0.2830 0.0629  0.2836 0.0630  0.2841 0.0633  0.2847 0.0637  0.2853 0.0642  0.2859 0.0643  0.2865 0.0653  0.2871 0.0664  0.2877 0.0660  0.2883 0.0662  0.2889 0.0681  0.2895 0.0683  0.2901 0.0684  0.2907 0.0680  0.2913 0.0684  0.2919 0.0694  0.2924 0.0692  0.2930 0.0686  0.2936 0.0688  0.2942 0.0697  0.2948 0.0703  0.2954 0.0712  0.2960 0.0717  0.2966 0.0710  0.2972 0.0715  0.2978 0.0717  0.2984 0.0725  0.2990 0.0739  0.2996 0.0731  0.3001 0.0730  0.3007 0.0750  0.3013 0.0754  0.3019 0.0744  0.3025 0.0746  0.3031 0.0750  0.3037 0.0757  0.3043 0.0768  0.3049 0.0768  0.3055 0.0761  0.3061 0.0766  0.3067 0.0766  0.3073 0.0769  0.3079 0.0779  0.3084 0.0787  0.3090 0.0782  0.3096 0.0789  0.3102 0.0811  0.3108 0.0805  0.3114 0.0799  0.3120 0.0806  0.3126 0.0811  0.3132 0.0821  0.3138 0.0827  0.3144 0.0823  0.3150 0.0835  0.3156 0.0857  0.3161 0.0852  0.3167 0.0837  0.3173 0.0844  0.3179 0.0848  0.3185 0.0862  0.3191 0.0871  0.3197 0.0871  0.3203 0.0866  0.3209 0.0873  0.3215 0.0873  0.3221 0.0881  0.3227 0.0891  0.3233 0.0887  0.3239 0.0894  0.3244 0.0895  0.3250 0.0902  0.3256 0.0899  0.3262 0.0922  0.3268 0.0941  0.3274 0.0921  0.3280 0.0915  0.3286 0.0926  0.3292 0.0935  0.3298 0.0948  0.3304 0.0948  0.3310 0.0954  0.3316 0.0946  0.3321 0.0934  0.3327 0.0946  0.3333 0.0964  0.3339 0.0993  0.3345 0.0992  0.3351 0.0983  0.3357 0.0980  0.3363 0.0981  0.3369 0.0979  0.3375 0.0967  0.3381 0.0978  0.3387 0.1008  0.3393 0.1022  0.3399 0.1013  0.3404 0.1036  0.3410 0.1013  0.3416 0.0972  0.3422 0.1000  0.3428 0.1008  0.3434 0.0997  0.3440 0.1007  0.3446 0.1039  0.3452 0.1066  0.3458 0.1061  0.3464 0.1066  0.3470 0.1072  0.3476 0.1092  0.3481 0.1082  0.3487 0.1047  0.3493 0.1088  0.3499 0.1097  0.3505 0.1070  0.3511 0.1077  0.3517 0.1091  0.3523 0.1109  0.3529 0.1111  0.3535 0.1113  0.3541 0.1129  0.3547 0.1110  0.3553 0.1128  0.3559 0.1166  0.3564 0.1144  0.3570 0.1154  0.3576 0.1158  0.3582 0.1125  0.3588 0.1133  0.3594 0.1164  0.3600 0.1171  0.3606 0.1155  0.3612 0.1146  0.3618 0.1141  0.3624 0.1170  0.3630 0.1172  0.3636 0.1181  0.3641 0.1220  0.3647 0.1203  0.3653 0.1206  0.3659 0.1209  0.3665 0.1220  0.3671 0.1254  0.3677 0.1232  0.3683 0.1241  0.3689 0.1223  0.3695 0.1235  0.3701 0.1300  0.3707 0.1287  0.3713 0.1230  0.3719 0.1222  0.3724 0.1282  0.3730 0.1334  0.3736 0.1323  0.3742 0.1277  0.3748 0.1262  0.3754 0.1315  0.3760 0.1339  0.3766 0.1328  0.3772 0.1309  0.3778 0.1335  0.3784 0.1370  0.3790 0.1323  0.3796 0.1327  0.3801 0.1354  0.3807 0.1316  0.3813 0.1333  0.3819 0.1404  0.3825 0.1375  0.3831 0.1374  0.3837 0.1425  0.3843 0.1388  0.3849 0.1387  0.3855 0.1407  0.3861 0.1375  0.3867 0.1418  0.3873 0.1426  0.3879 0.1371  0.3884 0.1385  0.3890 0.1437  0.3896 0.1458  0.3902 0.1427  0.3908 0.1415  0.3914 0.1480  0.3920 0.1483  0.3926 0.1453  0.3932 0.1477  0.3938 0.1506  0.3944 0.1521  0.3950 0.1549  0.3956 0.1524  0.3961 0.1490  0.3967 0.1508  0.3973 0.1530  0.3979 0.1558  0.3985 0.1526  0.3991 0.1500  0.3997 0.1545  0.4003 0.1577  0.4009 0.1589  0.4015 0.1561  0.4021 0.1563  0.4027 0.1573  0.4033 0.1556  0.4039 0.1574  0.4044 0.1597  0.4050 0.1575  0.4056 0.1595  0.4062 0.1601  0.4068 0.1630  0.4074 0.1662  0.4080 0.1615  0.4086 0.1645  0.4092 0.1662  0.4098 0.1657  0.4104 0.1638  0.4110 0.1623  0.4116 0.1646  0.4121 0.1702  0.4127 0.1640  0.4133 0.1596  0.4139 0.1650  0.4145 0.1690  0.4151 0.1728  0.4157 0.1705  0.4163 0.1756  0.4169 0.1797  0.4175 0.1765  0.4181 0.1759  0.4187 0.1759  0.4193 0.1731  0.4199 0.1731  0.4204 0.1828  0.4210 0.1880  0.4216 0.1834  0.4222 0.1798  0.4228 0.1789  0.4234 0.1821  0.4240 0.1809  0.4246 0.1849  0.4252 0.1795  0.4258 0.1726  0.4264 0.1809  0.4270 0.1850  0.4276 0.1872  0.4281 0.1862  0.4287 0.1865  0.4293 0.1844  0.4299 0.1829  0.4305 0.1945  0.4311 0.1949  0.4317 0.1888  0.4323 0.1913  0.4329 0.1879  0.4335 0.1840  0.4341 0.1881  0.4347 0.1915  0.4353 0.1927  0.4359 0.1891  0.4364 0.1920  0.4370 0.1988  0.4376 0.1966  0.4382 0.1932  0.4388 0.1857  0.4394 0.1875  0.4400 0.1956  0.4406 0.2059  0.4412 0.2095  0.4418 0.2042  0.4424 0.2018  0.4430 0.2009  0.4436 0.2014  0.4441 0.2067  0.4447 0.2078  0.4453 0.2122  0.4459 0.2071  0.4465 0.2040  0.4471 0.2114  0.4477 0.2137  0.4483 0.2175  0.4489 0.2129  0.4495 0.2125  0.4501 0.2044  0.4507 0.1995  0.4513 0.2063  0.4519 0.2123  0.4524 0.2114  0.4530 0.2121  0.4536 0.2246  0.4542 0.2333  0.4548 0.2290  0.4554 0.2182  0.4560 0.2175  0.4566 0.2160  0.4572 0.2200  0.4578 0.2289  0.4584 0.2262  0.4590 0.2249  0.4596 0.2298  0.4601 0.2249  0.4607 0.2240  0.4613 0.2344  0.4619 0.2312  0.4625 0.2241  0.4631 0.2196  0.4637 0.2219  0.4643 0.2303  0.4649 0.2254  0.4655 0.2257  0.4661 0.2330  0.4667 0.2328  0.4673 0.2290  0.4679 0.2319  0.4684 0.2304  0.4690 0.2306  0.4696 0.2367  0.4702 0.2431  0.4708 0.2472  0.4714 0.2483  0.4720 0.2455  0.4726 0.2426  0.4732 0.2431  0.4738 0.2486  0.4744 0.2461  0.4750 0.2314  0.4756 0.2329  0.4761 0.2462  0.4767 0.2497  0.4773 0.2443  0.4779 0.2510  0.4785 0.2542  0.4791 0.2549  0.4797 0.2537  0.4803 0.2483  0.4809 0.2507  0.4815 0.2525  0.4821 0.2574  0.4827 0.2612  0.4833 0.2589  0.4839 0.2635  0.4844 0.2609  0.4850 0.2553  0.4856 0.2539  0.4862 0.2621  0.4868 0.2689  0.4874 0.2709  0.4880 0.2795  0.4886 0.2734  0.4892 0.2702  0.4898 0.2736  0.4904 0.2658  0.4910 0.2614  0.4916 0.2711  0.4921 0.2745  0.4927 0.2697  0.4933 0.2702  0.4939 0.2683  0.4945 0.2775  0.4951 0.2811  0.4957 0.2828  0.4963 0.2918  0.4969 0.2810  0.4975 0.2787  0.4981 0.2842  0.4987 0.2720  0.4993 0.2744  0.4999 0.2857  0.5004 0.2781  0.5010 0.2777  0.5016 0.2841  0.5022 0.2831  0.5028 0.2879  0.5034 0.2940  0.5040 0.2939  0.5046 0.2949  0.5052 0.2868  0.5058 0.2860  0.5064 0.2947  0.5070 0.2963  0.5076 0.2917  0.5081 0.2935  0.5087 0.2992  0.5093 0.2996  0.5099 0.3033  0.5105 0.2983  0.5111 0.2942  0.5117 0.3103  0.5123 0.3141  0.5129 0.2916  0.5135 0.2897  0.5141 0.3046  0.5147 0.3065  0.5153 0.3005  0.5159 0.2933  0.5164 0.2992  0.5170 0.3075  0.5176 0.3172  0.5182 0.3275  0.5188 0.3189  0.5194 0.3069  0.5200 0.3099  0.5206 0.3121  0.5212 0.3135  0.5218 0.3256  0.5224 0.3085  0.5230 0.3112  0.5236 0.3195  0.5241 0.3120  0.5247 0.3200  0.5253 0.3123  0.5259 0.3217  0.5265 0.3308  0.5271 0.3232  0.5277 0.3283  0.5283 0.3379  0.5289 0.3384  0.5295 0.3255  0.5301 0.3189  0.5307 0.3379  0.5313 0.3460  0.5319 0.3395  0.5324 0.3402  0.5330 0.3403  0.5336 0.3305  0.5342 0.3326  0.5348 0.3556  0.5354 0.3558  0.5360 0.3408  0.5366 0.3504  0.5372 0.3631  0.5378 0.3595  0.5384 0.3453  0.5390 0.3439  0.5396 0.3588  0.5401 0.3665  0.5407 0.3608  0.5413 0.3473  0.5419 0.3508  0.5425 0.3627  0.5431 0.3644  0.5437 0.3508  0.5443 0.3510  0.5449 0.3703  0.5455 0.3747  0.5461 0.3552  0.5467 0.3450  0.5473 0.3608  0.5479 0.3670  0.5484 0.3636  0.5490 0.3682  0.5496 0.3654  0.5502 0.3640  0.5508 0.3729  0.5514 0.3697  0.5520 0.3708  0.5526 0.3815  0.5532 0.3825  0.5538 0.3749  0.5544 0.3777  0.5550 0.3909  0.5556 0.3946  0.5561 0.3867  0.5567 0.3877  0.5573 0.3941  0.5579 0.3981  0.5585 0.3918  0.5591 0.3949  0.5597 0.4039  0.5603 0.3834  0.5609 0.3748  0.5615 0.3953  0.5621 0.4008  0.5627 0.3973  0.5633 0.4011  0.5639 0.3874  0.5644 0.4009  0.5650 0.3975  0.5656 0.3965  0.5662 0.4092  0.5668 0.3959  0.5674 0.4065  0.5680 0.4212  0.5686 0.4249  0.5692 0.4223  0.5698 0.4214  0.5704 0.4149  0.5710 0.4221  0.5716 0.4132  0.5721 0.4003  0.5727 0.4107  0.5733 0.4154  0.5739 0.4138  0.5745 0.4147  0.5751 0.4337  0.5757 0.4358  0.5763 0.4321  0.5769 0.4302  0.5775 0.4236  0.5781 0.4242  0.5787 0.4359  0.5793 0.4254  0.5799 0.4210  0.5804 0.4300  0.5810 0.4344  0.5816 0.4466  0.5822 0.4487  0.5828 0.4444  0.5834 0.4370  0.5840 0.4409  0.5846 0.4363  0.5852 0.4331  0.5858 0.4508  0.5864 0.4563  0.5870 0.4345  0.5876 0.4358  0.5881 0.4491  0.5887 0.4557  0.5893 0.4584  0.5899 0.4667  0.5905 0.4799  0.5911 0.4682  0.5917 0.4570  0.5923 0.4642  0.5929 0.4780  0.5935 0.4814  0.5941 0.4673  0.5947 0.4669  0.5953 0.4818  0.5959 0.4872  0.5964 0.4767  0.5970 0.4818  0.5976 0.4838  0.5982 0.4879  0.5988 0.4894  0.5994 0.4812  0.6000 0.4965  0.6006 0.4855  0.6012 0.4835  0.6018 0.4810  0.6024 0.4833  0.6030 0.4973  0.6036 0.5007  0.6041 0.5056  0.6047 0.4943  0.6053 0.4970  0.6059 0.4766  0.6065 0.4822  0.6071 0.5185  0.6077 0.5153  0.6083 0.4993  0.6089 0.4952  0.6095 0.5132  0.6101 0.5079  0.6107 0.5043  0.6113 0.5044  0.6119 0.5039  0.6124 0.5079  0.6130 0.5054  0.6136 0.5199  0.6142 0.5093  0.6148 0.5041  0.6154 0.5223  0.6160 0.5216  0.6166 0.5064  0.6172 0.5120  0.6178 0.5363  0.6184 0.5509  0.6190 0.5457  0.6196 0.5332  0.6201 0.5350  0.6207 0.5295  0.6213 0.5261  0.6219 0.5358  0.6225 0.5264  0.6231 0.5431  0.6237 0.5668  0.6243 0.5381  0.6249 0.5389  0.6255 0.5370  0.6261 0.5470  0.6267 0.5747  0.6273 0.5583  0.6279 0.5529  0.6284 0.5562  0.6290 0.5663  0.6296 0.5629  0.6302 0.5513  0.6308 0.5638  0.6314 0.5660  0.6320 0.5535  0.6326 0.5652  0.6332 0.5907  0.6338 0.6007  0.6344 0.5900  0.6350 0.5885  0.6356 0.5969  0.6361 0.5941  0.6367 0.5933  0.6373 0.5874  0.6379 0.5866  0.6385 0.5970  0.6391 0.5943  0.6397 0.5752  0.6403 0.5627  0.6409 0.5779  0.6415 0.5918  0.6421 0.6022  0.6427 0.6078  0.6433 0.5925  0.6439 0.5971  0.6444 0.6134  0.6450 0.6021  0.6456 0.5953  0.6462 0.6046  0.6468 0.6044  0.6474 0.6030  0.6480 0.6102  0.6486 0.6160  0.6492 0.6113  0.6498 0.6045  0.6504 0.6234  0.6510 0.6356  0.6516 0.6311  0.6521 0.6385  0.6527 0.6278  0.6533 0.6166  0.6539 0.6196  0.6545 0.6297  0.6551 0.6344  0.6557 0.6321  0.6563 0.6301  0.6569 0.6242  0.6575 0.6344  0.6581 0.6471  0.6587 0.6499  0.6593 0.6443  0.6599 0.6381  0.6604 0.6412  0.6610 0.6515  0.6616 0.6674  0.6622 0.6632  0.6628 0.6563  0.6634 0.6585  0.6640 0.6612  0.6646 0.6688  0.6652 0.6676  0.6658 0.6633  0.6664 0.6663  0.6670 0.6800  0.6676 0.6847  0.6681 0.6876  0.6687 0.6862  0.6693 0.6949  0.6699 0.6971  0.6705 0.6817  0.6711 0.6921  0.6717 0.6948  0.6723 0.6914  0.6729 0.7001  0.6735 0.6988  0.6741 0.7087  0.6747 0.7226  0.6753 0.7127  0.6759 0.7031  0.6764 0.7143  0.6770 0.7101  0.6776 0.7011  0.6782 0.7040  0.6788 0.7088  0.6794 0.7203  0.6800 0.7200  0.6806 0.7257  0.6812 0.7430  0.6818 0.7578  0.6824 0.7426  0.6830 0.7314  0.6836 0.7487  0.6841 0.7472  0.6847 0.7380  0.6853 0.7405  0.6859 0.7453  0.6865 0.7515  0.6871 0.7504  0.6877 0.7598  0.6883 0.7578  0.6889 0.7453  0.6895 0.7603  0.6901 0.7620  0.6907 0.7672  0.6913 0.7733  0.6919 0.7609  0.6924 0.7744  0.6930 0.7780  0.6936 0.7668  0.6942 0.7704  0.6948 0.7739  0.6954 0.7810  0.6960 0.7861  0.6966 0.7923  0.6972 0.7977  0.6978 0.8012  0.6984 0.8066  0.6990 0.8024  0.6996 0.7919  0.7001 0.7905  0.7007 0.8138  0.7013 0.8223  0.7019 0.8140  0.7025 0.8291  0.7031 0.8288  0.7037 0.8081  0.7043 0.8081  0.7049 0.8130  0.7055 0.8247  0.7061 0.8367  0.7067 0.8394  0.7073 0.8291  0.7079 0.8178  0.7084 0.8241  0.7090 0.8266  0.7096 0.8330  0.7102 0.8601  0.7108 0.8484  0.7114 0.8317  0.7120 0.8490  0.7126 0.8577  0.7132 0.8635  0.7138 0.8520  0.7144 0.8568  0.7150 0.8706  0.7156 0.8757  0.7161 0.8801  0.7167 0.8659  0.7173 0.8556  0.7179 0.8744  0.7185 0.8948  0.7191 0.8815  0.7197 0.8736  0.7203 0.8846  0.7209 0.8853  0.7215 0.8796  0.7221 0.8829  0.7227 0.9043  0.7233 0.9059  0.7239 0.8983  0.7244 0.8983  0.7250 0.9027  0.7256 0.9024  0.7262 0.9040  0.7268 0.9199  0.7274 0.9167  0.7280 0.9164  0.7286 0.9123  0.7292 0.9226  0.7298 0.9361  0.7304 0.9219  0.7310 0.9319  0.7316 0.9431  0.7321 0.9271  0.7327 0.9318  0.7333 0.9378  0.7339 0.9304  0.7345 0.9394  0.7351 0.9383  0.7357 0.9527  0.7363 0.9698  0.7369 0.9564  0.7375 0.9554  0.7381 0.9658  0.7387 0.9749  0.7393 0.9721  0.7399 0.9656  0.7404 0.9866  0.7410 1.0037  0.7416 0.9943  0.7422 0.9825  0.7428 0.9941  0.7434 1.0008  0.7440 0.9930  0.7446 1.0102  0.7452 1.0178  0.7458 1.0046  0.7464 0.9973  0.7470 0.9990  0.7476 1.0166  0.7481 1.0276  0.7487 1.0286  0.7493 1.0303  0.7499 1.0272  0.7505 1.0224  0.7511 1.0150  0.7517 1.0296  0.7523 1.0467  0.7529 1.0382  0.7535 1.0353  0.7541 1.0458  0.7547 1.0501  0.7553 1.0621  0.7559 1.0665  0.7564 1.0710  0.7570 1.0878  0.7576 1.0918  0.7582 1.0862  0.7588 1.0827  0.7594 1.0826  0.7600 1.0879  0.7606 1.0865  0.7612 1.0904  0.7618 1.1095  0.7624 1.1039  0.7630 1.0884  0.7636 1.0836  0.7641 1.1021  0.7647 1.1113  0.7653 1.1189  0.7659 1.1294  0.7665 1.1194  0.7671 1.1236  0.7677 1.1331  0.7683 1.1258  0.7689 1.1230  0.7695 1.1354  0.7701 1.1466  0.7707 1.1529  0.7713 1.1453  0.7719 1.1503  0.7724 1.1549  0.7730 1.1662  0.7736 1.1745  0.7742 1.1755  0.7748 1.1772  0.7754 1.1657  0.7760 1.1688  0.7766 1.1870  0.7772 1.1856  0.7778 1.1606  0.7784 1.1729  0.7790 1.2019  0.7796 1.2059  0.7801 1.2023  0.7807 1.2012  0.7813 1.2098  0.7819 1.2200  0.7825 1.2244  0.7831 1.2204  0.7837 1.2091  0.7843 1.2157  0.7849 1.2259  0.7855 1.2024  0.7861 1.2001  0.7867 1.2396  0.7873 1.2426  0.7879 1.2588  0.7884 1.2665  0.7890 1.2444  0.7896 1.2502  0.7902 1.2630  0.7908 1.2631  0.7914 1.2617  0.7920 1.2737  0.7926 1.2811  0.7932 1.2832  0.7938 1.2874  0.7944 1.2929  0.7950 1.2801  0.7956 1.2877  0.7961 1.3023  0.7967 1.3019  0.7973 1.3135  0.7979 1.3166  0.7985 1.3195  0.7991 1.3204  0.7997 1.3167  0.8003 1.3239  0.8009 1.3255  0.8015 1.3337  0.8021 1.3548  0.8027 1.3551  0.8033 1.3600  0.8039 1.3721  0.8044 1.3746  0.8050 1.3660  0.8056 1.3651  0.8062 1.3673  0.8068 1.3762  0.8074 1.3842  0.8080 1.3820  0.8086 1.3888  0.8092 1.4010  0.8098 1.4155  0.8104 1.4103  0.8110 1.4036  0.8116 1.4113  0.8121 1.4052  0.8127 1.4082  0.8133 1.4325  0.8139 1.4380  0.8145 1.4339  0.8151 1.4318  0.8157 1.4402  0.8163 1.4479  0.8169 1.4555  0.8175 1.4654  0.8181 1.4682  0.8187 1.4585  0.8193 1.4582  0.8199 1.4755  0.8204 1.4916  0.8210 1.4868  0.8216 1.5023  0.8222 1.5174  0.8228 1.4975  0.8234 1.4997  0.8240 1.5084  0.8246 1.5124  0.8252 1.5222  0.8258 1.5263  0.8264 1.5256  0.8270 1.5316  0.8276 1.5489  0.8281 1.5582  0.8287 1.5583  0.8293 1.5601  0.8299 1.5608  0.8305 1.5626  0.8311 1.5628  0.8317 1.5792  0.8323 1.5917  0.8329 1.5958  0.8335 1.6034  0.8341 1.5904  0.8347 1.6005  0.8353 1.6316  0.8359 1.6344  0.8364 1.6242  0.8370 1.6134  0.8376 1.6358  0.8382 1.6560  0.8388 1.6557  0.8394 1.6556  0.8400 1.6489  0.8406 1.6526  0.8412 1.6713  0.8418 1.6812  0.8424 1.6861  0.8430 1.6949  0.8436 1.6926  0.8441 1.6901  0.8447 1.7070  0.8453 1.7180  0.8459 1.7174  0.8465 1.7178  0.8471 1.7151  0.8477 1.7273  0.8483 1.7336  0.8489 1.7414  0.8495 1.7376  0.8501 1.7333  0.8507 1.7362  0.8513 1.7515  0.8519 1.7758  0.8524 1.7753  0.8530 1.7761  0.8536 1.7897  0.8542 1.7974  0.8548 1.8050  0.8554 1.8026  0.8560 1.8045  0.8566 1.8223  0.8572 1.8240  0.8578 1.8350  0.8584 1.8451  0.8590 1.8415  0.8596 1.8468  0.8601 1.8534  0.8607 1.8584  0.8613 1.8537  0.8619 1.8588  0.8625 1.8787  0.8631 1.8840  0.8637 1.8889  0.8643 1.8968  0.8649 1.8986  0.8655 1.9009  0.8661 1.9197  0.8667 1.9393  0.8673 1.9441  0.8679 1.9505  0.8684 1.9265  0.8690 1.9270  0.8696 1.9663  0.8702 1.9813  0.8708 1.9854  0.8714 1.9793  0.8720 1.9834  0.8726 1.9900  0.8732 1.9960  0.8738 2.0173  0.8744 2.0258  0.8750 2.0342  0.8756 2.0457  0.8761 2.0481  0.8767 2.0620  0.8773 2.0689  0.8779 2.0729  0.8785 2.0781  0.8791 2.0840  0.8797 2.0898  0.8803 2.1059  0.8809 2.1158  0.8815 2.1178  0.8821 2.1271  0.8827 2.1303  0.8833 2.1403  0.8839 2.1522  0.8844 2.1340  0.8850 2.1484  0.8856 2.1813  0.8862 2.1967  0.8868 2.2057  0.8874 2.1989  0.8880 2.2054  0.8886 2.2146  0.8892 2.2292  0.8898 2.2205  0.8904 2.2278  0.8910 2.2538  0.8916 2.2568  0.8921 2.2741  0.8927 2.2787  0.8933 2.2933  0.8939 2.2864  0.8945 2.3022  0.8951 2.3365  0.8957 2.3199  0.8963 2.3216  0.8969 2.3442  0.8975 2.3579  0.8981 2.3546  0.8987 2.3660  0.8993 2.3768  0.8999 2.3796  0.9004 2.3932  0.9010 2.4067  0.9016 2.4103  0.9022 2.4139  0.9028 2.4213  0.9034 2.4395  0.9040 2.4578  0.9046 2.4692  0.9052 2.4751  0.9058 2.4770  0.9064 2.4860  0.9070 2.4949  0.9076 2.4991  0.9081 2.5174  0.9087 2.5400  0.9093 2.5512  0.9099 2.5594  0.9105 2.5684  0.9111 2.5790  0.9117 2.5909  0.9123 2.6015  0.9129 2.6047  0.9135 2.6047  0.9141 2.6206  0.9147 2.6345  0.9153 2.6429  0.9159 2.6606  0.9164 2.6734  0.9170 2.6905  0.9176 2.7002  0.9182 2.7049  0.9188 2.7240  0.9194 2.7120  0.9200 2.7271  0.9206 2.7720  0.9212 2.7851  0.9218 2.8001  0.9224 2.8097  0.9230 2.8184  0.9236 2.8207  0.9241 2.8636  0.9247 2.8571  0.9253 2.8371  0.9259 2.8771  0.9265 2.8881  0.9271 2.9004  0.9277 2.9131  0.9283 2.9255  0.9289 2.9455  0.9295 2.9642  0.9301 2.9735  0.9307 2.9788  0.9313 2.9965  0.9319 3.0196  0.9324 3.0350  0.9330 3.0539  0.9336 3.0764  0.9342 3.0957  0.9348 3.0692  0.9354 3.0352  0.9360 2.9902  0.9366 3.0772  0.9372 3.0296  0.9378 2.8979  0.9384 4.0617  0.9390 4.0756  0.9396 3.0787  0.9401 3.2240  0.9407 3.2381  0.9413 3.2486  0.9419 3.2584  0.9425 3.2770  0.9431 3.2924  0.9437 3.3114  0.9443 3.3291  0.9449 3.3497  0.9455 3.3746  0.9461 3.3741  0.9467 3.4141  0.9473 3.4179  0.9479 3.4178  0.9484 3.4656  0.9490 3.4613  0.9496 3.4864  0.9502 3.5158  0.9508 3.5333  0.9514 3.5573  0.9520 3.5380  0.9526 3.6005  0.9532 3.6165  0.9538 3.6259  0.9544 3.6758  0.9550 3.6672  0.9556 3.7158  0.9561 3.6722  0.9567 3.7062  0.9573 3.7728  0.9579 3.7891  0.9585 3.8582  0.9591 3.8056  0.9597 3.8553  0.9603 3.8972  0.9609 3.8582  0.9615 3.9447  0.9621 3.9662  0.9627 3.9265  0.9633 3.9330  0.9639 4.0083  0.9644 4.0482  0.9650 3.9435  0.9656 4.0839  0.9662 3.9921  0.9668 3.7584  0.9674 7.0973  0.9680 6.8641  0.9686 3.7256  0.9692 4.1037  0.9698 5.3301  0.9704 5.2589  0.9710 4.1115  0.9716 4.8577  0.9721 4.8023  0.9727 4.3559  0.9733 4.5810  0.9739 4.5041  0.9745 4.5268  0.9751 4.5968  0.9757 4.4709  0.9763 4.6138  0.9769 4.4082  0.9775 5.2787  0.9781 5.3420  0.9787 4.5252  0.9793 4.9990
 /






\color{black}
\normalcolor
%
%
%\color{blue}
%\put {\LARGE$\bullet$} at 0.0 -1.5442
%\color{red}
%\setdots <12pt>
%\setplotsymbol ({$\bullet$})
%\plot 0.0125 0.0001  0.0250 0.0005  0.0375 0.0010  0.0500 0.0019  0.0625 0.0029  0.0750 0.0043  0.0875 0.0059  0.1000 0.0077  0.1125 0.0099  0.1250 0.0124  0.1375 0.0151  0.1500 0.0182  0.1625 0.0216  0.1750 0.0254  0.1875 0.0295  0.2000 0.0340  0.2125 0.0388  0.2250 0.0441  0.2375 0.0497  0.2500 0.0558  0.2625 0.0623  0.2750 0.0693  0.2875 0.0767  0.3000 0.0846  0.3125 0.0931  0.3250 0.1020  0.3375 0.1116  0.3500 0.1217  0.3625 0.1324  0.3750 0.1437  0.3875 0.1557  0.4000 0.1684  0.4125 0.1817  0.4250 0.1959  0.4375 0.2108  0.4500 0.2265  0.4625 0.2432  0.4750 0.2607  0.4875 0.2791  0.5000 0.2986  0.5125 0.3191  0.5250 0.3408  0.5375 0.3636  0.5500 0.3876  0.5625 0.4130  0.5750 0.4398  0.5875 0.4680  0.6000 0.4979  0.6125 0.5294  0.6250 0.5627  0.6375 0.5979  0.6500 0.6352  0.6625 0.6747  0.6750 0.7166  0.6875 0.7611  0.7000 0.8084  0.7125 0.8587  0.7250 0.9123  0.7375 0.9695  0.7500 1.0307  0.7625 1.0963  0.7750 1.1668  0.7875 1.2427  0.8000 1.3248  0.8125 1.4137  0.8250 1.5105  0.8375 1.6164  0.8500 1.7328  0.8625 1.8615  0.8750 2.0049  0.8875 2.1661  0.9000 2.3494  0.9125 2.5606  0.9250 2.8085  0.9375 3.1064  0.9500 3.4769  0.9625 3.9621  0.9750 4.6568  0.9875 5.8633 0.9920 6.6476  0.9960 7.8722
%  /

\normalcolor
\color{black}

\endpicture

==> Figures/figure20.tex <==


\beginpicture

\normalcolor
\color{black}
\setcoordinatesystem units <40pt,2.15pt>
\axes{0}{-50}{0}{0}{7}{50}{-3}
\axis left shiftedto x=0 label {\Large$\Pi_{3_1} L^{3}$} 
      ticks
      withvalues -25 25 /
      at -25 25 /
 /  
\axis bottom shiftedto y=0 %label {$\phi$} 
    ticks
    withvalues 1 2 3 4 5 6 /
    at 1 2 3 4 5 6 /
/

\put {\Large$\phi L^{4/3}$} at 5.5 -15

\plot 3.7 0 3.7 -35 /
\put {$\phi_0L^{4/3}$} at 3.7 -40

\setplotsymbol ({\fiverm.})



%% 31 scaled

%L=4
\color{B04}
\multiput {\tiny{$\bullet$}} at
 2.6787 -51.6554  2.8772 -41.4562  3.0756 -32.9493  3.2740 -25.3423  3.4724 -18.1794  3.6709 -11.2004  3.8693 -4.1502  4.0677 3.2381  4.2661 11.2141  4.4646 20.0849  4.6630 30.1032  4.8614 41.6622 /

%L=5
\color{B05}
\multiput {\tiny{$\bullet$}} at
2.1204 -48.9126  2.2572 -44.4106  2.3940 -40.3497  2.5308 -36.5925  2.6676 -32.9944  2.8044 -29.5239  2.9412 -26.1266  3.0780 -22.7143  3.2148 -19.3273  3.3516 -15.9757  3.4884 -12.5893  3.6251 -9.1689  3.7619 -5.6860  3.8987 -2.1565  4.0355 1.4962  4.1723 5.3338  4.3091 9.2090  4.4459 13.2627  4.5827 17.5734  4.7195 22.0731  4.8563 26.7473  4.9931 31.6999  5.1299 36.9784  5.2667 42.5550  5.4035 48.4795  /

%L=6
\color{B06}
\multiput {\tiny{$\bullet$}} at
1.5647 -51.6702  1.6657 -48.2373  1.7666 -45.3183  1.8676 -42.7619  1.9685 -40.4405  2.0695 -38.2313  2.1704 -36.0780  2.2714 -34.0172  2.3724 -31.9495  2.4733 -29.9306  2.5743 -27.9337  2.6752 -25.9187  2.7762 -23.9380  2.8771 -21.9216  2.9781 -19.9234  3.0790 -17.9261  3.1800 -15.9044  3.2809 -13.8513  3.3819 -11.8128  3.4828 -9.7020  3.5838 -7.5292  3.6847 -5.3855  3.7857 -3.3143  3.8866 -1.1229  3.9876 1.3299  4.0885 3.6397  4.1895 5.8383  4.2904 8.2573  4.3914 10.8180  4.4923 13.3638  4.5933 15.8771  4.6942 18.5021  4.7952 21.3002  4.8961 24.1797  4.9971 27.1549  5.0980 30.1685  5.1990 33.2493  5.2999 36.5141  5.4009 39.7708  5.5018 43.1883  5.6028 46.7539  5.7037 50.4559  /

%L=7
\color{B07}
\multiput {\tiny{$\bullet$}} at
1.2883 -48.7215  1.3664 -46.2807  1.4445 -44.3006  1.5225 -42.5553  1.6006 -40.9399  1.6787 -39.4194  1.7568 -38.0192  1.8349 -36.5922  1.9129 -35.1934  1.9910 -33.8776  2.0691 -32.5235  2.1472 -31.1301  2.2252 -30.3253  2.3033 -29.7399  2.3814 -27.8465  2.4595 -25.8995  2.5376 -24.7264  2.6156 -23.3817  2.6937 -21.9347  2.7718 -20.6483  2.8499 -19.3020  2.9280 -17.9089  3.0060 -16.5656  3.0841 -15.1667  3.1622 -13.7253  3.2403 -12.2530  3.3184 -10.8893  3.3964 -9.4419  3.4745 -7.9394  3.5526 -6.4565  3.6307 -4.9393  3.7087 -3.4486  3.7868 -1.8536  3.8649 -0.3570  3.9430 1.1790  4.0211 2.8497  4.0991 4.5099  4.1772 6.1403  4.2553 7.6879  4.3334 10.6770  4.4115 12.1559  4.4895 13.8832  4.5676 15.9983  4.6457 16.5024  4.7238 18.4840  4.8018 20.4258  4.8799 22.3996  4.9580 24.3642  5.0361 26.4443  5.1142 28.5070  5.1922 30.6775  5.2703 32.8413  5.3484 34.8530  5.4265 37.0447  5.5046 39.3518  5.5826 41.7573  5.6607 44.2332  5.7388 46.9122  5.8169 49.4462  5.8950 51.8546 
   /

%L=8
\color{B08}
\multiput {\tiny{$\bullet$}} at
0.9688 -51.0177  1.0312 -48.2340  1.0938 -46.3942  1.1562 -44.6401  1.2188 -42.7716  1.2812 -41.6705  1.3438 -40.4242  1.4062 -38.8847  1.4688 -38.2168  1.5312 -37.8911  1.5938 -36.5831  1.6562 -34.6919  1.7188 -34.1705  1.7812 -33.9047  1.8438 -33.8159  1.9062 -32.4070  1.9688 -30.8738  2.0312 -30.5196  2.0938 -28.6649  2.1562 -28.1208  2.2188 -27.3177  2.2812 -24.9992  2.3438 -25.3530  2.4062 -25.7182  2.4688 -23.3889  2.5312 -21.2616  2.5938 -21.2511  2.6562 -21.2573  2.7188 -18.8393  2.7812 -19.0471  2.8438 -19.4168  2.9062 -15.7374  2.9688 -15.5340  3.0312 -15.8566  3.0938 -12.8441  3.1562 -14.5062  3.2188 -14.4500  3.2812 -11.5342  3.3438 -8.2994  3.4062 -4.9231  3.4688 -6.7226  3.5312 -5.5774  3.5938 -4.4358  3.6562 -5.0217  3.7188 -1.4719  3.7812 -0.8661  3.8438 -0.0704  3.9062 1.2037  3.9688 1.4910  4.0312 3.5821  4.0938 3.2238  4.1562 4.8811  4.2188 6.2652  4.2812 6.3450  4.3438 10.6604  4.4062 10.2544  4.4688 11.3649  4.5312 14.4739  4.5938 11.2113  4.6562 13.9785  4.7188 18.0733  4.7812 18.9623  4.8438 21.2597  4.9062 21.0802  4.9688 22.7148  5.0312 24.0311  5.0938 25.4311  5.1562 28.9849  5.2188 30.3008  5.2812 31.8599  5.3438 33.5327  5.4062 35.4472  5.4688 37.0385  5.5312 38.5295  5.5938 40.4951  5.6562 42.2097  5.7188 43.9115  5.7812 45.5410  5.8438 49.3807
  /

%L=9
\color{B09}
\multiput {\tiny{$\bullet$}} at
0.7961 -50.3708  0.8474 -47.7401  0.8988 -45.9768  0.9502 -44.2472  1.0015 -42.6771  1.0529 -41.6689  1.1042 -40.3926  1.1556 -39.4630  1.2070 -38.6570  1.2583 -37.6040  1.3097 -37.2416  1.3610 -36.6037  1.4124 -35.0825  1.4638 -34.4902  1.5151 -34.9602  1.5665 -33.7920  1.6178 -32.8764  1.6692 -33.0786  1.7206 -31.8787  1.7719 -30.8833  1.8233 -30.0413  1.8746 -29.5651  1.9260 -29.2762  1.9774 -26.9138  2.0287 -26.7879  2.0801 -27.2389  2.1314 -26.6464  2.1828 -26.0214  2.2342 -25.7110  2.2855 -25.0448  2.3369 -23.2215  2.3882 -22.8399  2.4396 -22.6120  2.4910 -21.4405  2.5423 -20.1782  2.5937 -20.5970  2.6450 -19.9537  2.6964 -18.8853  2.7478 -18.3792  2.7991 -19.1578  2.8505 -17.0925  2.9018 -15.0558  2.9532 -15.6779  3.0046 -13.7316  3.0559 -12.9121  3.1073 -9.4855  3.1586 -9.8828  3.2100 -12.0931  3.2614 -7.7332  3.3127 -9.8198  3.3641 -11.1726  3.4154 -5.5717  3.4668 -2.1527  3.5182 -3.8048  3.5695 -6.8794  3.6209 -4.8842  3.6722 -2.8098  3.7236 -2.1369  3.7750 -1.5652  3.8263 0.1728  3.8777 3.0562  3.9290 -1.3633  3.9804 -1.2963  4.0318 4.0543  4.0831 5.9676  4.1345 7.0432  4.1858 7.1676  4.2372 7.9039  4.2886 7.6540  4.3399 8.7464  4.3913 10.9397  4.4426 11.4842  4.4940 14.8864  4.5454 13.1128  4.5967 10.9863  4.6481 13.8227  4.6994 15.4299  4.7508 20.1855  4.8022 20.7571  4.8535 20.3204  4.9049 20.2322  4.9562 20.3468  5.0076 30.7688  5.0590 25.3885  5.1103 19.5500  5.1617 33.6821  5.2130 27.7884  5.2644 24.3795  5.3158 30.5871  5.3671 38.1284  5.4185 41.9276  5.4699 32.2416  5.5212 35.5224  5.5726 44.0752  5.6239 41.9538  5.6753 39.5956  5.7267 45.8972  5.7780 44.9250  5.8294 41.8096  5.8807 43.3590  5.9321 48.5565  5.9835 53.4307  6.0348 50.0179  6.0862 51.2218 
 /

%L=10
\color{B10}
\multiput {\tiny{$\bullet$}} at
0.6679 -49.9195  0.7110 -47.3913  0.7541 -45.0664  0.7971 -43.2279  0.8402 -42.0551  0.8833 -40.8935  0.9264 -39.9015  0.9695 -39.7683  1.0126 -38.8829  1.0557 -38.2958  1.0988 -37.7469  1.1419 -36.1008  1.1849 -35.7320  1.2280 -35.3776  1.2711 -35.0297  1.3142 -33.8759  1.3573 -33.6813  1.4004 -33.0232  1.4435 -32.5230  1.4866 -33.3438  1.5296 -32.5276  1.5727 -31.3103  1.6158 -31.5370  1.6589 -32.0305  1.7020 -30.7689  1.7451 -30.3071  1.7882 -29.8108  1.8313 -27.9212  1.8744 -28.0000  1.9174 -28.5220  1.9605 -26.6439  2.0036 -25.5382  2.0467 -25.9021  2.0898 -26.1801  2.1329 -24.9093  2.1760 -24.7033  2.2191 -25.6508  2.2622 -24.6642  2.3052 -23.7207  2.3483 -22.5570  2.3914 -21.7337  2.4345 -19.2956  2.4776 -18.5484  2.5207 -20.6773  2.5638 -19.2841  2.6069 -18.7708  2.6500 -18.6536  2.6930 -16.3588  2.7361 -14.9069  2.7792 -13.7462  2.8223 -14.7242  2.8654 -15.7714  2.9085 -14.8727  2.9516 -12.4387  2.9947 -12.6952  3.0378 -11.2367  3.0808 -11.5349  3.1239 -10.0288  3.1670 -7.7169  3.2101 -11.2658  3.2532 -10.8377  3.2963 -8.7774  3.3394 -7.3469  3.3825 -8.4207  3.4256 -6.2457  3.4686 -3.4005  3.5117 -4.9539  3.5548 -3.4655  3.5979 -1.4021  3.6410 -2.2964  3.6841 -3.1642  3.7272 -0.3843  3.7703 0.5473  3.8133 -0.0712  3.8564 0.5583  3.8995 1.8052  3.9426 4.0417  3.9857 2.9101  4.0288 3.4140  4.0719 6.2185  4.1150 5.6260  4.1581 5.9366  4.2011 7.6220  4.2442 5.0804  4.2873 8.3447  4.3304 10.7734  4.3735 6.8466  4.4166 13.5373  4.4597 13.2734  4.5028 9.7942  4.5459 14.4351  4.5889 15.4176  4.6320 16.1722  4.6751 15.5978  4.7182 20.4387  4.7613 19.1176  4.8044 19.3838  4.8475 23.7412  4.8906 22.9983  4.9337 23.4153  4.9767 22.7160  5.0198 24.0435  5.0629 24.2725  5.1060 26.2615  5.1491 27.8321  5.1922 33.4935  5.2353 32.0046  5.2784 29.2060  5.3215 32.8201  5.3645 31.3148  5.4076 30.3237  5.4507 35.1911  5.4938 37.6053  5.5369 36.5752  5.5800 36.4549  5.6231 39.5519  5.6662 43.5261  5.7093 40.8779  5.7523 40.7619  5.7954 48.0625  5.8385 42.4485  5.8816 38.6583  5.9247 48.6628  5.9678 48.1279  6.0109 47.2129  6.0540 50.8769  
  /

%L=11
\color{B11}
\multiput {\tiny{$\bullet$}} at
0.5698 -49.5525  0.6065 -46.8426  0.6433 -44.9481  0.6801 -43.3631  0.7168 -41.7946  0.7536 -40.7778  0.7903 -39.6436  0.8271 -38.6701  0.8639 -38.0930  0.9006 -37.0967  0.9374 -36.6076  0.9741 -36.1607  1.0109 -35.2273  1.0477 -34.9290  1.0844 -34.6018  1.1212 -34.4878  1.1579 -34.3176  1.1947 -33.3543  1.2315 -33.4047  1.2682 -33.6442  1.3050 -33.0926  1.3417 -31.6028  1.3785 -30.6688  1.4153 -30.8540  1.4520 -30.4044  1.4888 -29.8030  1.5255 -30.1879  1.5623 -30.0545  1.5991 -29.2895  1.6358 -29.0152  1.6726 -28.6586  1.7093 -28.2907  1.7461 -28.0648  1.7829 -29.4278  1.8196 -28.3371  1.8564 -26.3842  1.8931 -27.7001  1.9299 -25.3401  1.9667 -23.4434  2.0034 -24.7276  2.0402 -25.5278  2.0769 -25.5253  2.1137 -24.2044  2.1505 -24.0450  2.1872 -23.6642  2.2240 -24.5490  2.2607 -23.5204  2.2975 -22.1658  2.3343 -20.7601  2.3710 -19.8174  2.4078 -20.5890  2.4445 -19.5324  2.4813 -19.7407  2.5181 -19.8192  2.5548 -17.5497  2.5916 -18.3348  2.6283 -19.3564  2.6651 -16.9589  2.7019 -16.6653  2.7386 -15.3716  2.7754 -13.9690  2.8121 -12.6990  2.8489 -12.9258  2.8857 -14.8598  2.9224 -12.3685  2.9592 -12.5228  2.9959 -13.3267  3.0327 -11.1072  3.0695 -9.9423  3.1062 -8.5471  3.1430 -9.0706  3.1797 -10.8636  3.2165 -10.5309  3.2533 -8.3217  3.2900 -6.4647  3.3268 -7.0824  3.3635 -8.0678  3.4003 -4.1856  3.4371 -4.3839  3.4738 -4.0405  3.5106 -2.8226  3.5473 -5.6598  3.5841 -5.8320  3.6209 -5.0143  3.6576 -2.2953  3.6944 -1.5466  3.7311 0.6254  3.7679 1.6682  3.8047 2.8835  3.8414 4.1139  3.8782 2.2224  3.9149 2.9790  3.9517 -0.8397  3.9885 0.6134  4.0252 7.8951  4.0620 8.6674  4.0987 5.4012  4.1355 5.8806  4.1723 7.6410  4.2090 6.4689  4.2458 7.3691  4.2825 8.7444  4.3193 9.2643  4.3561 10.2001  4.3928 12.2970  4.4296 12.5746  4.4663 11.7634  4.5031 10.9627  4.5399 11.3230  4.5766 20.1213  4.6134 21.2224  4.6501 13.7114  4.6869 15.6876  4.7237 18.2656  4.7604 18.1375  4.7972 12.7007  4.8339 19.9672  4.8707 28.9220  4.9075 18.8119  4.9442 22.8606  4.9810 22.9131  5.0177 16.9354  5.0545 28.1458  5.0913 30.9611  5.1280 22.9235  5.1648 31.2314  5.2015 33.0857  5.2383 25.3951  5.2751 28.5560  5.3118 31.6156  5.3486 32.5653  5.3853 32.9316  5.4221 31.2180  5.4589 30.8317  5.4956 30.5874  5.5324 35.7436  5.5691 38.9295  5.6059 41.7606  5.6427 40.9728  5.6794 36.9791  5.7162 39.6877  5.7529 43.6579  5.7897 44.3524  5.8265 44.3882  5.8632 46.4751  5.9000 40.6979  5.9367 41.0415  5.9735 44.8201  6.0103 52.1609  6.0470 51.6511 
 /

%L=12
\color{B12}
\multiput {\tiny{$\bullet$}} at
0.4929 -48.8155  0.5247 -46.0943  0.5565 -44.1174  0.5883 -42.8102  0.6201 -41.7407  0.6519 -40.8294  0.6836 -39.6207  0.7154 -38.3659  0.7472 -37.9667  0.7790 -37.2844  0.8108 -36.5956  0.8426 -36.4826  0.8744 -35.5000  0.9062 -35.1804  0.9380 -34.7524  0.9698 -34.0338  1.0016 -34.1863  1.0334 -33.7923  1.0652 -33.3601  1.0970 -33.2787  1.1288 -33.1819  1.1606 -32.5593  1.1924 -31.9622  1.2242 -31.7913  1.2560 -31.9376  1.2878 -31.9959  1.3196 -31.5384  1.3514 -30.7136  1.3832 -30.4235  1.4150 -30.3444  1.4468 -30.0898  1.4786 -29.3562  1.5104 -28.8026  1.5422 -29.2606  1.5740 -28.6062  1.6058 -27.1301  1.6376 -27.2523  1.6694 -28.8745  1.7012 -28.2873  1.7330 -26.4709  1.7648 -26.4415  1.7966 -27.3219  1.8284 -26.6771  1.8602 -24.4907  1.8920 -25.5750  1.9238 -26.7289  1.9556 -24.2091  1.9874 -23.4847  2.0191 -23.3490  2.0509 -22.3021  2.0827 -23.3960  2.1145 -23.6224  2.1463 -21.6495  2.1781 -22.6004  2.2099 -22.6917  2.2417 -21.3177  2.2735 -20.5098  2.3053 -20.2890  2.3371 -20.6073  2.3689 -20.0979  2.4007 -20.3655  2.4325 -19.7335  2.4643 -20.1737  2.4961 -20.5708  2.5279 -17.0451  2.5597 -16.3308  2.5915 -16.4495  2.6233 -15.3490  2.6551 -18.4040  2.6869 -18.1646  2.7187 -15.3517  2.7505 -13.1096  2.7823 -12.5649  2.8141 -14.1794  2.8459 -14.3048  2.8777 -12.8847  2.9095 -13.9933  2.9413 -13.7230  2.9731 -8.5642  3.0049 -9.7594  3.0367 -11.8904  3.0685 -9.8180  3.1003 -10.3535  3.1321 -9.3775  3.1639 -9.0872  3.1957 -7.7719  3.2275 -6.3309  3.2593 -10.7807  3.2911 -6.1619  3.3229 -2.5018  3.3546 -6.1974  3.3864 -7.6528  3.4182 -4.6906  3.4500 -2.9378  3.4818 -4.6973  3.5136 -5.8048  3.5454 -5.3862  3.5772 1.3162  3.6090 0.4558  3.6408 -2.3652  3.6726 -0.2024  3.7044 0.6031  3.7362 -1.4218  3.7680 -0.8028  3.7998 1.2447  3.8316 -0.1187  3.8634 1.0745  3.8952 4.8280  3.9270 4.1027  3.9588 4.5184  3.9906 5.8656  4.0224 3.0197  4.0542 3.0597  4.0860 8.1382  4.1178 11.0759  4.1496 8.4663  4.1814 11.0239  4.2132 7.1235  4.2450 3.5509  4.2768 11.9567  4.3086 10.8700  4.3404 8.5295  4.3722 9.0141  4.4040 13.3053  4.4358 16.3183  4.4676 13.7167  4.4994 13.9470  4.5312 15.2869  4.5630 15.3787  4.5948 15.2718  4.6266 19.3425  4.6584 20.1651  4.6901 19.5320  4.7219 16.8405  4.7537 18.0168  4.7855 21.0538  4.8173 20.0349  4.8491 23.3268  4.8809 23.6754  4.9127 20.2119  4.9445 20.0318  4.9763 21.5048  5.0081 25.6157  5.0399 28.7365  5.0717 24.8465  5.1035 23.2077  5.1353 24.2275  5.1671 28.7269  5.1989 29.6494  5.2307 32.0678  5.2625 37.5003  5.2943 27.0128  5.3261 26.2407  5.3579 34.9674  5.3897 33.5866  5.4215 34.8332  5.4533 35.1215  5.4851 35.6659  5.5169 39.2202  5.5487 40.0435  5.5805 41.4210  5.6123 37.2128  5.6441 38.1810  5.6759 40.4087  5.7077 36.5785  5.7395 43.9322  5.7713 45.6145  5.8031 42.1254  5.8349 43.5760  5.8667 44.5478  5.8985 42.3322  5.9303 39.9189  5.9621 48.2166  5.9939 53.4388  6.0256 46.5678
   /

%L=13
\color{B13}
\multiput {\tiny{$\bullet$}} at
0.4313 -48.9543  0.4591 -46.3314  0.4870 -44.1403  0.5148 -42.4015  0.5426 -41.0456  0.5704 -39.8756  0.5983 -38.8436  0.6261 -37.9965  0.6539 -37.2621  0.6817 -36.6363  0.7096 -36.0909  0.7374 -35.4387  0.7652 -34.9205  0.7931 -34.5385  0.8209 -34.3641  0.8487 -34.0297  0.8765 -33.6650  0.9044 -33.3811  0.9322 -33.0235  0.9600 -32.7391  0.9878 -32.4384  1.0157 -32.2900  1.0435 -32.0579  1.0713 -31.6330  1.0991 -31.3167  1.1270 -31.1225  1.1548 -30.8778  1.1826 -30.9745  1.2105 -30.7657  1.2383 -30.4201  1.2661 -29.9179  1.2939 -29.6495  1.3218 -29.9392  1.3496 -29.7169  1.3774 -29.5273  1.4052 -29.3345  1.4331 -28.9836  1.4609 -28.5795  1.4887 -28.2546  1.5165 -28.0794  1.5444 -28.0592  1.5722 -27.7777  1.6000 -27.2676  1.6278 -27.0231  1.6557 -26.7863  1.6835 -26.5840  1.7113 -26.2144  1.7392 -25.9608  1.7670 -25.8396  1.7948 -25.7174  1.8226 -25.3190  1.8505 -24.8719  1.8783 -25.0366  1.9061 -24.7937  1.9339 -24.1871  1.9618 -23.8874  1.9896 -23.8363  2.0174 -23.2245  2.0452 -23.0125  2.0731 -23.0544  2.1009 -22.3749  2.1287 -21.7601  2.1565 -21.2910  2.1844 -21.0545  2.2122 -21.1229  2.2400 -20.4550  2.2679 -20.0070  2.2957 -19.8562  2.3235 -19.3008  2.3513 -19.3938  2.3792 -18.9174  2.4070 -18.3736  2.4348 -18.0590  2.4626 -18.0016  2.4905 -17.8018  2.5183 -17.2825  2.5461 -16.9482  2.5739 -16.5308  2.6018 -16.9681  2.6296 -16.2483  2.6574 -15.0503  2.6853 -15.5007  2.7131 -16.1640  2.7409 -15.5318  2.7687 -14.2607  2.7966 -13.9299  2.8244 -13.5995  2.8522 -12.9112  2.8800 -12.7357  2.9079 -13.4976  2.9357 -11.9384  2.9635 -11.1971  2.9913 -11.6692  3.0192 -10.2515  3.0470 -10.3426  3.0748 -9.3407  3.1026 -8.6466  3.1305 -8.7973  3.1583 -8.6051  3.1861 -8.6508  3.2140 -7.9250  3.2418 -7.6095  3.2696 -7.4869  3.2974 -7.3572  3.3253 -5.6495  3.3531 -4.1669  3.3809 -4.4975  3.4087 -5.0402  3.4366 -4.5625  3.4644 -4.1105  3.4922 -3.2912  3.5200 -2.9708  3.5479 -3.1710  3.5757 -1.6115  3.6035 -1.4385  3.6314 -2.5766  3.6592 -2.0977  3.6870 -0.9586  3.7148 -1.0683  3.7427 0.8623  3.7705 2.0045  3.7983 1.1259  3.8261 1.6188  3.8540 1.6455  3.8818 2.6018  3.9096 4.0410  3.9374 4.9009  3.9653 5.1728  3.9931 2.8517  4.0209 2.9222  4.0487 4.7086  4.0766 6.2737  4.1044 6.4048  4.1322 5.1803  4.1601 7.7410  4.1879 9.4090  4.2157 8.6969  4.2435 7.7735  4.2714 8.9640  4.2992 10.2143  4.3270 10.1151  4.3548 11.7228  4.3827 12.8689  4.4105 13.6020  4.4383 13.5948  4.4661 14.7059  4.4940 15.5452  4.5218 13.2785  4.5496 13.8289  4.5775 14.8373  4.6053 16.3030  4.6331 20.1434  4.6609 20.3457  4.6888 18.8392  4.7166 17.0284  4.7444 17.3393  4.7722 18.1384  4.8001 18.6493  4.8279 19.8956  4.8557 21.3855  4.8835 22.8818  4.9114 20.7369  4.9392 20.7134  4.9670 23.0825  4.9948 25.5613  5.0227 27.4602  5.0505 25.0534  5.0783 24.4707  5.1062 24.4406  5.1340 25.6243  5.1618 29.0980  5.1896 27.9768  5.2175 25.6408  5.2453 28.4975  5.2731 33.4347  5.3009 33.5921  5.3288 32.3745  5.3566 32.8002  5.3844 34.7003  5.4122 33.9870  5.4401 33.8784  5.4679 36.3256  5.4957 37.1604  5.5235 38.8084  5.5514 38.1234  5.5792 39.0558  5.6070 39.2082  5.6349 37.8110  5.6627 38.6257  5.6905 41.3726  5.7183 41.8462  5.7462 40.8878  5.7740 43.6968  5.8018 43.8504  5.8296 44.1209  5.8575 44.8016  5.8853 45.3939  5.9131 45.1118  5.9409 45.7378  5.9688 48.1869  5.9966 46.9999  6.0244 47.8157 
/


%L=14
\color{B14}
\multiput {\tiny{$\bullet$}} at
0.3812 -48.2732  0.4058 -45.4904  0.4304 -43.5077  0.4550 -41.9405  0.4796 -40.6015  0.5042 -39.5249  0.5288 -38.4345  0.5533 -38.0170  0.5779 -37.3665  0.6025 -36.4415  0.6271 -36.2904  0.6517 -35.2548  0.6763 -34.5273  0.7009 -34.6546  0.7255 -34.1731  0.7501 -33.8480  0.7747 -33.8044  0.7993 -33.4412  0.8239 -33.1146  0.8485 -32.6995  0.8731 -31.8464  0.8977 -31.8671  0.9222 -32.1941  0.9468 -31.5274  0.9714 -31.5376  0.9960 -31.4928  1.0206 -31.0645  1.0452 -30.6509  1.0698 -29.7781  1.0944 -30.0655  1.1190 -30.3743  1.1436 -30.3246  1.1682 -30.3461  1.1928 -29.7550  1.2174 -29.7098  1.2420 -29.7630  1.2666 -29.6432  1.2911 -29.6000  1.3157 -29.3952  1.3403 -29.2478  1.3649 -28.7305  1.3895 -28.1505  1.4141 -28.0304  1.4387 -28.2620  1.4633 -28.2505  1.4879 -27.7118  1.5125 -27.9747  1.5371 -28.9418  1.5617 -28.0227  1.5863 -26.1442  1.6109 -26.2768  1.6355 -27.3931  1.6600 -27.2064  1.6846 -26.0047  1.7092 -25.4545  1.7338 -25.0821  1.7584 -25.8055  1.7830 -25.5649  1.8076 -24.2141  1.8322 -24.3991  1.8568 -24.3253  1.8814 -23.3204  1.9060 -23.2799  1.9306 -24.6075  1.9552 -23.0598  1.9798 -21.9166  2.0044 -23.0446  2.0289 -24.3066  2.0535 -22.6497  2.0781 -21.6390  2.1027 -21.6095  2.1273 -20.0776  2.1519 -20.0372  2.1765 -20.1475  2.2011 -20.6715  2.2257 -20.0745  2.2503 -20.1776  2.2749 -20.4430  2.2995 -18.3600  2.3241 -17.3884  2.3487 -19.3581  2.3733 -18.6751  2.3978 -17.7703  2.4224 -18.7576  2.4470 -17.3765  2.4716 -17.6485  2.4962 -17.4036  2.5208 -17.5094  2.5454 -18.1883  2.5700 -16.9344  2.5946 -15.9593  2.6192 -16.7445  2.6438 -16.4485  2.6684 -13.0664  2.6930 -13.9899  2.7176 -13.7777  2.7422 -12.5460  2.7667 -12.9989  2.7913 -12.6016  2.8159 -14.1298  2.8405 -11.6938  2.8651 -13.0314  2.8897 -14.8590  2.9143 -12.0945  2.9389 -11.5382  2.9635 -9.9689  2.9881 -10.5529  3.0127 -9.9092  3.0373 -8.3919  3.0619 -10.2333  3.0865 -11.3556  3.1111 -12.2490  3.1356 -8.5521  3.1602 -8.4134  3.1848 -8.4996  3.2094 -6.1080  3.2340 -10.1505  3.2586 -7.6816  3.2832 -3.6218  3.3078 -4.8298  3.3324 -3.2925  3.3570 -1.9001  3.3816 -1.4842  3.4062 -2.4058  3.4308 -3.0708  3.4554 -1.7753  3.4800 -3.5289  3.5045 1.1303  3.5291 3.3753  3.5537 -4.1832  3.5783 -6.2018  3.6029 -3.7461  3.6275 -2.4621  3.6521 -1.7582  3.6767 -2.1998  3.7013 -0.7192  3.7259 0.8756  3.7505 2.0909  3.7751 3.1249  3.7997 2.1201  3.8243 1.3554  3.8488 0.6845  3.8734 1.3111  3.8980 1.4889  3.9226 2.5076  3.9472 5.2536  3.9718 5.4049  3.9964 3.1631  4.0210 3.4423  4.0456 7.1524  4.0702 11.2342  4.0948 7.6063  4.1194 7.9772  4.1440 8.0888  4.1686 6.8629  4.1932 11.1548  4.2177 7.9673  4.2423 5.1015  4.2669 6.3299  4.2915 11.3122  4.3161 10.2115  4.3407 13.1079  4.3653 15.5885  4.3899 6.6191  4.4145 9.4712  4.4391 11.3246  4.4637 10.2128  4.4883 11.7376  4.5129 10.5490  4.5375 9.8428  4.5621 8.9156  4.5866 13.4269  4.6112 28.0889  4.6358 24.8255  4.6604 12.5994  4.6850 23.4416  4.7096 15.8200  4.7342 18.5758  4.7588 24.3507  4.7834 19.1650  4.8080 20.5695  4.8326 17.4436  4.8572 25.8087  4.8818 24.3101  4.9064 26.4232  4.9310 32.9723  4.9555 19.4931  4.9801 15.1692  5.0047 30.2864  5.0293 28.4703  5.0539 23.1262  5.0785 21.4499  5.1031 21.8346  5.1277 18.5124  5.1523 24.1145  5.1769 38.8958  5.2015 30.2366  5.2261 22.9394  5.2507 27.2315  5.2753 32.4144  5.2999 39.7320  5.3244 35.2432  5.3490 29.3884  5.3736 32.3261  5.3982 35.1552  5.4228 44.3525  5.4474 45.4375  5.4720 36.3951  5.4966 39.6902  5.5212 41.0406  5.5458 32.8382  5.5704 33.7604  5.5950 44.1585  5.6196 43.1308  5.6442 32.8834  5.6688 44.9074  5.6933 52.8577  5.7179 40.3613  5.7425 37.3559  5.7671 44.4586  5.7917 49.7970  5.8163 50.1518  5.8409 44.2895  5.8655 44.0953  5.8901 51.6967  5.9147 46.9935  5.9393 42.7713  5.9639 41.1067  5.9885 37.3430  6.0131 43.9187  6.0377 50.9254  6.0622 50.5054  6.0868 47.5556
/

%L=15
\color{B15}
\multiput {\tiny{$\bullet$}} at
0.3179 -51.3482  0.3398 -47.7884  0.3617 -45.0265  0.3836 -42.9641  0.4056 -41.6902  0.4275 -40.3889  0.4494 -38.9622  0.4713 -37.9378  0.4932 -37.1654  0.5152 -36.5470  0.5371 -36.1770  0.5590 -35.3158  0.5809 -35.0291  0.6029 -34.4991  0.6248 -33.5172  0.6467 -33.8214  0.6686 -33.3611  0.6905 -33.1735  0.7125 -33.0258  0.7344 -32.5246  0.7563 -32.4187  0.7782 -32.1541  0.8001 -32.0622  0.8221 -32.0147  0.8440 -32.3073  0.8659 -32.0553  0.8878 -31.2199  0.9098 -31.0074  0.9317 -31.5026  0.9536 -30.3179  0.9755 -29.5733  0.9974 -30.0916  1.0194 -30.5061  1.0413 -30.5943  1.0632 -29.1732  1.0851 -29.1347  1.1071 -29.4734  1.1290 -29.6465  1.1509 -29.4544  1.1728 -29.4475  1.1947 -29.8422  1.2167 -29.1026  1.2386 -29.0254  1.2605 -28.9854  1.2824 -29.4298  1.3044 -29.3070  1.3263 -28.6513  1.3482 -28.7545  1.3701 -27.9645  1.3920 -26.9744  1.4140 -28.1975  1.4359 -27.9936  1.4578 -27.0667  1.4797 -29.3201  1.5016 -27.1099  1.5236 -26.8966  1.5455 -25.2880  1.5674 -24.9085  1.5893 -28.3580  1.6113 -26.3717  1.6332 -25.0926  1.6551 -25.7313  1.6770 -25.0812  1.6989 -23.9210  1.7209 -24.4586  1.7428 -24.6782  1.7647 -24.9438  1.7866 -25.7457  1.8086 -24.9684  1.8305 -22.7413  1.8524 -21.8085  1.8743 -22.4160  1.8962 -23.3418  1.9182 -23.0961  1.9401 -22.5030  1.9620 -22.0641  1.9839 -22.5693  2.0059 -21.3129  2.0278 -20.2162  2.0497 -21.6592  2.0716 -19.7150  2.0935 -20.2375  2.1155 -21.8356  2.1374 -23.2241  2.1593 -21.5252  2.1812 -18.4439  2.2031 -19.4978  2.2251 -18.9505  2.2470 -19.7414  2.2689 -19.9751  2.2908 -18.3770  2.3128 -18.7247  2.3347 -19.0628  2.3566 -18.0780  2.3785 -18.1749  2.4004 -20.4934  2.4224 -20.0585  2.4443 -17.6659  2.4662 -16.3943  2.4881 -14.1739  2.5101 -15.9566  2.5320 -17.5645  2.5539 -16.8702  2.5758 -14.6307  2.5977 -13.2534  2.6197 -15.4730  2.6416 -15.9108  2.6635 -15.5567  2.6854 -14.6648  2.7074 -13.8315  2.7293 -14.3956  2.7512 -14.9355  2.7731 -14.5511  2.7950 -14.1455  2.8170 -15.1009  2.8389 -12.5321  2.8608 -9.8231  2.8827 -10.4570  2.9046 -10.3668  2.9266 -11.4547  2.9485 -10.9362  2.9704 -10.2120  2.9923 -10.3422  3.0143 -10.1571  3.0362 -11.2011  3.0581 -10.5245  3.0800 -9.4782  3.1019 -8.5294  3.1239 -8.9005  3.1458 -10.6951  3.1677 -8.7266  3.1896 -7.2135  3.2116 -7.9982  3.2335 -6.0879  3.2554 -4.5385  3.2773 -5.9635  3.2992 -6.2594  3.3212 -6.2131  3.3431 -7.3224  3.3650 -4.2247  3.3869 -3.2217  3.4089 -2.3684  3.4308 -2.8525  3.4527 -4.0427  3.4746 -2.3919  3.4965 -3.6543  3.5185 -4.0078  3.5404 -2.1123  3.5623 -2.8617  3.5842 -3.8377  3.6062 0.7846  3.6281 0.7527  3.6500 -2.5240  3.6719 -0.4459  3.6938 1.7745  3.7158 0.4473  3.7377 1.9104  3.7596 3.5707  3.7815 -0.7795  3.8034 0.2179  3.8254 2.4195  3.8473 -0.1221  3.8692 3.9557  3.8911 2.5735  3.9131 0.5444  3.9350 3.5413  3.9569 6.3864  3.9788 5.9936  4.0007 4.7570  4.0227 7.8534  4.0446 9.5013  4.0665 5.1872  4.0884 6.7058  4.1104 7.2814  4.1323 8.0238  4.1542 9.0360  4.1761 7.3422  4.1980 10.6071  4.2200 9.8368  4.2419 10.9032  4.2638 10.5338  4.2857 11.6565  4.3077 11.4250  4.3296 10.9915  4.3515 13.4598  4.3734 10.2703  4.3953 10.2115  4.4173 14.3347  4.4392 11.1600  4.4611 11.1087  4.4830 12.6522  4.5049 13.0022  4.5269 15.7987  4.5488 16.7612  4.5707 17.2355  4.5926 16.4024  4.6146 17.2819  4.6365 18.4802  4.6584 19.1692  4.6803 17.8323  4.7022 17.5844  4.7242 18.7647  4.7461 18.2910  4.7680 18.3220  4.7899 18.0234  4.8119 18.7164  4.8338 20.3871  4.8557 22.9254  4.8776 24.9705  4.8995 25.8443  4.9215 24.0240  4.9434 22.0728  4.9653 25.6982  4.9872 26.7258  5.0092 24.1984  5.0311 26.8881  5.0530 26.2435  5.0749 27.6838  5.0968 26.8185  5.1188 21.9750  5.1407 24.7815  5.1626 31.2332  5.1845 31.8612  5.2064 31.9226  5.2284 29.6252  5.2503 26.0676  5.2722 34.4958  5.2941 34.7893  5.3161 31.2880  5.3380 31.9339  5.3599 31.6494  5.3818 34.7080  5.4037 35.0223  5.4257 33.9932  5.4476 36.5652  5.4695 35.7407  5.4914 35.1381  5.5134 33.5246  5.5353 33.2120  5.5572 37.9792  5.5791 35.5839  5.6010 37.9349  5.6230 39.9225  5.6449 39.2884  5.6668 43.2014  5.6887 41.5256  5.7107 40.5924  5.7326 42.5458  5.7545 43.9372  5.7764 40.9696  5.7983 45.8057  5.8203 48.3145  5.8422 44.3397  5.8641 45.7810  5.8860 47.8745  5.9079 46.0539  5.9299 43.0058  5.9518 48.0895  5.9737 48.0388  5.9956 49.3373  6.0176 51.2896  6.0395 49.5401  6.0614 49.9693  6.0833 55.0232  6.1052 51.8184  6.1272 47.9601  6.1491 50.0700 
/




\color{black}
\normalcolor


\color{blue}

\normalcolor
\color{black}

\endpicture

==> Figures/figure21.tex <==


\beginpicture

\setcoordinatesystem units <40pt,2.15pt>
\axes{0}{-50}{0}{0}{7}{50}{-3}
\axis left shiftedto x=0 label {\Large$\Pi_{4_1} L^{3}$} 
      ticks
      withvalues -25 25 /
      at -25 25 /
 /  
\axis bottom shiftedto y=0 %label {$\phi$} 
    ticks
    withvalues 1 2 3 4 5 6 /
    at 1 2 3 4 5 6 /
/

\put {\Large$\phi L^{4/3}$} at 5.5 -15

\plot 4.1 0 4.1 -35 /
\put {$\phi_0L^{4/3}$} at 4.1 -40



\setplotsymbol ({\fiverm.})



%% 41 scaled

%L=4
\color{B04}
\multiput {\tiny{$\bullet$}} at
  3.6709 -49.4791  3.8693 -38.1848  4.0677 -27.3349  4.2661 -16.4908  4.4646 -5.2691  4.6630 6.7822  4.8614 20.1416  5.0598 35.4168  5.2583 53.3958  
 /

%L=5
\color{B05}
\multiput {\tiny{$\bullet$}} at
  3.0780 -49.3574  3.2148 -44.3745  3.3516 -39.6114  3.4884 -34.9596  3.6251 -30.3724  3.7619 -25.8599  3.8987 -21.4062  4.0355 -16.9348  4.1723 -12.3568  4.3091 -7.6971  4.4459 -2.9959  4.5827 1.8395  4.7195 6.8802  4.8563 12.1622  4.9931 17.6503  5.1299 23.3435  5.2667 29.2834  5.4035 35.5603  5.5403 42.2757  5.6771 49.4301 
  /

%L=6
\color{B06}
\multiput {\tiny{$\bullet$}} at
  2.5743 -50.8837  2.6752 -47.9563  2.7762 -45.1843  2.8771 -42.4612  2.9781 -39.8025  3.0790 -37.1073  3.1800 -34.4784  3.2809 -31.9079  3.3819 -29.2615  3.4828 -26.6953  3.5838 -24.1019  3.6847 -21.4786  3.7857 -18.8770  3.8866 -16.2517  3.9876 -13.5870  4.0885 -10.8938  4.1895 -8.2290  4.2904 -5.4916  4.3914 -2.6807  4.4923 0.1957  4.5933 3.1773  4.6942 6.1695  4.7952 9.1524  4.8961 12.2468  4.9971 15.5169  5.0980 18.7570  5.1990 22.0089  5.2999 25.4583  5.4009 29.0158  5.5018 32.6746  5.6028 36.4174  5.7037 40.2858  5.8047 44.2623  5.9056 48.3184  6.0066 52.5774 
  /

%L=7
\color{B07}
\multiput {\tiny{$\bullet$}} at
  2.2252 -50.3159  2.3033 -48.4344  2.3814 -46.6078  2.4595 -44.8524  2.5376 -42.9934  2.6156 -41.8004  2.6937 -40.2016  2.7718 -37.2976  2.8499 -35.6401  2.9280 -34.5634  3.0060 -32.7312  3.0841 -30.9872  3.1622 -29.3240  3.2403 -27.5780  3.3184 -25.8123  3.3964 -24.1024  3.4745 -22.4387  3.5526 -20.7384  3.6307 -18.9211  3.7087 -17.0842  3.7868 -15.3555  3.8649 -13.5393  3.9430 -11.6846  4.0211 -9.9134  4.0991 -8.0095  4.1772 -6.1687  4.2553 -4.2752  4.3334 -2.2933  4.4115 -0.4520  4.4895 1.3820  4.5676 3.4384  4.6457 5.5349  4.7238 7.5786  4.8018 9.7643  4.8799 11.9326  4.9580 14.0590  5.0361 16.2628  5.1142 18.3799  5.1922 20.5223  5.2703 22.8875  5.3484 25.3324  5.4265 27.5492  5.5046 29.9358  5.5826 32.6013  5.6607 35.0853  5.7388 37.6092  5.8169 40.2328  5.8950 43.0429  5.9730 45.6732  6.0511 48.3237
   /

%L=8
\color{B08}
\multiput {\tiny{$\bullet$}} at
  1.9062 -51.1269  1.9688 -49.4554  2.0312 -48.5128  2.0938 -47.2613  2.1562 -46.0258  2.2188 -44.9276  2.2812 -42.3622  2.3438 -42.1446  2.4062 -41.4034  2.4688 -38.4666  2.5312 -37.2225  2.5938 -36.6890  2.6562 -36.5272  2.7188 -35.8422  2.7812 -33.9160  2.8438 -32.1632  2.9062 -31.5335  2.9688 -30.2593  3.0312 -28.8938  3.0938 -28.4603  3.1562 -26.8738  3.2188 -23.8920  3.2812 -22.5419  3.3438 -23.2966  3.4062 -23.8768  3.4688 -20.6771  3.5312 -18.2103  3.5938 -18.9454  3.6562 -16.7347  3.7188 -14.4630  3.7812 -13.5311  3.8438 -10.6775  3.9062 -10.9441  3.9688 -8.8012  4.0312 -6.2670  4.0938 -7.4328  4.1562 -7.7563  4.2188 -2.8767  4.2812 0.6198  4.3438 -0.4962  4.4062 0.1181  4.4688 -0.2468  4.5312 2.9402  4.5938 5.7336  4.6562 7.4496  4.7188 5.9176  4.7812 7.6195  4.8438 11.6720  4.9062 12.9840  4.9688 14.9040  5.0312 14.5687  5.0938 15.8616  5.1562 17.4674  5.2188 19.4829  5.2812 23.1731  5.3438 24.6429  5.4062 26.0704  5.4688 31.4000  5.5312 32.1385  5.5938 30.3468  5.6562 33.5199  5.7188 35.3029  5.7812 37.3989  5.8438 39.5241  5.9062 38.7523  5.9688 40.8227  6.0312 45.5666
  /

%L=9
\color{B09}
\multiput {\tiny{$\bullet$}} at
  1.6692 -50.9354  1.7206 -50.3468  1.7719 -48.8643  1.8233 -48.3027  1.8746 -46.7151  1.9260 -45.7262  1.9774 -45.0449  2.0287 -44.3247  2.0801 -42.6941  2.1314 -41.4932  2.1828 -41.1580  2.2342 -40.1133  2.2855 -39.0579  2.3369 -38.4868  2.3882 -38.7407  2.4396 -36.5503  2.4910 -35.7547  2.5423 -36.5358  2.5937 -35.0885  2.6450 -33.3225  2.6964 -33.3888  2.7478 -31.7113  2.7991 -30.2882  2.8505 -31.5499  2.9018 -29.0706  2.9532 -25.7363  3.0046 -25.7449  3.0559 -25.7908  3.1073 -24.9908  3.1586 -26.4853  3.2100 -23.5941  3.2614 -20.8058  3.3127 -20.6589  3.3641 -19.1555  3.4154 -19.4927  3.4668 -19.3024  3.5182 -18.2022  3.5695 -15.3799  3.6209 -16.0023  3.6722 -15.2031  3.7236 -13.4194  3.7750 -13.8696  3.8263 -10.7707  3.8777 -11.5860  3.9290 -11.5822  3.9804 -7.7344  4.0318 -8.2501  4.0831 -6.3008  4.1345 -4.3543  4.1858 -1.2144  4.2372 -2.7383  4.2886 -4.5558  4.3399 -1.1685  4.3913 0.7087  4.4426 2.5381  4.4940 1.8796  4.5454 2.9868  4.5967 5.0990  4.6481 5.5979  4.6994 4.5391  4.7508 11.1312  4.8022 14.7885  4.8535 11.0048  4.9049 14.4897  4.9562 13.5514  5.0076 14.9472  5.0590 16.9269  5.1103 13.5229  5.1617 18.5803  5.2130 22.4153  5.2644 23.4297  5.3158 25.4259  5.3671 27.7982  5.4185 23.7163  5.4699 21.5221  5.5212 25.8817  5.5726 31.0401  5.6239 30.6303  5.6753 28.6672  5.7267 30.7050  5.7780 30.2921  5.8294 31.4887  5.8807 44.7506  5.9321 50.4017  5.9835 29.4506  6.0348 38.6136
 /

%L=10
\color{B10}
\multiput {\tiny{$\bullet$}} at
  1.4435 -50.2743  1.4866 -49.2821  1.5296 -48.6087  1.5727 -48.6499  1.6158 -47.9772  1.6589 -46.8446  1.7020 -46.0950  1.7451 -45.6951  1.7882 -44.3642  1.8313 -43.5836  1.8744 -43.7125  1.9174 -42.4219  1.9605 -41.7458  2.0036 -41.7200  2.0467 -40.8157  2.0898 -40.1330  2.1329 -39.3787  2.1760 -38.1346  2.2191 -37.9660  2.2622 -37.8031  2.3052 -36.3822  2.3483 -36.8865  2.3914 -36.1915  2.4345 -33.3239  2.4776 -32.9119  2.5207 -33.0425  2.5638 -33.7682  2.6069 -32.8023  2.6500 -32.1700  2.6930 -32.1041  2.7361 -30.6115  2.7792 -29.9090  2.8223 -28.4576  2.8654 -26.6862  2.9085 -26.7676  2.9516 -26.5493  2.9947 -24.8781  3.0378 -23.6969  3.0808 -24.5261  3.1239 -22.6642  3.1670 -22.6519  3.2101 -21.3372  3.2532 -20.6078  3.2963 -21.0005  3.3394 -18.2028  3.3825 -18.0321  3.4256 -16.8368  3.4686 -15.7569  3.5117 -15.0715  3.5548 -15.5915  3.5979 -12.9374  3.6410 -14.2573  3.6841 -13.4251  3.7272 -9.6817  3.7703 -12.8031  3.8133 -10.2680  3.8564 -8.6698  3.8995 -10.0311  3.9426 -7.7957  3.9857 -7.4910  4.0288 -7.4635  4.0719 -6.5950  4.1150 -4.3388  4.1581 -1.9919  4.2011 -2.3177  4.2442 -3.1664  4.2873 -3.7263  4.3304 0.4641  4.3735 3.6838  4.4166 2.1774  4.4597 -0.0877  4.5028 4.5399  4.5459 3.5094  4.5889 4.8989  4.6320 8.1850  4.6751 5.6247  4.7182 8.2252  4.7613 7.8998  4.8044 9.1599  4.8475 11.7692  4.8906 12.0138  4.9337 14.3395  4.9767 13.7512  5.0198 13.2700  5.0629 11.1238  5.1060 12.3878  5.1491 20.5868  5.1922 25.1295  5.2353 25.4482  5.2784 19.2220  5.3215 16.6131  5.3645 20.6526  5.4076 27.6320  5.4507 29.7763  5.4938 23.6903  5.5369 25.2860  5.5800 36.8751  5.6231 33.9356  5.6662 29.0427  5.7093 29.0808  5.7523 33.0387  5.7954 37.1803  5.8385 38.0099  5.8816 39.0517  5.9247 39.9309  5.9678 40.6118  6.0109 40.0330  6.0540 40.6446  6.0971 43.8730
  /

%L=11
\color{B11}
\multiput {\tiny{$\bullet$}} at
  1.2315 -50.3545  1.2682 -49.6451  1.3050 -49.9596  1.3417 -49.4196  1.3785 -48.1738  1.4153 -48.1550  1.4520 -47.5768  1.4888 -46.9920  1.5255 -46.5041  1.5623 -44.4997  1.5991 -45.0207  1.6358 -44.4326  1.6726 -42.8712  1.7093 -44.0009  1.7461 -43.6565  1.7829 -42.8454  1.8196 -42.0106  1.8564 -40.8199  1.8931 -41.2780  1.9299 -41.1582  1.9667 -38.6668  2.0034 -38.4706  2.0402 -40.2225  2.0769 -38.3709  2.1137 -36.9126  2.1505 -37.5747  2.1872 -36.9923  2.2240 -34.9518  2.2607 -33.7389  2.2975 -33.9938  2.3343 -33.6074  2.3710 -33.3515  2.4078 -32.8395  2.4445 -33.5880  2.4813 -32.6435  2.5181 -31.1628  2.5548 -31.4210  2.5916 -29.9839  2.6283 -30.2905  2.6651 -30.9150  2.7019 -29.5009  2.7386 -28.1567  2.7754 -27.7746  2.8121 -27.4929  2.8489 -26.7919  2.8857 -25.1408  2.9224 -26.1059  2.9592 -25.7148  2.9959 -23.4972  3.0327 -23.0152  3.0695 -21.2937  3.1062 -22.7678  3.1430 -20.3112  3.1797 -17.9662  3.2165 -19.9092  3.2533 -20.0577  3.2900 -18.0943  3.3268 -16.9230  3.3635 -19.6781  3.4003 -18.3233  3.4371 -16.7117  3.4738 -16.3562  3.5106 -14.4088  3.5473 -13.1075  3.5841 -14.0293  3.6209 -13.7616  3.6576 -11.8525  3.6944 -12.7656  3.7311 -9.7838  3.7679 -10.0268  3.8047 -10.4507  3.8414 -8.8529  3.8782 -10.7023  3.9149 -6.9060  3.9517 -5.6921  3.9885 -7.2838  4.0252 -5.7356  4.0620 -2.2838  4.0987 -3.8251  4.1355 -5.6879  4.1723 0.3167  4.2090 1.5507  4.2458 -1.4758  4.2825 -0.4553  4.3193 1.6909  4.3561 0.4081  4.3928 1.9731  4.4296 3.2235  4.4663 4.0051  4.5031 7.9002  4.5399 7.1874  4.5766 4.6622  4.6134 6.0554  4.6501 5.4518  4.6869 6.3039  4.7237 7.8898  4.7604 9.9071  4.7972 12.1869  4.8339 12.2040  4.8707 11.8235  4.9075 15.8995  4.9442 14.0709  4.9810 10.5357  5.0177 20.5254  5.0545 19.8510  5.0913 16.8435  5.1280 18.6688  5.1648 19.4453  5.2015 16.6222  5.2383 19.1619  5.2751 27.4764  5.3118 22.7245  5.3486 21.3983  5.3853 25.0577  5.4221 24.8817  5.4589 29.5903  5.4956 29.7862  5.5324 28.2043  5.5691 31.9320  5.6059 32.3726  5.6427 31.5421  5.6794 31.0243  5.7162 30.1034  5.7529 31.5463  5.7897 36.1647  5.8265 38.8745  5.8632 38.4237  5.9000 41.3191  5.9367 40.3535  5.9735 36.7039  6.0103 40.5066  6.0470 40.7076  6.0838 44.9853
 /

%L=12
\color{B12}
\multiput {\tiny{$\bullet$}} at
  1.0652 -50.6716  1.0970 -49.3175  1.1288 -49.0995  1.1606 -49.7857  1.1924 -48.9380  1.2242 -47.6356  1.2560 -47.1995  1.2878 -48.0541  1.3196 -47.6589  1.3514 -46.5527  1.3832 -45.1231  1.4150 -43.9879  1.4468 -44.4824  1.4786 -44.4092  1.5104 -43.6901  1.5422 -43.5083  1.5740 -43.7223  1.6058 -42.1310  1.6376 -41.3336  1.6694 -41.7206  1.7012 -41.4081  1.7330 -41.5619  1.7648 -41.0244  1.7966 -40.8658  1.8284 -40.1301  1.8602 -39.6059  1.8920 -40.0929  1.9238 -39.5033  1.9556 -37.4942  1.9874 -36.4070  2.0191 -36.8839  2.0509 -36.5660  2.0827 -35.5810  2.1145 -35.8304  2.1463 -36.3153  2.1781 -34.1918  2.2099 -33.4597  2.2417 -34.2867  2.2735 -33.6622  2.3053 -33.3169  2.3371 -32.9273  2.3689 -31.8812  2.4007 -30.8294  2.4325 -30.8571  2.4643 -32.1617  2.4961 -32.2003  2.5279 -29.7474  2.5597 -29.6123  2.5915 -30.0434  2.6233 -30.3644  2.6551 -29.6880  2.6869 -26.5947  2.7187 -27.8328  2.7505 -27.7066  2.7823 -26.8068  2.8141 -27.1121  2.8459 -24.4737  2.8777 -24.5439  2.9095 -26.0892  2.9413 -25.1287  2.9731 -23.6573  3.0049 -23.9667  3.0367 -22.4048  3.0685 -22.1202  3.1003 -22.7602  3.1321 -20.8374  3.1639 -19.9962  3.1957 -18.9998  3.2275 -18.9151  3.2593 -17.6948  3.2911 -15.6271  3.3229 -16.9638  3.3546 -17.6579  3.3864 -15.4647  3.4182 -16.4192  3.4500 -16.8241  3.4818 -11.9055  3.5136 -11.6538  3.5454 -13.9453  3.5772 -15.7830  3.6090 -14.9699  3.6408 -11.7555  3.6726 -10.7022  3.7044 -11.3309  3.7362 -12.9361  3.7680 -11.3733  3.7998 -8.9914  3.8316 -7.0309  3.8634 -5.3838  3.8952 -4.2852  3.9270 -6.5540  3.9588 -8.0699  3.9906 -5.7466  4.0224 -5.9579  4.0542 -5.2418  4.0860 -4.2387  4.1178 -4.3170  4.1496 -1.2080  4.1814 -0.8834  4.2132 -0.9461  4.2450 -0.4825  4.2768 -1.5028  4.3086 -0.4763  4.3404 1.4441  4.3722 3.7628  4.4040 3.5100  4.4358 4.4322  4.4676 6.7639  4.4994 6.6732  4.5312 4.7649  4.5630 3.3736  4.5948 7.0475  4.6266 10.1673  4.6584 11.9186  4.6901 7.7924  4.7219 7.7818  4.7537 13.1898  4.7855 11.1100  4.8173 10.9882  4.8491 15.8534  4.8809 17.1004  4.9127 14.4250  4.9445 11.9112  4.9763 17.1680  5.0081 16.4371  5.0399 12.5476  5.0717 18.0298  5.1035 20.0552  5.1353 20.6122  5.1671 18.8424  5.1989 22.2647  5.2307 22.8360  5.2625 18.8737  5.2943 21.9179  5.3261 25.5286  5.3579 24.0340  5.3897 27.4550  5.4215 29.5173  5.4533 26.6718  5.4851 27.2001  5.5169 26.8482  5.5487 26.6998  5.5805 25.3405  5.6123 28.0918  5.6441 29.6930  5.6759 36.3380  5.7077 36.4708  5.7395 31.3182  5.7713 37.1011  5.8031 39.8306  5.8349 37.1325  5.8667 37.6177  5.8985 34.0241  5.9303 32.9051  5.9621 38.8305  5.9939 40.8180  6.0256 44.5900  6.0574 46.2045 
   /

%L=13
\color{B13}
\multiput {\tiny{$\bullet$}} at
  0.9600 -47.1707  0.9878 -51.8041  1.0157 -54.0981  1.0435 -51.8388  1.0713 -50.3702  1.0991 -49.1242  1.1270 -50.0341  1.1548 -46.7930  1.1826 -45.6235  1.2105 -44.5625  1.2383 -43.8674  1.2661 -44.5979  1.2939 -43.5246  1.3218 -42.0511  1.3496 -42.7404  1.3774 -43.6549  1.4052 -42.0359  1.4331 -41.7874  1.4609 -42.5914  1.4887 -41.8038  1.5165 -41.2778  1.5444 -41.3519  1.5722 -40.1427  1.6000 -39.7460  1.6278 -40.7866  1.6557 -39.0449  1.6835 -38.3894  1.7113 -39.5751  1.7392 -38.8794  1.7670 -38.6297  1.7948 -37.8253  1.8226 -35.7048  1.8505 -34.6008  1.8783 -34.9798  1.9061 -36.3742  1.9339 -36.7770  1.9618 -36.1349  1.9896 -36.1227  2.0174 -34.5457  2.0452 -34.1824  2.0731 -35.4630  2.1009 -31.8455  2.1287 -31.5525  2.1565 -34.5546  2.1844 -32.8277  2.2122 -32.7748  2.2400 -30.6643  2.2679 -26.5240  2.2957 -29.5995  2.3235 -33.1092  2.3513 -29.3853  2.3792 -27.5266  2.4070 -29.0102  2.4348 -28.2961  2.4626 -27.7889  2.4905 -28.7756  2.5183 -27.8116  2.5461 -26.2607  2.5739 -26.0657  2.6018 -26.7472  2.6296 -27.8016  2.6574 -27.9634  2.6853 -24.1817  2.7131 -23.2579  2.7409 -26.8154  2.7687 -26.2815  2.7966 -21.6733  2.8244 -17.0418  2.8522 -17.1478  2.8800 -18.3347  2.9079 -19.7263  2.9357 -18.9508  2.9635 -25.8185  2.9913 -24.8240  3.0192 -18.3477  3.0470 -21.4776  3.0748 -22.3337  3.1026 -26.8533  3.1305 -19.6880  3.1583 -14.7861  3.1861 -19.3144  3.2140 -22.6575  3.2418 -21.9179  3.2696 -17.0315  3.2974 -17.5045  3.3253 -16.6793  3.3531 -16.3515  3.3809 -15.5313  3.4087 -15.8688  3.4366 -16.3557  3.4644 -12.1197  3.4922 -11.6001  3.5200 -14.0193  3.5479 -13.0411  3.5757 -12.3814  3.6035 -12.1914  3.6314 -11.4748  3.6592 -10.4300  3.6870 -10.8544  3.7148 -10.7165  3.7427 -6.9986  3.7705 -6.0138  3.7983 -10.1352  3.8261 -9.7577  3.8540 -7.7742  3.8818 -7.3748  3.9096 -6.9963  3.9374 -3.2067  3.9653 -2.7765  3.9931 -5.0754  4.0209 -4.8377  4.0487 -4.5950  4.0766 -3.3113  4.1044 -6.9908  4.1322 -5.7415  4.1601 -1.5382  4.1879 -1.0138  4.2157 -0.4848  4.2435 4.2591  4.2714 0.3522  4.2992 -2.8122  4.3270 2.2815  4.3548 5.9634  4.3827 6.3882  4.4105 2.2674  4.4383 3.2745  4.4661 4.0795  4.4940 4.4184  4.5218 5.3453  4.5496 6.1673  4.5775 6.3467  4.6053 6.6817  4.6331 7.3524  4.6609 7.2003  4.6888 11.6915  4.7166 12.1254  4.7444 8.9846  4.7722 10.3438  4.8001 13.0102  4.8279 13.8886  4.8557 12.6765  4.8835 13.3700  4.9114 14.1175  4.9392 15.0301  4.9670 14.8179  4.9948 15.2431  5.0227 16.8667  5.0505 18.1254  5.0783 18.5529  5.1062 19.0143  5.1340 19.2792  5.1618 19.5691  5.1896 19.8942  5.2175 20.3662  5.2453 20.8575  5.2731 20.4328  5.3009 22.2504  5.3288 23.8390  5.3566 23.5736  5.3844 24.9238  5.4122 25.0966  5.4401 26.6313  5.4679 27.7159  5.4957 26.8966  5.5235 27.7295  5.5514 29.1452  5.5792 30.2753  5.6070 30.8763  5.6349 30.4618  5.6627 31.2267  5.6905 31.6895  5.7183 32.2460  5.7462 33.0473  5.7740 33.6850  5.8018 36.2147  5.8296 37.5578  5.8575 37.4270  5.8853 37.8449  5.9131 38.2358  5.9409 37.9312  5.9688 39.4683  5.9966 41.0829  6.0244 40.9788 
/


%L=14
\color{B14}
\multiput {\tiny{$\bullet$}} at
   0.7747 -50.9303  0.7993 -50.2555  0.8239 -49.5427  0.8485 -49.4554  0.8731 -49.2226  0.8977 -48.2520  0.9222 -47.5436  0.9468 -46.7589  0.9714 -46.5534  0.9960 -46.6464  1.0206 -45.9231  1.0452 -46.2996  1.0698 -46.2559  1.0944 -44.9172  1.1190 -44.3658  1.1436 -44.4301  1.1682 -43.6726  1.1928 -43.7512  1.2174 -44.0799  1.2420 -43.1200  1.2666 -42.2298  1.2911 -42.1670  1.3157 -42.0625  1.3403 -41.4734  1.3649 -41.1594  1.3895 -41.7391  1.4141 -41.2072  1.4387 -40.6827  1.4633 -41.3083  1.4879 -41.4599  1.5125 -40.3062  1.5371 -40.1612  1.5617 -40.4630  1.5863 -39.9518  1.6109 -40.3243  1.6355 -38.8288  1.6600 -37.9366  1.6846 -38.3105  1.7092 -38.9366  1.7338 -38.2012  1.7584 -36.5299  1.7830 -37.2123  1.8076 -37.1274  1.8322 -36.6725  1.8568 -37.0122  1.8814 -35.9413  1.9060 -36.0631  1.9306 -35.2930  1.9552 -34.8435  1.9798 -35.5854  2.0044 -35.0475  2.0289 -35.2643  2.0535 -34.3524  2.0781 -32.6899  2.1027 -33.4434  2.1273 -34.4332  2.1519 -32.4501  2.1765 -31.9640  2.2011 -33.0626  2.2257 -31.7539  2.2503 -30.7655  2.2749 -31.3122  2.2995 -31.3640  2.3241 -30.7457  2.3487 -30.5602  2.3733 -30.0818  2.3978 -29.0046  2.4224 -29.4655  2.4470 -27.4451  2.4716 -25.9261  2.4962 -28.7281  2.5208 -28.9250  2.5454 -26.7685  2.5700 -26.9925  2.5946 -26.4940  2.6192 -25.6150  2.6438 -26.7647  2.6684 -27.4669  2.6930 -24.8571  2.7176 -23.9942  2.7422 -24.2380  2.7667 -22.7514  2.7913 -23.0104  2.8159 -22.4221  2.8405 -22.5365  2.8651 -23.0048  2.8897 -22.1309  2.9143 -20.8330  2.9389 -20.6518  2.9635 -20.4782  2.9881 -19.0352  3.0127 -19.3056  3.0373 -20.4016  3.0619 -20.6831  3.0865 -20.4055  3.1111 -19.5889  3.1356 -17.9663  3.1602 -18.2641  3.1848 -20.1453  3.2094 -17.9648  3.2340 -16.4936  3.2586 -17.2413  3.2832 -17.4434  3.3078 -14.2640  3.3324 -12.6239  3.3570 -16.2271  3.3816 -16.1541  3.4062 -15.9610  3.4308 -15.0206  3.4554 -12.0301  3.4800 -12.1857  3.5045 -13.8761  3.5291 -13.3993  3.5537 -13.5089  3.5783 -12.4725  3.6029 -10.9434  3.6275 -9.8837  3.6521 -10.3820  3.6767 -11.3077  3.7013 -10.7001  3.7259 -9.9902  3.7505 -7.7007  3.7751 -9.4597  3.7997 -8.7934  3.8243 -5.3971  3.8488 -5.9241  3.8734 -7.1377  3.8980 -6.4426  3.9226 -4.0943  3.9472 -5.1517  3.9718 -6.2779  3.9964 -3.6681  4.0210 -2.3770  4.0456 -3.9457  4.0702 -6.8588  4.0948 -3.2503  4.1194 -1.0038  4.1440 -2.8250  4.1686 -2.0376  4.1932 0.3806  4.2177 2.2085  4.2423 -0.5432  4.2669 -0.1813  4.2915 3.8922  4.3161 2.2626  4.3407 3.5210  4.3653 3.8483  4.3899 1.8103  4.4145 2.9099  4.4391 4.7899  4.4637 2.7811  4.4883 3.5568  4.5129 7.0048  4.5375 8.0128  4.5621 10.5489  4.5866 10.4240  4.6112 9.9829  4.6358 8.3516  4.6604 9.6245  4.6850 9.8839  4.7096 10.3626  4.7342 10.8198  4.7588 11.2002  4.7834 11.4988  4.8080 11.6155  4.8326 10.3687  4.8572 10.2153  4.8818 13.5472  4.9064 14.1378  4.9310 14.7854  4.9555 15.1367  4.9801 17.6652  5.0047 19.3899  5.0293 16.3025  5.0539 16.8196  5.0785 17.9324  5.1031 19.3839  5.1277 20.1948  5.1523 20.8393  5.1769 20.0263  5.2015 18.2443  5.2261 23.8531  5.2507 25.2270  5.2753 22.9183  5.2999 21.7770  5.3244 23.9819  5.3490 25.1910  5.3736 24.1065  5.3982 22.8643  5.4228 27.2582  5.4474 29.3834  5.4720 25.9694  5.4966 25.9421  5.5212 23.8070  5.5458 27.8878  5.5704 32.8788  5.5950 29.8225  5.6196 32.0654  5.6442 37.3423  5.6688 33.5275  5.6933 30.0406  5.7179 35.6489  5.7425 37.0186  5.7671 33.9284  5.7917 37.3641  5.8163 35.4811  5.8409 35.2734  5.8655 39.0019  5.8901 40.7251  5.9147 34.2966  5.9393 36.4247  5.9639 46.1104  5.9885 47.7594  6.0131 46.8228  6.0377 43.8240  6.0622 41.5773  6.0868 40.4654
/

%L=15
\color{B15}
\multiput {\tiny{$\bullet$}} at
  0.6905 -50.6187  0.7125 -50.0763  0.7344 -49.5361  0.7563 -48.9733  0.7782 -48.2945  0.8001 -47.8177  0.8221 -47.3296  0.8440 -46.8429  0.8659 -46.3540  0.8878 -45.9774  0.9098 -45.5631  0.9317 -45.3049  0.9536 -45.1436  0.9755 -45.2077  0.9974 -45.1678  1.0194 -43.9546  1.0413 -43.5769  1.0632 -43.8154  1.0851 -43.5083  1.1071 -43.0629  1.1290 -42.3209  1.1509 -41.8985  1.1728 -42.3046  1.1947 -42.3107  1.2167 -42.0907  1.2386 -41.6564  1.2605 -42.2838  1.2824 -41.7994  1.3044 -40.4243  1.3263 -41.8750  1.3482 -41.8691  1.3701 -41.1543  1.3920 -41.4684  1.4140 -40.6803  1.4359 -40.6659  1.4578 -40.3989  1.4797 -40.0997  1.5016 -39.3978  1.5236 -38.6192  1.5455 -39.3066  1.5674 -38.2428  1.5893 -36.9040  1.6113 -38.0215  1.6332 -39.3329  1.6551 -38.0710  1.6770 -38.0863  1.6989 -37.9578  1.7209 -36.8285  1.7428 -37.7536  1.7647 -37.5074  1.7866 -37.4007  1.8086 -36.8593  1.8305 -36.9148  1.8524 -35.8664  1.8743 -33.9314  1.8962 -35.9014  1.9182 -35.9884  1.9401 -32.0890  1.9620 -33.3023  1.9839 -35.4594  2.0059 -32.4133  2.0278 -36.4413  2.0497 -34.3165  2.0716 -29.8707  2.0935 -33.3387  2.1155 -32.9609  2.1374 -32.5812  2.1593 -31.2122  2.1812 -30.3861  2.2031 -31.2533  2.2251 -31.0899  2.2470 -30.0066  2.2689 -32.3861  2.2908 -31.6950  2.3128 -28.1212  2.3347 -28.7973  2.3566 -31.4334  2.3785 -29.2955  2.4004 -27.0882  2.4224 -28.2202  2.4443 -27.0184  2.4662 -27.5352  2.4881 -28.7959  2.5101 -28.8341  2.5320 -27.2937  2.5539 -26.1261  2.5758 -23.8418  2.5977 -25.3350  2.6197 -27.6446  2.6416 -25.2606  2.6635 -24.6915  2.6854 -22.8546  2.7074 -23.4688  2.7293 -25.4761  2.7512 -23.5904  2.7731 -23.8376  2.7950 -24.2885  2.8170 -23.4585  2.8389 -23.4367  2.8608 -23.7837  2.8827 -23.8928  2.9046 -22.4486  2.9266 -21.6638  2.9485 -20.7141  2.9704 -19.4743  2.9923 -19.3920  3.0143 -19.7616  3.0362 -20.0890  3.0581 -19.4663  3.0800 -17.4188  3.1019 -19.4974  3.1239 -18.3474  3.1458 -15.3474  3.1677 -17.5080  3.1896 -15.6508  3.2116 -15.9519  3.2335 -17.9971  3.2554 -17.2390  3.2773 -14.6159  3.2992 -14.2156  3.3212 -14.5840  3.3431 -13.4046  3.3650 -14.7654  3.3869 -15.0483  3.4089 -14.2491  3.4308 -14.0018  3.4527 -12.7334  3.4746 -12.5721  3.4965 -12.4353  3.5185 -10.8263  3.5404 -10.6135  3.5623 -11.8173  3.5842 -12.1140  3.6062 -11.4001  3.6281 -9.9484  3.6500 -9.8927  3.6719 -11.8264  3.6938 -9.0591  3.7158 -10.6206  3.7377 -11.6890  3.7596 -6.7092  3.7815 -3.8633  3.8034 -6.3927  3.8254 -6.8382  3.8473 -4.5689  3.8692 -4.8142  3.8911 -5.9094  3.9131 -6.0606  3.9350 -2.2768  3.9569 -2.2060  3.9788 -1.8104  4.0007 -0.2290  4.0227 -1.9502  4.0446 -3.3472  4.0665 0.6085  4.0884 -1.0106  4.1104 -3.0855  4.1323 -1.1791  4.1542 -2.4230  4.1761 0.3497  4.1980 0.9023  4.2200 -0.5920  4.2419 -0.1202  4.2638 0.9952  4.2857 5.8624  4.3077 3.9807  4.3296 0.7293  4.3515 2.1098  4.3734 4.3032  4.3953 5.1052  4.4173 3.7034  4.4392 5.5331  4.4611 5.5072  4.4830 3.2131  4.5049 6.7878  4.5269 10.2748  4.5488 7.7773  4.5707 7.2689  4.5926 7.5816  4.6146 7.2523  4.6365 6.8269  4.6584 9.4471  4.6803 10.2879  4.7022 8.7940  4.7242 12.6588  4.7461 11.6480  4.7680 9.5371  4.7899 12.7392  4.8119 9.4704  4.8338 7.7287  4.8557 13.4584  4.8776 14.7814  4.8995 17.8833  4.9215 21.3193  4.9434 19.1230  4.9653 15.9315  4.9872 14.4416  5.0092 14.5190  5.0311 16.2746  5.0530 17.0814  5.0749 18.0829  5.0968 21.7574  5.1188 22.5186  5.1407 21.1626  5.1626 19.2112  5.1845 18.0444  5.2064 21.4110  5.2284 24.0353  5.2503 25.3389  5.2722 29.1942  5.2941 25.8193  5.3161 23.5514  5.3380 29.0282  5.3599 28.3377  5.3818 24.3236  5.4037 25.0328  5.4257 26.3583  5.4476 25.6709  5.4695 28.2353  5.4914 29.8639  5.5134 24.5132  5.5353 24.8340  5.5572 32.5684  5.5791 29.2306  5.6010 24.6170  5.6230 33.8000  5.6449 37.8111  5.6668 34.8968  5.6887 36.7508  5.7107 31.6492  5.7326 35.1759  5.7545 36.5633  5.7764 32.5145  5.7983 32.4204  5.8203 33.3414  5.8422 37.5161  5.8641 35.4847  5.8860 36.6648  5.9079 35.2072  5.9299 35.6624  5.9518 37.6208  5.9737 41.3635  5.9956 40.5823  6.0176 40.9020 
/




\color{black}
\normalcolor


\color{blue}

\normalcolor
\color{black}

\endpicture

==> Figures/figureknots.tex <==

\beginpicture
\setcoordinatesystem units <1pt,1pt>
\setplotarea x from -20 to 420, y from -10 to 110
\setplotarea x from 0 to 400, y from 0 to 100

\setplotsymbol ({\footnotesize{$\bullet$}})

\setquadratic
%%unknot
\color{red}
\ellipticalarc axes ratio 8:10  360 degrees from 40 0 center at 40 50 
\color{black}
\normalcolor

\put {\Large$0_1$} at 50 -12 

%%trefoil
\color{red}
\setcoordinatesystem units <1pt,1pt> point at -135 0
\plot 92 52 80 35 70 24 60 15 50 8 40 2 30 0 /
\plot 30 0 20 2 10 12 0 30 0 50 10 70 30 80  / 
\plot 50 80 60 78 70 75 80 70 90 65 102 55  110 40 113 20 108 5 95 0 80 5 75 10 70 15 /
\plot 60 27 50 40 40 70 40 80 42 90 45 100 50 105 65 110 80 107 90 103 100 93 104 80 100 70   /
\color{black}
\normalcolor

\put {\Large$3_1$} at 65 -10 

%%figure eight
\color{red}
\setcoordinatesystem units <1pt,1pt> point at -300 0
\plot 55 50 65 40 67 30 65 20 60 12 50 4 40 0  30 2  20 7 10 15 0 30 -5 52 0 68 7 75 20 80 /
\plot 35 80 40 81 50 81.5 60 81 70 79 80 75 90 65 100 45 100 25 97 18  93 10 83 0 65 4  /
\plot 50 15 45 20 42 26 40 37 45 50 50 58 58 64 63 68 65 72  /
\plot 66 88  65 97 60 104 55 108 50 108  40 105 30 95  28 85 31 70  35 65 40 60  /
\color{black}
\normalcolor

\put {\Large$4_1$} at 55 -10 

\endpicture
